Transfer Learning via Contextual Invariants for One-to-Many Cross-Domain Recommendation

The rapid proliferation of new users and items on the social web has aggravated the gray-sheep user/long-tail item challenge in recommender systems. Historically, cross-domain co-clustering methods have successfully leveraged shared users and items across dense and sparse domains to improve inference quality. However, they rely on shared rating data and cannot scale to multiple sparse target domains (i.e., the one-to-many transfer setting). This, combined with the increasing adoption of neural recommender architectures, motivates us to develop scalable neural layer-transfer approaches for cross-domain learning. Our key intuition is to guide neural collaborative filtering with domain-invariant components shared across the dense and sparse domains, improving the user and item representations learned in the sparse domains. We leverage contextual invariances across domains to develop these shared modules, and demonstrate that with user-item interaction context, we can learn-to-learn informative representation spaces even with sparse interaction data. We show the effectiveness and scalability of our approach on two public datasets and a massive transaction dataset from Visa, a global payments technology company (19% Item Recall, 3x faster vs. training separate models for each domain). Our approach is applicable to both implicit and explicit feedback settings.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> SIGIR 2020 copy/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile/.tex/.pdf}; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*


==> SIGIR 2020 copy/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

==> SIGIR 2020 copy/datadesc.tex <==
% !TEX Root=draft.tex
\vspace{-5pt}
\section{Dataset Description}
\label{sec:Platform Description}


\begin{center}
 \begin{table}[b]
  \begin{tabular}{p{0.15\linewidth}lp{0.52\linewidth}}
   \toprule
   \textbf{Platform}                          & \textbf{Action} & \textbf{Description}              \\
   \midrule
   \multirow{7}{2cm}{\textbf{Coursera MOOC}}  & Play            & First lecture segment view        \\
                                              & Rewatch         & Repeat lecture segment view       \\
                                              & Clear Concept   & Back and forth movement, pauses   \\
                                              & Skip            & Unwatched lecture segment         \\
                                              & Create Thread   & Create forum thread for inquiries \\
                                              & Post            & Reply to existing threads         \\
                                              & Comment         & Comment on existing posts         \\
   \midrule
   \multirow{5}{2cm}{\textbf{Stack-Exchange}} & Question        & Posting a question                \\
                                              & Answer          & Authoring answer to a question    \\
                                              & Comment         & Comment on a question/answer      \\
                                              & Edit            & Modify posted content             \\
                                              & Follow          & Following posted content          \\
   \bottomrule
  \end{tabular}
  
  
%   \vspace{-5pt}
	\caption{User Action Description (Coursera/Stack-Exchange)}
  	\vspace{-15pt}
  	\label{t1}
 	\end{table}
	\end{center}
%\begin{center}
%\begin{table}
%\begin{tabular}{llll}
%\toprule
%\textbf{Platform} & \textbf{Link Label} & \textbf{Source Int} & \textbf{Target Int}\\
%\midrule
%\multirow{2}{*}{MOOC} & Commenting & Comment & Post\\
%& Posting & Post & Create Thread\\
%\midrule
%\multirow{3}{*}{Stack Ex.} & Commenting & Comment & Question/Answer\\
%& Answering & Answer & Question\\
%& Editing & Edit & Question/Answer\\
%%\bottomrule
%\bottomrule
%\end{tabular}
%\caption{Interaction Links}
%\label{t11}
%\end{table}
%\end{center}
%\begin{table*}
%\caption{Minimum Requirements for Automatic \textbf{Readmission} into the Commerce Faculty}
%\centering
%\begin{tabular}{ccccc}
%\toprule
%& \multicolumn{2}{c}{BCom} &
%\multicolumn{2}{c}{B.Bus.Sci} \\
%\cmidrule(r{4pt}){2-3} \cmidrule(l){4-5}
%& Number of courses required to pass & Cumulative Total of Courses & Number of courses &         Cumulative Total of Courses\\
%\midrule
%First year & 4 & 8 & 4 & 18 \\
%\bottomrule
%\end{tabular}
%\label{table:mr}
%\end{table*}
%\begin{center}
%\begin{table}
%\begin{tabular}{cp{0.7\linewidth}}
%\toprule
%\textbf{Symbol} & \textbf{Description} \\
%\midrule
%Question & Authoring a question on the stack exchange website\\
%Answer & Authoring an answer to a question on the stack exchange website\\
%Comment & Authoring a comment on a question or answer\\
%Edit & Modifying existing content via addition or deletion of text\\
%Favorite & Liking interesting or relevant content\\
%\bottomrule
%\end{tabular}
%\caption{User Action Set - Stack Exchange}
%\label{t2}
%\end{table}
%\end{center}
%
%\begin{center}
%\begin{table}
%\begin{tabular}{lll}
%\toprule
%\textbf{Link Label} & \textbf{Source Interaction} & \textbf{Target Interaction}\\
%\midrule
%Commenting & Comment & Question/Answer\\
%Answering & Answer & Question\\
%Editing & Edit & Question/Answer\\
%\bottomrule
%\end{tabular}
%\caption{Interaction Links - Stack Exchange}
%\label{t22}
%\end{table}
%\end{center}
% \vspace{-16pt}
% \textbf{Stack-Exchange Q\&A Networks: }
\vspace{-15pt}
We now provide a brief description of the Coursera MOOC and Stack-Exchange datasets that we use in our experiments and characterize them in terms of skew and sparsity.

Stack-Exchanges are community Q\&A websites where participants discuss a wide range of topics. Users interact with each other and perform a range of actions (e.g. post question, answer, comment etc.). We experiment on 10 Stack-Exchanges, chosen for thematic diversity and size variation. Coursera MOOCs feature video lectures for students to watch and a forum where students and instructors can interact. We analyze the actions (e.g. play, skip, rewind etc.) on the videos, lecture content via subtitles, and the forum interaction for four MOOCs, chosen for thematic diversity. The user action types and datasets are summarized in~~\Cref{t1} and~\Cref{d1} respectively.

% exchanges between students and instructors via course forums. Patterns of lecture viewing obtained from video clickstreams provide valuable cues on learning behavior \cite{mooc1, ladfg}, in addition to forum activity \cite{forum1}. We combine these two sources to define the action set of students (\Cref{t1}). Lecture content is extracted from subtitle files. Students engage in exchanges by posting or commenting on forum content. We conduct our experiment with both, technical and non-technical MOOCs (\Cref{d1}).



% domains of public interest. Users interact by asking/answering questions, and editing, following and commenting on content (\Cref{t1}). Users engage in knowledge-exchange by answering questions and editing/commenting each other's content. We conduct our experiments on several Stack-Exchange websites chosen to capture diverse technical and non-technical subjects and differently sized user populations (\Cref{d1}).
%reacting to other users' activity, specifically liking and editing content, favorite, and answering questions hence establishing Editing, Liking and Answering links between pairs of users, indicative of their interests and knowledge
\begin{center}
 \begin{table}
  \caption{Preliminary analysis indicates significant behavior skew and inactive user proportion, although slightly reduced in specialized domains like Christianity}
  \vspace{-10pt}
  \begin{tabular}{@{}p{0.14\linewidth}p{0.19\linewidth}cccc@{}}
   \toprule
   \textbf{Platform}                             & \textbf{Dataset} & \textbf{Users} & \textbf{Interactions} & \textbf{$\eta_t$} & \textbf{$S_N$} \\
   \midrule
   \multirow{4}{2.2cm}{\textbf{Coursera MOOC}} & Comp Sci-1       & 26,542         & 834,439               & -2.51             & 0.67           \\  
   												& Math             & 10,796         & 162,810               & -2.90             & 0.69           \\
                                                 & Nature           & 6,940          & 197,367               & -2.43             & 0.70           \\
                                                 
                                                 & Comp Sci-2       & 10,796         & 165,830               & -2.14             & 0.73           \\
   \midrule
   \multirow{10}{2.2cm}{\textbf{Stack-Exchange}} & Ask-Ubuntu       & 220,365        & 2,075,611             & -2.81             & 0.65           \\
                                                 & Android          & 28,749         & 182,284               & -2.32             & 0.56           \\
                                                 & Travel           & 20,961         & 277,823               & -2.01             & 0.66           \\
                                                 & Movies           & 14,965         & 150,195               & -2.17             & 0.67           \\
                                                 & Chemistry        & 13,052         & 175,519               & -2.05             & 0.63           \\
                                                 & Biology          & 10,031         & 138,850               & -2.03             & 0.71           \\
                                                 & Workplace        & 19,820         & 275,162               & -2.05             & 0.59           \\
                                                 & Christianity     & 6,417          & 130,822               & -1.71             & 0.64           \\
                                                 & Comp Sci         & 16,954         & 183,260               & -2.26             & 0.62           \\
                                                 & Money            & 16,688         & 179,581               & -1.72             & 0.63           \\
   \bottomrule
  \end{tabular}

  \label{d1}
%   \vspace{-5pt}
 \end{table}

\end{center}


% \vspace{-13pt}
% \textbf{Coursera MOOC Platform: } Coursera MOOCs feature a structured learning environment with lecture content and exchanges between students and instructors via course forums. Patterns of lecture viewing obtained from video clickstreams provide valuable cues on learning behavior \cite{mooc1, ladfg}, in addition to forum activity \cite{forum1}. We combine these two sources to define the action set of students (\Cref{t1}). Lecture content is extracted from subtitle files. Students engage in exchanges by posting or commenting on forum content. We conduct our experiment with both, technical and non-technical MOOCs (\Cref{d1}).

% \vspace{2pt}
\vspace{-18pt}
To get a feel for these datasets, let us examine sparsity and behavior skew. To understand sparsity, we compute the power-law ($f_w = c.w^{\eta_t}$) exponent $\eta_t$ that best describes the fraction of users $f_w$ who were active for $w$-weeks. A more negative index indicates that fewer users are consistently active. As a reference point, when $\eta_t=0$, a constant fraction of users are always active. Thus when we notice that $\eta_t=-2.81$ for \texttt{Ask Ubuntu} Stack Exchange in~\Cref{d1}, it means that the number of users who are active for two weeks is just $14\%$ of those active for one week.~\Cref{d1} indicates that larger Stack Exchanges tend to have greater sparsity.

We measure skew by first identifying the dominant action type or style of each user (e.g commenter, editor) and then compute the normalized entropy $S_N$ of the resulting user distribution.
% Activity skew (excluding text content) can be approximated by grouping users by dominant action type (e.g. users who mostly comment or ask questions), and computing the normalized entropy ($S_N$) of the resulting distribution.
In a large Stack-Exchange such as \texttt{Ask-Ubuntu}, while less than 5\% (c.f~\Cref{skew_sparsity})  of the users have `Answer' as their dominant type, over 60\% of the users have `Comment' as their dominant action. This does not consider content topics, which result in even greater skew. When $S_N=1$, all dominant action types are equally likely; in contrast $S_N=0$ indicates a single dominant action type. In MOOCs, 'Play' is the dominant action type with low forum participation (participation rates $\sim$10-15\% in our MOOC forums).




% It is interesting to observe that larger Stack-Exchanges have more inactive users in comparison to more niche domains of discussion. We explicitly compare the effects of skew and sparsity in our prediction results on these datasets (\Cref{sec:Result Analysis} and 7.5).


==> SIGIR 2020 copy/experiments.tex <==
%!TEX root = draft.tex
\section{Experimental Results}
\label{sec:Experimental Results}
In this section, we present experimental analyses on diverse multi-domain recommendation datasets and show two key results. First, when we adapt modules trained on a rich source domain to the sparse target domains, we significantly reduce the computational costs and improve performance in comparison to learning directly on the sparse domains. Second, our model is comparable to \textit{state-of-the-art} baselines when trained on a single domain without transfer.
%\noindent
%\textbf{A: } Our recommender outperforms state-of-the-art baselines when trained in isolation, i.e., without meta-transfer.
%
%\noindent
%\textbf{B: } We observe performance and scalability gains under meta-transfer to the sparse targets vs. training them separately.
%
%We introduce datasets, baseline methods in \Cref{subsec:Datasets}, followed by the recommendation task and meta-transfer gains on sparse target domains in \Cref{subsec:Recommendation}, \Cref{subsec:Meta-Transfer-Exp}, qualitative analyses in \Cref{subsec:Qualitative} and scalability, robustness in~\Cref{subsec:Scale-Robust}. Finally, we discuss limitations and future directions in \Cref{subsec:Limitations}.
%We examine two critical questions: Q1---\textit{What is the effect of adversary weight $\lambda$ on interest space collapse and does this depend on the generator architecture?} and Q2---\textit{Is adversarial training robust to missing social or item history user data?} Finally, we analyze parameter sensitivity in \Cref{subsec:Parameter Sensitivity} and discuss limitations in~\Cref{subsec:Limitations}.
\begin{table}[b]
\centering
\vspace{-12pt}
\begin{tabular}{@{}p{0.120\linewidth}p{0.025\linewidth}p{0.240\linewidth}p{0.11\linewidth}p{0.10\linewidth}p{0.205\linewidth}@{}}
\toprule
\textbf{Dataset} &\textbf{}& \textbf{State} & \textbf{Users} & \textbf{Items} & \textbf{Interactions} \\ 
\midrule
 & \textbf{S} & \textbf{Bay-Area CA} & \textbf{1.20 m} & \textbf{8.90 k} & \textbf{25.0 m}  \\
\multirow{1}{*}{\textbf{FT-Data}} & $\mathbf{T}_1$ & Arkansas  & 0.40 m & 3.10 k & 5.20 m  \\
\multirow{1}{*}{$|\mathbf{C}| = 220$} & $\mathbf{T}_2$ & Kansas & 0.35 m & 2.90 k & 5.10 m  \\
& $\mathbf{T}_3$ & New-Mexico & 0.32 m & 2.80 k & 6.20 m  \\
& $\mathbf{T}_4$ & Iowa & 0.30 m & 3.00 k &  4.80 m  \\
\midrule
& \textbf{S} & \textbf{Pennsylvania} & \textbf{10.3 k} & \textbf{5.5 k} &\textbf{170 k}  \\
\multirow{1}{*}{\textbf{Yelp}}  & $\mathbf{T}_1$ & Alberta, Canada & 5.10 k & 3.5 k & 55.0 k  \\
\multirow{1}{*}{$|\mathbf{C}| = 120$} & $\mathbf{T}_2$ & Illinois  & 1.80 k& 1.05 k & 23.0 k  \\
& $\mathbf{T}_3$ & S.Carolina  & 0.60 k & 0.40 k & 6.20 k  \\
\midrule
  \multirow{1}{*}{\textbf{Google}}& \textbf{S} & \textbf{California} & \textbf{46 k} & \textbf{28 k} & \textbf{320 k}  \\
\multirow{1}{*}{\textbf{Local}} & $\mathbf{T}_1$ & Colorado & 10 k & 5.7 k & 51.0 k  \\
\multirow{1}{*}{$|\mathbf{C}| = 90$} & $\mathbf{T}_2$ & Michigan & 7.0 k & 4.0 k & 29.0 k  \\
& $\mathbf{T}_3$ & Ohio & 5.4 k & 3.2 k & 23.0 k  \\
\bottomrule
\end{tabular}
\label{data_stats}
\caption{\textit{Source} and \textit{Target} statistics for each of our datasets. Source states denoted S have more interactions and interaction density per user than target states denoted $\mathbf{T}_{i}$.}
\vspace{-14pt}
\end{table}
\subsection{Datasets and Baselines}
\label{subsec:Datasets}
We evaluate our recommendation model both with and without module transfer over the publicly available \textit{Yelp}\footnote{\url{https://www.yelp.com/dataset/challenge}} and \textit{Google Local Reviews}\footnote{\url{http://cseweb.ucsd.edu/~jmcauley/datasets.html}} datasets for benchmarking purposes. Reviews are split across U.S and Canadian states in these datasets. We treat each state as a separate recommendation domain for training and transfer purposes. There is no \textit{user or item overlap} across the states (recommendation domains) in any of our datasets. We repeat our experiments with a large-scale restaurant transaction dataset obtained from Visa (referred to as \textit{FT-Data}), also split across U.S. states. 
% They provide direct and inferred contextual features for each user rating (\textit{explicit feedback}) on businesses across FT-Data provides \textit{implicit feedback} to user (cardholder) preferences via transactions with businesses. Across all datasets, we observe significant performance gaps across states owing to variations in the interaction volume, density and quality. 
\begin{description}[leftmargin=0pt, labelindent=\parindent]
\item[\textbf{Google Local Reviews Dataset} (\textit{Explicit feedback})\footnote{\url{http://cseweb.ucsd.edu/~jmcauley/datasets.html}}\cite{mcauley1, mcauley2}:] Users rate businesses on a 0-5 scale with temporal, spatial, and textual context available for each review. We also infer additional context features - users' preferred locations on weekdays and weekends, spatial patterns and preferred product categories.
\item[\textbf{Yelp Challenge Dataset} (\textit{Explicit feedback}) \footnote{https://www.yelp.com/dataset/challenge}:] Users rate restaurants on a 0-5 scale, reviews include similar context features as the Google Local dataset. Further, \textit{user check-ins} and restaurant attributes (e.g., \textit{accepts-cards}) are available.
\item[\textbf{\textit{FT-Data}} (\textit{Implicit feedback}):] Contains the credit/debit card payments of users to restaurants in the U.S, with spatial, temporal, financial context features, and inferred transaction attributes. We leverage transaction histories also to infer user spending habits, restaurant popularity, peak hours, and tipping patterns.
\end{description}
In each dataset, we extract the same context features for every state with state-wise normalization, either with min-max normalization or quantile binning. We retain users and items with three or more reviews in the Google Local dataset and ten or more reviews in the Yelp dataset. In \textit{FT-Data}, we retain users and restaurants with over ten, twenty transactions, respectively, over three months. In each dataset, we choose a dense state with ample data as the source domain where all modules are trained, and multiple sparse states as target domains for module transfer from the source.
\vspace{-2pt}
\subsubsection{Source to Target Module Transfer}
\label{subsec:metabaselines}
We evaluate the performance gains obtained when we transfer or adapt modules $\mathcal{M}^1, \mathcal{M}^3$ and $\mathcal{M}^4$ from the source state to each target state, in comparison to training all four modules directly on the target. We also compare target domain gains with \textit{state-of-the-art} meta-learning baselines:
\begin{description}[leftmargin=0pt]
\item \textbf{LWA} \cite{nips17}: Learns a shared meta-model across all domains, with a user-specific linear component.
\item \textbf{NLBA} \cite{nips17}: Replaces LWA's linear component with a neural network with user-specific layer biases.
\item \textbf{$\mathbf{s^2}$-Meta} \cite{kdd19}: Develops a meta-learner to instantiate and train recommender models for each scenario. In our datasets, scenarios are the different states.
%\vspace{0.10in}
\item[\textbf{Direct Layer-Transfer (Our Variant)}:] Transfers source-trained meta-modules to the target-trained models as in \Cref{subsec:DLT}.
\item[\textbf{Anneal (Our Variant)}:] We apply simulated annealing to adapt the transferred meta-modules to the target as in \Cref{subsec:anneal}.
\item[\textbf{DRR - Distributionally Regularized Residuals}: ] \textbf{(Our Main Approach)} Adapts the inputs of each transferred module with separate residual layers in each target state. (\Cref{subsec:DRR}).
\end{description}
\vspace{-2pt}
\subsubsection{Single Domain Recommendation Performance}
We also evaluate the performance of our models independently without transfer on the source and target states in each dataset. We compare with the following \textit{state-of-the-art} recommendation baselines: 
%For each dataset, we train our recommender system on each state in isolation. When each model is trained and tested on its own state, the source-trained model significantly outperforms the target-only models. We compare our source model performance against , and demonstate the effectiveness of the proposed context transform model. We also experimentally validate that the learned transforms are generalizable and extensible to the target states. Our baselines are:
%% \vspace{-2pt}
%
\vspace{-2pt}
\begin{description}[leftmargin=0pt, labelindent=\parindent]
\item \textbf{NCF} \cite{ncf}: \textit{State-of-the-art} non context-aware model for comparisons and context validation.
\item \textbf{CAMF-C} \cite{camf}: Augments Matrix Factorization to incorporate a context-bias term for item latent factors. This version assumes a fixed bias for a given context feature for all items.
\item \textbf{CAMF} \cite{camf}: CAMF-C with separate context bias values for each item. We use this version for comparisons.
\item \textbf{MTF} \cite{ctf}: Obtains latent representations via decomposition of the User-Item-Context tensor. This model scales very poorly with the size of the context vector.
\item \textbf{NFM} \cite{nfm}:  Employs a bilinear interaction model applied to the context features of each interaction for representation. 
\item \textbf{AFM} \cite{afm}: Incorporates an attention mechanism to reweight the bilinear pooled factors in the NFM model. Scales poorly with the number of pooled contextual factors.
\item \textbf{AIN} \cite{cikm18context}: Reweights the interactions of user and item representations with each contextual factor via attention.
%\vspace{0.10in}
\item \textbf{MMT-Net (Our Main Approach)}: We refer to our model with all four modules as Multi-Linear Module Transfer Network (MMT-Net).
\item \textbf{FMT-Net (Our Variant)}: We replace $\mathcal{M}^1$s layers with feedforward \textit{RelU} layers to demonstrate the importance of multiplicative context invariants.
\item \textbf{MMT-Net Multimodal (Our Variant)}: \textbf{MMT-Net} with the information-gain terms described in \Cref{multimodal}. Only applied to \textit{FT-Data} due to lack of interactional features in other datasets.
\end{description}
\subsubsection{Experiment Setup}
We tune each baseline in parameter ranges centered at the author provided values for each dataset and set all embedding dimensions to $200$ for uniformity. We split each state in each dataset into training (80\%), validation (10\%), and test (10\%) sets for training, tuning, and testing purposes. 
For the \textit{implicit feedback} setting in \textit{FT-Data}, we adopt the standard negative-sample evaluation \cite{ncf} and draw one-hundred negatives per positive, equally split between item and context negatives similar to the training process in \Cref{subsec:Train}. We then evaluate the average \textbf{Hit-Rate@K} (\textbf{H@K}) metric for $K=1,5$ in \Cref{implicit_results}, indicating if the positive sample was ranked highly among the negative samples. For the \textit{explicit feedback} setting in the other two datasets, we follow the standard \textbf{RMSE} and \textbf{MAE} metrics in \Cref{explicit_results} \cite{camf, cikm18context} (no negative samples required). All models were implemented with \textit{Tensorflow} and tested on a \textit{Nvidia Tesla V100 GPU}. 
\begin{table}[hbtp]
 \centering
 \vspace{-6pt}
 \caption{Comparing aspects addressed by baseline recommendation models against our proposed \textbf{MMT-Net} approach}
 \vspace{-9pt}
 \begin{tabular}{@{}p{0.055\linewidth}p{0.165\linewidth}p{0.22\linewidth}p{0.08\linewidth}p{0.115\linewidth}p{0.18\linewidth}@{}}
  \toprule
     \textbf{} & \textbf{Bi-Linear Pooling} & \textbf{Multi-Linear Pooling} & \textbf{Low-Rank} & \textbf{Factor Weights} & \textbf{$\mathbf{\Theta}$(Context)}                                                                                                                           \\
  \midrule
\textbf{NFM} & Yes & No & No & No & Linear\\
\textbf{AFM} & Yes & No & No & Yes & Quadratic\\
\textbf{AIN} & No & No & Yes & Yes & Linear\\
\textbf{FMT} & No & No & Yes & Yes & Linear\\
\midrule
\textbf{MMT} & Yes & Yes & Yes & Yes & Linear\\
  \bottomrule
 \end{tabular}
 \label{methods}
 \vspace{-12pt}
\end{table}
\subsection{Module Transfer to Sparse Target States}
\label{subsec:Meta-Transfer-Exp}
\begin{table}[b]
\vspace{-10pt}
\centering
\begin{tabular}{@{}p{0.120\linewidth}p{0.03\linewidth}p{0.085\linewidth}p{0.1\linewidth}p{0.080\linewidth}p{0.080\linewidth}p{0.085\linewidth}p{0.140\linewidth}@{}}
\toprule
\textbf{Dataset} & \textbf{} & \textbf{Direct} & \textbf{Anneal} & \textbf{DRR} & \textbf{LWA} & \textbf{NLBA}  & $\mathbf{s^2}$\textbf{-Meta}   \\ 
\small\textbf{} & \small\textbf{} & \small\textbf{\%H@1} & \small\textbf{\%H@1} & \small\textbf{\%H@1} & \small\textbf{\%H@1} & \small\textbf{\%H@1} & \small\textbf{\%H@1} \\
\midrule
\multirow{4}{*}{\textbf{FT-Data}} & $T_1$ & 2\% & \textbf{19\%}  & 18\%  & 6\%  & x & x \\
& $T_2$ & 0\%  & \textbf{16\%}  & \textbf{16\%}  & 8\%  & x & x \\
& $T_3$ & 3\%  & \textbf{18\%}  & \textbf{18\%}  & 6\%   & x & x \\
& $T_4$ & -1\%  & \textbf{14\%} &  12\%  & 11\%  & x & x \\
\bottomrule
\end{tabular}
\vspace{2pt}
\caption{Percentage improvements (\textbf{\% Hit-Rate@1}) on \textit{FT-Data} target states with module transfer approaches and meta-learning baselines against training all modules on the target state directly as in \Cref{implicit_results}.}
\label{implicit_meta_results}
\vspace{-21pt}
\end{table}
We evaluate module transfer methods by the percentage improvements in the \textbf{Hit-Rate@1} for the implicit feedback setting in \textit{FT-Data} (\Cref{implicit_meta_results}), or the drop in \textbf{RMSE} (\Cref{explicit_meta_results}) for the explicit feedback datasets when we transfer the $\mathcal{M}^1, \mathcal{M}^3$ and $\mathcal{M}^4$ modules from the source state rather than training all four modules from scratch on that target domain. Similarly, meta-learning baselines were evaluated by comparing their joint meta-model performance on the target state against our model trained only on that state. The performance numbers for training our model on each target state without transfer are recorded in \Cref{explicit_results}, \Cref{implicit_results}.
We could not scale the NLBA, LWA and \textbf{$\mathbf{s^2}$-Meta} approaches to \textit{FT-Data} owing to the costs of training the meta-models on all users combined across the source and multiple target domains. In \Cref{explicit_meta_results}, we demonstrate the percentage reduction in RMSE with module transfer for Google Local, Yelp, and in \Cref{implicit_meta_results}, we demonstrate significant improvements in the hit-rates for \textit{FT-Data}. We start with an analysis of the training process for module transfer with simulated annealing and DRR adaptation.
%\begin{figure}
%\includegraphics[width=0.89\linewidth]{images/plots/scaling-image.pdf}
%\caption{.}
%\label{scaling-image}
%\end{figure}
%\begin{figure}
%\includegraphics[width=0.89\linewidth]{images/plots/Google-Local-MI.pdf}
%\label{Google-Local-MI}
%\caption{The Train-RMSE values of MMT-Net when trained on just the target (Google-Local MI), when annealed and learned with residuals after 2 epochs of pre-training.}
%\end{figure}
%
%\begin{figure}
%\includegraphics[width=0.89\linewidth]{images/plots/Google-Local-OH.pdf}
%\label{Google-Local-OH}
%\caption{The Train-RMSE values of MMT-Net when trained on just the target (Google-Local OH), when annealed and learned with residuals after 2 epochs of pre-training.}
%\end{figure}
\begin{table}[t]
\centering
%\begin{tabular}{@{}p{0.102\linewidth}p{0.05\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}p{0.039\linewidth}@{}}
%\toprule
%\textbf{Dataset} & \textbf{Target} & \multicolumn{2}{c}{\textbf{Direct}} & \multicolumn{2}{c}{\textbf{Anneal}} & \multicolumn{2}{c}{\textbf{DRR}} & \multicolumn{2}{c}{\textbf{LWA}}  & \multicolumn{2}{c}{\textbf{NLBA}}  & \multicolumn{2}{c}{$\mathbf{s^2}$\textbf{-Meta}}   \\ 
%
%\textit{} & \textit{} & \textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} &\textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} \\
\caption{Percentage RMSE improvements on the Yelp and Google Local target states with module transfer approaches and meta-learning baselines against training all modules on the target state directly as in \Cref{explicit_results}.}
\vspace{-10pt}
\begin{tabular}{@{}p{0.12\linewidth}p{0.03\linewidth}p{0.085\linewidth}p{0.1\linewidth}p{0.080\linewidth}p{0.080\linewidth}p{0.085\linewidth}p{0.140\linewidth}@{}}
\toprule
\textbf{Dataset} & \textbf{} & \textbf{Direct} & \textbf{Anneal} & \textbf{DRR} & \textbf{LWA} & \textbf{NLBA}  & $\mathbf{s^2}$\textbf{-Meta}   \\ 
\small\textbf{} & \small\textbf{} & \small\textbf{\%RMSE} & \small\textbf{\%RMSE} & \small\textbf{\%RMSE} & \small\textbf{\%RMSE} & \small\textbf{\%RMSE} & \small\textbf{\%RMSE} \\
\midrule
\multirow{3}{*}{\textbf{Yelp}} & $T_1$ & -2.2\% &\textbf{ 7.7\%}  &7.2\% & 2.6\% & 4.1\% & 3.7\%  \\
& $T_2$ & -2.6\% & \textbf{9.0\%}  & 7.9\%& 1.8\% & 3.6\%  & 3.1\%  \\
& $T_3$ & 0.8\%  & \textbf{8.5\%}  & 8.1\%  & 0.3\%  & 5.3\%  & 1.8\%  \\
\midrule
\multirow{1}{*}{\parbox{0.12\linewidth}{\textbf{Google}}} & $T_1$ & -1.2\%  & \textbf{11.2\%}  & 11.0\%  & 3.3\% & 4.3\%  & 3.1\%  \\
\textbf{Local} & $T_2$ & -1.7\%  & \textbf{12.1\%}  & 10.9\%  & 4.6\%  & 4.9\% & 2.8\%\\
 & $T_3$ & -2.0\%  & \textbf{9.6\%}  & 8.8\%  & 2.4\%  & 6.3\% & 3.9\%  \\
\bottomrule
\end{tabular}
\label{explicit_meta_results}
\vspace{-22pt}
\end{table}

\textbf{Transfer Details: } On each target state in each dataset, all four modules of our MMT-Net model are pretrained over two gradient epochs on the target samples. The layers in modules $\mathcal{M}^1, \mathcal{M}^3$ and $\mathcal{M}^4$ are then replaced with those trained on the source state, while retaining module $\mathcal{M}^2$ without any changes (in our experiments $\mathcal{M}^2$ just contains user and item embeddings, but could also include neural layers if required). This is then followed by either simulated annealing or DRR adaptation of the transferred modules. We analyze the training loss curves in \Cref{subsec:convergence} to better understand the fast adaptation of the transferred modules. 

\textbf{Invariant Quality: }A surprising result was the similar performance of \textit{direct layer-transfer} with no adaptation to training all modules on the target state from scratch (\Cref{explicit_meta_results}). The transferred source state modules were directly applicable to the target state embeddings. This helps us validate the generalizability of context-based modules across independently trained state models even with no user or item overlap.

\textbf{Computational Gains: }We also plot the total training times including pretraining for DRR and annealing against the total number of target state interactions in \Cref{scaling-image}. On the target states, module transfer is ~3x faster then training all the modules from scratch. On the whole, there is a significant reduction in the overall training time and computational effort in the \textit{one-to-many} setting. Simulated annealing and DRR adaptation converge in fewer epochs when applied to the pre-trained target model, and outperform the target-trained model by significant margins (\Cref{explicit_meta_results}). These computational gains potentially enable a finer target domain granularity (e.g., adapt to towns or counties rather than states).
\begin{table*}[t]
\centering
\caption{We evaluate recommendation performance on each state (no transfer) with RMSE, MAE metrics for \textit{explicit feedback} against the ground-truth ratings. Metrics were averaged over five runs, $*$ indicates statistical significance (paired \textit{t-test}, p=0.05). On average, models incorporating both pooling and reweighting in \Cref{methods} exhibit significant relative gains (i.e., \textbf{AFM}, \textbf{MMT}).}
\vspace{-11pt}
\begin{tabular}{@{}p{0.06\linewidth}p{0.04\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}p{0.0355\linewidth}@{}}
\toprule
\textbf{Dataset} & \textbf{State} & \multicolumn{2}{c}{\textbf{CAMF}~\cite{camf}} & \multicolumn{2}{c}{\textbf{MTF}~\cite{ctf}} &  \multicolumn{2}{c}{\textbf{NCF}~\cite{ncf}} & \multicolumn{2}{c}{\textbf{NFM}~\cite{nfm}}  & \multicolumn{2}{c}{\textbf{AFM}~\cite{afm}}  & \multicolumn{2}{c}{\textbf{AIN}~\cite{cikm18context}}  & \multicolumn{2}{c}{\textbf{FMT-Net}}  & \multicolumn{2}{c}{\textbf{MMT-Net}} \\ 
\small\textbf{} & \small\textbf{} & \small\textbf{RMS} & \small\textbf{MAE} & \small\textbf{RMS} & \small\textbf{MAE} & \small\textbf{RMS} & \small\textbf{MAE} & \small\textbf{RMS} & \small\textbf{MAE} & \small\textbf{RMS} & \small\textbf{MAE} &\small\textbf{RMS} & \small\textbf{MAE} & \small\textbf{RMS} & \small\textbf{MAE} & \small\textbf{RMS} & \small\textbf{MAE} \\
\midrule
\multirow{4}{*}{\textbf{Yelp}} & \textbf{S} & 1.21 & 0.94 & 1.13 & 0.87 & 1.18 & 1.04 & 1.02 & 0.83 & 0.96 & 0.78 & 0.98 & 0.75 & 1.02 & 0.76 & \textbf{0.94} & \textbf{0.73}\\
\midrule
& $T_1$ & 1.56 & 1.20 & 1.41 & 1.12 & 1.39 & 0.99 &  1.29 & 1.01 & 1.27 & 0.94 & 1.36 & 0.91 & 1.34 &  0.95& \textbf{1.24}* & \textbf{0.88}*\\
& $T_2$ & 1.33 & 1.04 & 1.36 & 0.98 & 1.26 & 1.02 &  1.19 & 1.05 & 1.16 & \textbf{0.90} & 1.17 & 0.95 & 1.15 & 0.98 & \textbf{1.13}* & 0.91\\
& $T_3$ & 1.49 & 1.13 & 1.50 & 1.08 & 1.35 & 1.08 &  1.31 & 0.96 & \textbf{1.20}* & 0.93 & 1.25 & 0.98 & 1.29 & 1.02 & \textbf{1.20}* & \textbf{0.89}*\\
\midrule
 & \textbf{S} & 1.36 & 1.01 & 1.21 & 0.90 & 1.04 & 0.89 & 0.80 & 0.73 & \textbf{0.77} & 0.63 & 0.85 & 0.64 & 0.91 & 0.68 & \textbf{0.77} & \textbf{0.64} \\
\midrule
\multirow{1}{*}{\textbf{Google}} & $T_1$ & 1.49 & 1.20 & 1.38 & 1.14& 1.27 & 1.05 & 1.10 & 0.99 & 0.94 & 0.85 & 1.22 & 0.90 & 1.31 & 0.96 & \textbf{0.89} & \textbf{0.76}* \\
\multirow{1}{*}{\textbf{Local}} & $T_2$ & 1.37 & 1.16 & 1.31 & 1.20& 1.36 & 1.17 & 1.21 & 1.05 &  \textbf{1.14}* & 0.98 & 1.19 & 1.01 & 1.28 & 1.07 & 1.16 & \textbf{0.93}*\\
& $T_3$ & 1.39 & 1.23 & 1.20 & 1.07& 1.19 & 0.98 & 1.13 & 0.92 & 1.09 & 0.91 & 1.08 & 0.94 & 1.14 & 0.98 & \textbf{1.02}* & \textbf{0.85}* \\
\bottomrule
\end{tabular}
\label{explicit_results}
\vspace{-4pt}
\end{table*}
\begin{table*}[b]
\centering
\begin{tabular}{@{}p{0.06\linewidth}p{0.04\linewidth}|p{0.02\linewidth}p{0.02\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.02\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}p{0.0375\linewidth}@{}}
\toprule
\textbf{Dataset} & \textbf{State} & \multicolumn{1}{c}{\textbf{CAMF}} & \multicolumn{1}{c}{\textbf{MTF}} & \multicolumn{2}{c}{\textbf{NCF}~\cite{ncf}} & \multicolumn{2}{c}{\textbf{NFM}~\cite{nfm}}  & \multicolumn{1}{c}{\textbf{AFM}}  & \multicolumn{2}{c}{\textbf{AIN}~\cite{cikm18context}}  & \multicolumn{2}{c}{\textbf{FMT-Net}}  & \multicolumn{2}{c}{\textbf{MMT-Net}} & \multicolumn{2}{c}{\textbf{MMT-m}} \\ 
\textbf{} & \textbf{} & \cite{camf} &\cite{ctf} & \small\textbf{H@1} & \small\textbf{H@5} & \small\textbf{H@1} & \small\textbf{H@5} & \cite{afm} & \small\textbf{H@1} & \small\textbf{H@5} & \small\textbf{H@1} & \small\textbf{H@5} & \small\textbf{H@1} & \small\textbf{H@5} & \small\textbf{H@1} & \small\textbf{H@5}\\
\midrule
\multirow{5}{*}{\textbf{FT-Data}} & \textbf{S} & x & x & 0.42 & 0.77  & 0.52 & 0.91 & x & 0.44 & 0.89 & 0.37 & 0.76 & \textbf{0.56}* & \textbf{0.94} & \textbf{0.56}* & 0.93\\
\midrule
& $T_1$ & x & x & 0.36 & 0.71 & 0.41 & 0.83 & x & 0.34 & 0.76 & 0.32 & 0.75 &  0.45 & 0.84 & \textbf{0.47}* & \textbf{0.86}* \\
& $T_2$  & x & x & 0.25 & 0.64 & 0.30 & 0.77 & x & 0.30 & 0.72 & 0.26 & 0.72 &  \textbf{0.34}* & \textbf{0.79} & \textbf{0.34}* & 0.77 \\
& $T_3$  & x & x & 0.26 & 0.70 & 0.31 & 0.78 & x & 0.29 & 0.74 & 0.28 & 0.74 &  0.33 & \textbf{0.82}* & \textbf{0.34} & 0.80\\
& $T_4$  & x & x & 0.29 & 0.72 & 0.32 & 0.74 & x & 0.32 & 0.78 & 0.21 & 0.69 & 0.37 & 0.80 & \textbf{0.38} & \textbf{0.83}*\\
\bottomrule
\end{tabular}
\caption{We evaluate recommendation performance on each state (no transfer) with the \textit{H@1, 5} metrics for \textit{implicit feedback} in \textit{FT-Data}. Metrics were averaged over five runs, * indicates statistical significance (paired \textit{t-test}, p=0.05). On average, feature-pooling methods AFM, NFM and MMT outperform additive models AIN, FMT. x indicates timed-out or memory limit exceeded.}
\label{implicit_results}
\vspace{-20pt}
\end{table*}
\subsection{Single Domain Recommendation}
\label{subsec:Recommendation}
% Thus, our model is evaluated on its ability to predict the right merchant given the context and to predict the right context given the merchant for each user.
%\begin{table*}[b]
%\centering
%\begin{tabular}{@{}p{0.102\linewidth}p{0.037\linewidth}|p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}|p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}p{0.031\linewidth}@{}}
%\toprule
%\textbf{} & \textbf{} & \multicolumn{7}{c}{\textbf{RMSE Metric}} & \multicolumn{7}{c}{\textbf{MAE Metric}} \\
%\midrule
%\textbf{Dataset} & \textbf{State} & \multicolumn{1}{c}{\textbf{CAMF}} & \multicolumn{1}{c}{\textbf{MTF}} & \multicolumn{1}{c}{\textbf{NFM}}  & \multicolumn{1}{c}{\textbf{AFM}}  & \multicolumn{1}{c}{\textbf{AIN}}  & \multicolumn{1}{c}{\textbf{FMT}}  & \multicolumn{1}{c}{\textbf{MMT}} & \multicolumn{1}{c}{\textbf{CAMF}} & \multicolumn{1}{c}{\textbf{MTF}} & \multicolumn{1}{c}{\textbf{NFM}}  & \multicolumn{1}{c}{\textbf{AFM}}  & \multicolumn{1}{c}{\textbf{AIN}}  & \multicolumn{1}{c}{\textbf{FMT}}  & \multicolumn{1}{c}{\textbf{MMT}} \\ 
%
%%\textit{} & \textit{} & \textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} &\textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} & \textit{RMS} & \textit{MAE} \\
%
%\midrule
%
%\multirow{4}{*}{\textbf{Yelp}} & \textbf{S} & 1.21 & 1.13 & 1.02 & 0.96 & 0.98 & 1.02 & \textbf{0.94} & 0.92 &  0.87 & 0.83 & 0.78 & 0.75& 0.76 & \textbf{0.73}\\
%\midrule
%& $T_1$ & 1.56& 1.41 &  1.29& 1.27& 1.36 & 1.34 & \textbf{1.24} & 1.20  & 1.12  & 1.01  & 0.94  & 0.91  &  0.95 & \textbf{0.88}\\
%& $T_2$ & 1.33 & 1.36 &  1.19 & 1.16 & 1.18 & 1.22 & \textbf{1.13} & 1.04  & 0.98  & 1.05  & \textbf{0.90}  & 0.95  & 0.98  & 0.91\\
%& $T_3$ & 1.49 & 1.50 & 1.31 & \textbf{1.20} & 1.25 & 1.29 & \textbf{1.20} & 1.13 & 1.08 & 0.96 & 0.93 & 0.98 & 1.02 & \textbf{0.89}\\
%
%\midrule
%\multirow{4}{*}{\textbf{Google Local}} & \textbf{S} & 1.36 & 1.21 & 0.80 & 0.77 & 0.85 & 0.91 & \textbf{0.77}&  1.01 & 0.90 & 0.73 & \textbf{0.63} & 0.64 & 0.68 & 0.64 \\
%\midrule
%& $T_1$ & 1.49 & 1.38 & 1.10 & 0.94 & 1.22 & 1.31 &\textbf{ 0.89} & 1.20 & 1.14 & 0.99 & 0.85 &  0.90 &  0.96 &  \textbf{0.76} \\
%& $T_2$ & 1.37 & 1.31 & 1.22 & \textbf{1.14} & 1.19 & 1.28 & 1.16 & 1.16 & 1.20 & 1.05  & 0.98  & 1.01 & 1.07 & \textbf{0.93} \\
%& $T_3$ & 1.39 & 1.23 & 1.20 & 1.07 & 1.13 & 0.92 & 1.09 & 0.91 & 1.08 & 0.94 & 1.14 & 0.98 & \textbf{1.02} & \textbf{0.85} \\
%
%\bottomrule
%\end{tabular}
%\caption{We evaluate the isolated recommendation models on each state with the RMSE, MAE metrics for the \textit{explicit feedback} scenario against ground-truth ratings. Performance values were averaged over five runs, $*$ indicates statistical significance under a paired \textit{t-test} at p=0.05}
%\label{explicit_results}
%\vspace{-18pt}
%\end{table*}
\subsubsection{Comparative Analysis} 
We draw attention to the most relevant features of the baselines and our variants in \Cref{methods}. We highlight our key observations from the experimental results obtained with the baseline recommenders and our FMT-Net and MMT-Net variants (\Cref{implicit_results}, \Cref{explicit_results}). Note that methods with some form of context pooling significantly outperform those without pooled factors, indicating the importance of multi-linear model expressivity to handle interaction context.

We note that AFM performs competitively owing to its ability to reweight terms, similar to our approach (\Cref{explicit_results}), but fails to scale to the larger \textit{FT-Data}. NFM is linear with context size owing to a simple algebraic re-organization, and thus scales to \textit{FT-Data}, however losing the ability to reweight pairwise context product terms \cite{nfm}. Also note the differences between our FMT and MMT variants, demonstrating the importance of the pooled multi-linear formulation for the contextual invariants. These performance differences are more pronounced in the implicit feedback setting (\Cref{implicit_results}). This can be attributed to the greater relevance of transaction context (e.g., transactions provide accurate temporal features while review time is a proxy to the actual visit) and more context features in \textit{FT-Data} vs. Google Local and Yelp (220 vs. 90,120 respectively), magnifying the importance of feature pooling for \textit{FT-Data}.

The lack of pooled feature expressivity in the FMT-Net model impacts the training process as seen in \Cref{pooling-image}, demonstrating the importance of context intersection. The NFM and MMT models converge faster to a smaller Train-RMSE in \Cref{pooling-image} and outperform FMT on the test data (\Cref{implicit_results}, \Cref{explicit_results}). We also observe models incorporating pooled factors to outperform the inherently linear attention-based AIN model, although the performance gap is less pronounced in the smaller review datasets (\Cref{explicit_results}).  We now qualitatively analyze our results to interpret module adaptation.
%\begin{table}[t]
% \centering
% \caption{Statistics for the \textit{dense-source} and \textit{sparse-target} states in each dataset (marked by S and T respectively)}
% \vspace{-10pt}
% \begin{tabular}{@{}p{0.055\linewidth}p{0.165\linewidth}p{0.22\linewidth}p{0.08\linewidth}p{0.115\linewidth}p{0.18\linewidth}@{}}
%  \toprule
%     \textbf{} & \textbf{Bi-Linear Pooling} & \textbf{Multi-Linear Pooling} & \textbf{Low-Rank} & \textbf{Factor Weights} & \textbf{$\mathbf{\Theta}$(Context)}                                                                                                                           \\
%  \midrule
%\textbf{NFM} & Yes & No & No & No & Quadratic*\\
%\textbf{AFM} & Yes & No & No & Yes & Quadratic\\
%\textbf{AIN} & No & No & Yes & Yes & Linear\\
%\textbf{FMT} & No & No & Yes & Yes & Linear\\
%\midrule
%\textbf{MMT} & Yes & Yes & Yes & Yes & Linear\\
%  \bottomrule
% \end{tabular}
% 
% \label{methods}
%\end{table}
%\begin{figure}
%%\hfill
%%\subfigure[Asr-VAE $Recall@50$]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/performance/small_data_avg_perf_perf.pdf}}
%%\hfill
%%\subfigure[\% Gain Asr-VAE vs VAE $R@50$]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/performance/small_data_avg_perf_diff.pdf}}
%%\hfill
%%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}
%%\vspace{-15pt}
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across social link count and item count user quartiles (Q1 = lowest values, Q4 = highest values). Heatmap values are averaged over the smaller datasets (\textit{Ciao}, \textit{Epinions}, \textit{Delicious})}
%%\vspace{-25pt}
%\includegraphics[width=0.89\linewidth]{images/plots/Train-RMSE-multilinear.pdf}
%
%\caption{The Train-RMSE values of models incorporating context pooling converges faster and to a lower Train-RMSE value, indicating their greater expressivity and ability to fit the training data}
%\label{train-convergence}
%\end{figure}
%
%\subsubsection{The Importance of Multi-Linear Expressivity:} 
%\label{none1}
%To further analyze the performance gains achieved by context pooling models, we observe the convergence of the MMT, FMT and NFM recommender models on the source domains of \textit{FT-Data} and the Google Local dataset (\Cref{train-convergence}).
%
%
%
%\begin{figure}
%\includegraphics[width=0.89\linewidth]{images/plots/Train-MMT-context.pdf}
%\label{train-convergence}
%\caption{The Train-RMSE values of MMT trained with and without context bias on the Google Local California source state are nearly identical}
%\end{figure}
%\begin{table}[hbtp]
% \centering
% \caption{MMT-Net performance when trained with and without the context bias term}
% \begin{tabular}{@{}p{0.5\linewidth}p{0.25\linewidth}p{0.24\linewidth}@{}}
%  \toprule
%     \textbf{} & \textbf{Google Local Source} & \textbf{Yelp Source} \\
%  \midrule
%\textbf{RMSE without Context Bias} & 0.91 & 1.12 \\
%\textbf{RMSE with Context Bias} & 0.78 & 1.01 \\
%  \bottomrule
% \end{tabular}
% 
% \label{context-bias-table}
%\end{table}
 
%\begin{table}[hbtp]
% \centering
% \caption{Total MMT-Net training time on Google Local target state Colorado with target-only, and Annealing/DRR with 2 epochs of pre-training. Direct layer-transfer loses 0.1 RMSE points vs target-only with a fifth of the train time.}
% \begin{tabular}{@{}p{0.2\linewidth}p{0.2\linewidth}p{0.21\linewidth}p{0.15\linewidth}p{0.14\linewidth}@{}}
%  \toprule
%     \textbf{} & \textbf{Target-only} & \textbf{Direct-Layer} & \textbf{Anneal} & \textbf{DRR} \\
%  \midrule
%\textbf{Train Time Colorado(s)} & 110 s & \textbf{23} s & 49 s & 41 s \\
%  \bottomrule
% \end{tabular}
% 
% \label{computation-time-targets}
%\end{table}
%We highlight a few key observations:
%
%\begin{itemize}
%\item \textit{Review-Data vs FT-Data} -  The effects of context-pooling are more pronounced in FT-Data. A probable cause is the greater number (220 vs. 90) and quality of contextual features.
%\item \textit{Inconsistency across states} - The size and density of the target datasets are not always correlated to the gains achieved upon transfer. Skew (e.g., few towns vs. one big city) and other data factors play a significant role. For simplicity, we aggregated our target domains by state, although we expect a finer resolution (such as town) to yield better transfer performance.
%\item \textit{Direct Layer-Transfer} - The effectiveness of \textit{direct layer-transfer} is a practical metric for the quality of the inferred contextual invariants.
%\item \textit{Annealing} is a powerful adaptation method, but it produces a separate model for each target domain. It is important to avoid training multiple models, especially when we adopt a finer target granularity, as highlighted in the above observations.
%\end{itemize}
%\subsubsection{Transferability for Non Multi-Linear Formulations}
%
%In this subsection, we attempt to identify the advantages of employing multi-linear pooled context as the building blocks of our meta learner, and the impact of employing alternate formulations on the transferability of learned representations.
%
%\textbf{* Experiments to benchmark the FMT model for meta-transfer on the two public datasets underway}
\subsection{Qualitative Analysis}
\label{subsec:Qualitative}
We analyze our approach from the shared module training and convergence perspective for the different adaptation methods. We observe consistent trends across the direct layer-transfer, annealing, and DRR adaptation approaches. 
\subsubsection{Training without Context-Bias} To understand the importance of decorrelating training samples in the training process, we repeat the performance analysis on our MMT-Net model with and without the adaptive context-bias term in the training objective in \Cref{subsec:Train}. We observe a 15\% performance drop across the Yelp and Google Local datasets, although this does not reflect in the Train-RMSE convergence (\Cref{train-convergence-context}) of the two variations. In the absence of context-bias, the model overfits uninformative transactions to the user and item bias terms ($s_{u}$, $s_{v}$) in \Cref{explicit_rating}, \Cref{explicit_loss}  and thus achieves comparable Train-RMSE values. However, the overfit user and item terms are not generalizable, resulting in the observed drop in test performance.
\begin{figure}[t]
\vspace{-10pt}
%\hfill
\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.78\linewidth]{images/plots/Train-MMT-context.pdf}
%\hfill
%\subfigure[MMT-Net convergence with and without context-bias]{\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.49\linewidth]{images/plots/Train-MMT-context.pdf}}
%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}%
\vspace{-12pt}
\caption{MMT-Net trained with \& without context-bias (\Cref{eq:context_bias}) on the Google Local source exhibits similar Train-RMSE, but registers $>10\%$ drop in test performance.}
\vspace{-14pt}
\label{train-convergence-context}
\end{figure}
\subsubsection{Model Training and Convergence Analysis}
\label{subsec:convergence}
%We highlight a few consistent observations across datasets and target domains:
%\begin{itemize}
We compare the Train-RMSE convergence for the MMT-Net model fitted from scratch to the Google Local target state, Colorado ($\mathbf{T}_1$) vs. the training curve under DRR and annealing adaptation with two pretraining epochs on the target state in \Cref{fig:convergence}. Clearly, the target-trained model takes significantly longer to converge to a stable Train-RMSE in comparison to the Anneal and DRR adaptation. Although the final Train-RMSE is comparable (\Cref{scaling-image}), there is a significant performance difference between the two approaches on the test dataset, as observed in \Cref{explicit_meta_results}. Training loss convergence alone is not indicative of the final model performance; the target-only training method observes lower Train-RMSE by overfitting to the sparse data. We also compare the Train-RMSE convergence for target-trained models with and without pooled context factors (MMT-Net, NFM vs. FMT-Net) in \Cref{pooling-image}. We observe the NFM, MMT-Net models to converge faster to a better optimization minima than FMT-Net. This also reflects in their test performance in \Cref{implicit_results}.
\begin{figure}[b]
\vspace{-4pt}
%\hfill
\includegraphics[clip, trim=0cm 0cm 0cm 0.7cm, width=0.78\linewidth]{images/plots/Google-Local-CO.pdf}
%\hfill
%\subfigure[MMT-Net convergence with and without context-bias]{\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.49\linewidth]{images/plots/Train-MMT-context.pdf}}
%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}%
\vspace{-12pt}
\caption{MMT-Net convergence under target-training vs. Annealing/DRR adaptation after 2 epochs of pretraining on the Google Local Colorado target}
\vspace{-12pt}
\label{fig:convergence}
\end{figure}
\begin{figure}[b]
\vspace{-2pt}
%\hfill
\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.78\linewidth]{images/plots/Train-RMSE-multilinear.pdf}
%\hfill
%\subfigure[MMT-Net convergence with and without context-bias]{\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.49\linewidth]{images/plots/Train-MMT-context.pdf}}
%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}%
\vspace{-12pt}
\caption{MMT-Net convergence compared to NFM and FMT-Net on the Google Local Colorado target}
%\vspace{-25pt}
\label{pooling-image}
\end{figure}
\begin{figure}[t]
\vspace{-10pt}
%\hfill
\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.78\linewidth]{images/plots/scalability-numbers.pdf}
%\hfill
%\subfigure[MMT-Net convergence with and without context-bias]{\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.49\linewidth]{images/plots/Train-MMT-context.pdf}}
%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}%
\vspace{-12pt}
\caption{MMT-Net training duration with and without module transfer vs. target domain interaction volume}
\vspace{-14pt}
\label{scaling-image}
\end{figure}
%\item Direct layer-transfer is an alternative to the target-trained model (\Cref{explicit_meta_results}), principally entailing one-fifth the training cost (2 pre-training epochs vs. ten target-only epochs). Its performance indicates the generalizability of the contextual invariants learned on the source dataset and cross-domain \textit{dimensional-uniformity} of the learned embeddings.
%
%\item DRR is a strong alternative to the Annealing approach, although there is a small performance gap on most target states (\Cref{explicit_meta_results}). The primary advantage of DRR is the need to store a small number (in our case 3) of strategically placed residual layers for each target region, while the source model is left unchanged. DRR could also be investigated towards temporal updates to the source model for evolving user preferences; we leave this analysis for future work.
%\end{itemize}
%\begin{figure}
%\includegraphics[width=0.89\linewidth]{images/plots/volume-density-heatmap.pdf}
%\vspace{-15pt}
%\caption{Demonstrates the relative improvement in the \textbf{H@1} performance (0.32 = 32\%) across different Volume-Density subsets of the Arkansas target state in the \textit{FT-Data}}
%\vspace{-19pt}
%\label{volume-density-heatmap}
%\end{figure} 
%\begin{figure}[t]
%\vspace{-10pt}
%\hfill
%\subfigure[MMT-Net Convergence]{\includegraphics[clip, trim=0cm 0cm 0cm 0.7cm, width=0.49\linewidth]{images/plots/Google-Local-CO.pdf}}
%\hfill
%\subfigure[MMT-Net Training Duration]{\includegraphics[clip, trim=0cm 0cm 0cm 0.7cm, width=0.49\linewidth]{images/plots/scalability-numbers.pdf}}
%%\hfill
%%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}%
%\vspace{-12pt}
%\caption{MMT-Net convergence under Target-Training, and Anneal/DRR after 2 epochs of pre-training (Google Local Colorado), and their training durations against number of interactions. We achieve both performance and scalability gains over the target-trained model.}
%%\vspace{-25pt}
%\label{scaling-image}
%\end{figure}
%\begin{figure}[b]
%\vspace{-10pt}
%\hfill
%\subfigure[NFM, MMT-Net, FMT-Net convergence, Google Local California]{\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.49\linewidth]{images/plots/Train-RMSE-multilinear.pdf}}
%\hfill
%\subfigure[MMT-Net convergence with and without context-bias]{\includegraphics[clip, trim=0cm 0cm 0cm 1cm, width=0.49\linewidth]{images/plots/Train-MMT-context.pdf}}
%%\hfill
%%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}%
%\vspace{-12pt}
%\caption{Context pooling models NFM, MMT-Net converge faster to a lower Train-RMSE vs FMT-Net, indicating greater expressivity to fit the training data. MMT-Net trained with \& without context-bias exhibits similar Train-RMSE, but registers $>10\%$ drop in test performance.}
%%\vspace{-25pt}
%\label{train-convergence}
%\end{figure}
%\begin{figure}[b]
%\vspace{-10pt}
%\hfill
%\subfigure{\includegraphics[clip, trim=7.5cm 5cm 7.5cm 6cm, width=0.49\linewidth]{images/plots/CA-TSNE.pdf}}
%\hfill
%\subfigure{\includegraphics[clip, trim=7.5cm 5cm 7.5cm 6cm, width=0.49\linewidth]{images/plots/CA-CO-TSNE.pdf}}
%%\hfill
%%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}%
%\vspace{-12pt}
%\caption{2D TSNE Visualizations of the transformed user embeddings, Google Local California source (Left) and Colorado sparse target after meta-transfer via DRR (Right)}
%%\vspace{-25pt}
%\label{emb-TSNE}
%\end{figure}
%\begin{figure}
%\includegraphics[width=0.89\linewidth]{images/plots/CA-TSNE.pdf}
%
%\caption{2D TSNE Visualizations of Google Local California (source state) user embedding space}
%\label{CA-emb-TSNE}
%\end{figure}
%
%\begin{figure}
%\includegraphics[width=0.89\linewidth]{images/plots/CA-CO-TSNE.pdf}
%
%\caption{2D TSNE Visualizations of Google Local, Colorado (Target) user embedding space after Meta Transfer via DRR}
%\label{CA-CO-emb-TSNE}
%\end{figure}
%\subsubsection{The Volume-Density Perspective}
%\label{subsec:volume-density}
%In this section, we attempt to identify the sub-populations of users who benefit the most from meta transfer. Towards this goal, we vary two key parameters - Volume (total number of interactions) and density (interactions per user) in the training set and fit models to each training set separately. We then meta transfer the source model to each of these training sets and observe the gains achieved over the respective target-trained model. 
%
%We first split all users into four density quartiles based on their interaction quartiles. The collection of users in the highest density quartile would then constitute a very dense subset. To vary the interaction volume in each density quartile, we remove varying proportions of sparse or dense users from within the quartile, thus controlling for the total interaction volume. We then fit models separately to these modified training sets and observe the gains achieved with meta-transfer from the source domain. We demonstrate results on the largest target state in \textit{FT-data}, Arkansas (\Cref{volume-density-heatmap}).
%
%Our observation indicates strong gains in the lower-half and left-half of the heatmap (low-density, low-volume). Sparse users and small domains are best served by the generalizable context transforms learned on the large and dense source domain, where there is sufficient training data to infer the most important context factor associations with our overall modular formulation.
%% \textbf{Similar heatmaps will be added for the \textit{FT-Data} and \textit{Yelp} datasets as well.}
%
%
%
%\subsubsection{Embedding Visualization}
%
%Our Distributionally Regularized Residual (DRR) strategy ensures structural consistency in the transformed user and item embedding spaces of the target domain, thus enabling us to apply the source-learned modules to the target domain. To validate this hypothesis, we inspect the user embedding structure across the Source (California) and the largest target domain (Colorado) in the Google Local Dataset, after applying the DRR strategy for adaptation in \Cref{emb-TSNE}. The California user embedding space has a distinct spiral cluster structure, with multiple locally dense regions. We observe a very similar structure in the transformed Colorado user embedding space after DRR adaptation with the source-learned meta-modules. Each space is represented via 2-dimensional TSNE visualizations \cite{tsne} in \Cref{emb-TSNE}.
\subsection{Scalability and Robustness Analysis}
\label{subsec:Scale-Robust}
We demonstrate the scalability of meta-transfer with the number of transactions in the target domain in \Cref{scaling-image} against training separate models. Our previous observations in \Cref{subsec:Meta-Transfer-Exp} validate the ability of our approach to scale deeper architectures to a large number of target domains while also enabling a finer resolution for the selection of target domains. Towards tackling incomplete data, we also evaluated the robustness of the shared context layers by randomly dropping up to 20\% of the context features in each interaction at train and test time for both, the source and target states in \Cref{table-context-drop}. 
%\begin{figure}
%\includegraphics[width=0.69\linewidth]{images/plots/scalability-numbers.pdf}
%
%\caption{Training time for the Target-Only, Anneal and DRR approaches against Millions of Interactions (with user interaction density of 10)}
%\label{scaling-image}
%\end{figure}
\begin{table}[hbtp]
 \centering
 \vspace{-8pt}
 \caption{MMT-Net performance degradation was measured by the decrease in \textbf{H@1} or increase in \textbf{RMSE}, averaged over target states with random context feature dropout}
 \vspace{-11pt}
 \begin{tabular}{@{}p{0.25\linewidth}p{0.17\linewidth}p{0.16\linewidth}p{0.16\linewidth}p{0.16\linewidth}@{}}
  \toprule
     \textbf{Context Drop} & \textbf{5\%} & \textbf{10\%} & \textbf{15\%} & \textbf{20\%} \\
  \midrule
\textbf{FT-Data} & 1.1\% & 2.6\% & 4.1\% & 6.0\% \\
\textbf{Google Local} & 3.9\% & 4.2\% & 7.0\% & 8.8\% \\
\textbf{Yelp} & 1.8\% & 3.2\% & 5.4\% & 7.3\% \\
  \bottomrule
 \end{tabular}
 \label{table-context-drop}
  \vspace{-18pt}
 \end{table}
% (\Cref{}). These results support the generalizability and scalability of our approach to recommendation applications.
\subsection{Limitations and Discussion}
\label{subsec:Limitations}
%
We identify a few fundamental limitations of our model. While our approach presents a scalable and effective solution to bridge the weaknesses of gradient-based meta learning and co-clustering via user or item overlaps, contextual invariants do not extend to cold-start users or items. Second, our model does not trivially extend to the case where a significant number of users or items are shared across recommendation domains. We separate the embeddings and $\textit{learn-to-learn}$ aspect which improves modularity, but prevents direct reuse of representations across domains, since only the transformation layers are shared. Depending on the application, context features could potentially be filtered to enhance social inference and prevent loss of diversity in the generated recommendations.
%We tested our framework by incorporating \textbf{DAE}, \textbf{VAE-CF} and \textbf{LRML} as generators $\mathbf{G}$ in our framework. We refer to these variants as \textbf{Asr-DAE}, \textbf{Asr-VAE} and \textbf{Asr-LRML} (\textbf{Asr} denotes adversarial social regularization). Experiments were performed on a Nvidia Tesla V100 GPU with \textit{TensorFlow} implementations on the Linux platform. Our implementations will be made publicly available\footnote{\url{https://github.com/CrowdDynamicsLab/Adversarial-Social-Recommendation}}.
%
%\subsection{Recommendation}
%\label{subsec:Recommendation}
%% latex weirdness with two column floats
%
%\begin{table*}
%  \robustify\bfseries
%  \small
%  \centering
%  \begin{threeparttable}
%  \begin{tabular}{@{}
%                      cS@{\hspace{0.1mm}}S@{\hspace{0.1mm}}S@{\hspace{0.1mm}}S
%                      S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S
%                      S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S
%                      S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S
%                      S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S@{\hspace{-0.1mm}}S
%                      @{}}
%  
%%  {c|S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S@{\hspace{1.75mm}}S[round-mode=places,round-precision=2]@{\hspace{-0.8mm}}S}
%
%    \toprule
%    \multirow{3}{*}{\textbf{Method}} &
%     \multicolumn{12}{c}{\underline{Smaller Datasets}} &
%     \multicolumn{8}{|c}{\underline{Larger Datasets}}\\
%      
%      & \multicolumn{4}{c}{\textbf{Epinions}} &
%      \multicolumn{4}{c}{\textbf{Ciao}} &
%      \multicolumn{4}{c}{\textbf{Delicious}} &
%      \multicolumn{4}{|c}{\textbf{Ask-Ubuntu}} &
%      \multicolumn{4}{c}{\textbf{Yelp}}\\
%      
%%      & {\textbf{R@20}\hspace{0.9mm}} & {\textbf{N@20}\hspace{0.9mm}} & {\textbf{R@50}\hspace{0.9mm}} & {\textbf{N@50}\hspace{0.9mm}} &
%%      {\textbf{R@20}\hspace{0.9mm}} & {\textbf{N@20}\hspace{0.9mm}} & {\textbf{R@50}\hspace{0.9mm}} & {\textbf{N@50}\hspace{0.9mm}} &
%%      {\textbf{R@20}\hspace{0.9mm}} & {\textbf{N@20}\hspace{0.9mm}} & {\textbf{R@50}\hspace{0.9mm}} & {\textbf{N@50}\hspace{0.9mm}} &
%%      \multicolumn{1}{|c}{\textbf{R@20}\hspace{0.9mm}} & {\textbf{N@20}\hspace{0.9mm}} & {\textbf{R@50}\hspace{0.9mm}} & {\textbf{N@50}\hspace{0.9mm}} &
%%      {\textbf{R@20}\hspace{0.9mm}} & {\textbf{N@20}\hspace{0.9mm}} & {\textbf{R@50}\hspace{0.9mm}} & {\textbf{N@50}\hspace{0.9mm}}  \\ 
%
%%    & {\textit{R@20}\hspace{0.9mm}} & {\textit{N@20}\hspace{0.9mm}} & {\textit{R@50}\hspace{0.9mm}} & {\textit{N@50}\hspace{0.9mm}} &
%%      {\textit{R@20}\hspace{0.9mm}} & {\textit{N@20}\hspace{0.9mm}} & {\textit{R@50}\hspace{0.9mm}} & {\textit{N@50}\hspace{0.9mm}} &
%%      {\textit{R@20}\hspace{0.9mm}} & {\textit{N@20}\hspace{0.9mm}} & {\textit{R@50}\hspace{0.9mm}} & {\textit{N@50}\hspace{0.9mm}} &
%%      \multicolumn{1}{|c}{\textit{R@20}\hspace{0.9mm}} & {\textit{N@20}\hspace{0.9mm}} & {\textit{R@50}\hspace{0.9mm}} & {\textit{N@50}\hspace{0.9mm}} &
%%      {\textit{R@20}\hspace{0.9mm}} & {\textit{N@20}\hspace{0.9mm}} & {\textit{R@50}\hspace{0.9mm}} & {\textit{N@50}\hspace{0.9mm}}  \\ 
%      
%%      & {\text{R@20}\hspace{0.9mm}} & {\text{N@20}\hspace{0.9mm}} & {\text{R@50}\hspace{0.9mm}} & {\text{N@50}\hspace{0.9mm}} &
%%      {\text{R@20}\hspace{0.9mm}} & {\text{N@20}\hspace{0.9mm}} & {\text{R@50}\hspace{0.9mm}} & {\text{N@50}\hspace{0.9mm}} &
%%      {\text{R@20}\hspace{0.9mm}} & {\text{N@20}\hspace{0.9mm}} & {\text{R@50}\hspace{0.9mm}} & {\text{N@50}\hspace{0.9mm}} &
%%      \multicolumn{1}{|c}{\hspace{0.65mm}\text{R@20}\hspace{0.25mm}} & {\text{N@20}\hspace{0.9mm}} & {\text{R@50}\hspace{0.9mm}} & {\text{N@50}\hspace{0.9mm}} &
%%      {\text{R@20}\hspace{0.9mm}} & {\text{N@20}\hspace{0.9mm}} & {\text{R@50}\hspace{0.9mm}} & {\text{N@50}\hspace{0.9mm}}  \\ 
%
%
%& {\textit{R@20}\hspace{0.82mm}} & {\textit{N@20}\hspace{0.82mm}} & {\textit{R@50}\hspace{0.82mm}} & {\textit{N@50}\hspace{0.82mm}} &
%      {\textit{R@20}\hspace{0.82mm}} & {\textit{N@20}\hspace{0.82mm}} & {\textit{R@50}\hspace{0.82mm}} & {\textit{N@50}\hspace{0.82mm}} &
%      {\textit{R@20}\hspace{0.82mm}} & {\textit{N@20}\hspace{0.82mm}} & {\textit{R@50}\hspace{0.82mm}} & {\textit{N@50}\hspace{0.82mm}} &
%      \multicolumn{1}{|c}{\hspace{0.65mm}\textit{R@20}\hspace{0.25mm}} & {\textit{N@20}\hspace{0.82mm}} & {\textit{R@50}\hspace{0.82mm}} & {\textit{N@50}\hspace{0.82mm}} &
%      {\textit{R@20}\hspace{0.82mm}} & {\textit{N@20}\hspace{0.82mm}} & {\textit{R@50}\hspace{0.82mm}} & {\textit{N@50}\hspace{0.82mm}}  \\ 
%      
%    \midrule      
%      
%      & \multicolumn{20}{c}{\textbf{Social-Agnostic Recommenders}} \\
%      
%    \midrule      
%      
%      \textbf{BPR~\cite{bpr}} & 
%      0.264 & 0.141 & 0.440 & 0.176 &
%    0.232 & 0.128 & 0.428 & 0.162 &
%    0.363 & 0.271 & 0.590 & 0.328 &
%    0.377 & 0.199 & 0.514 & 0.264 &
%    0.228 & 0.125 & 0.431 & 0.170 \\
%      
%    
%    \textbf{NCF~\cite{ncf}} & 
%      0.310 & 0.138 & 0.462 & 0.181 &
%    0.282 & 0.147 & 0.471 & 0.193 &
%    0.498 & 0.283 & 0.753 & 0.401 &
%    0.420 & 0.215 & 0.538 & 0.281 &
%    0.196 & 0.118 & 0.488 & 0.209 \\    
%
%
%    \textbf{DAE~\cite{dae}} & 
%      0.324 & 0.164 & 0.498 & 0.198 &
%    0.290 & 0.143 & 0.493 & 0.191 &
%    0.572 & 0.340 & 0.762 & 0.393 &
%    0.416 & 0.301 & 0.569 & 0.392 &
%    0.270 & 0.158 & 0.473 & 0.213 \\    
%    
%    
%    \textbf{VAE-CF~\cite{vaecf}} & 
%      0.336 & 0.161 & 0.510 & 0.204 &
%    0.299 & 0.152 & 0.496 & 0.197 &
%    0.585 & 0.327 & 0.771 & 0.416 &
%    0.408 & 0.317 & 0.576 & 0.383 &
%    0.281 & 0.164 & 0.479 & 0.208 \\    
%
%
%    \textbf{LRML~\cite{lrml}} & 
%      0.329 & \hspace{1.5mm}\underline{0.173} & 0.509 & \hspace{1.5mm}\underline{0.219} &
%    0.317 & \hspace{1.3mm}\textbf{0.165} & 0.526 & 0.206 &
%    0.482 & 0.310 & 0.698 & 0.384 &
%    0.405 & 0.366 & 0.564 & 0.405 &
%    0.272 & 0.160 & 0.483 & 0.196 \\    
%    
%    \midrule
%     & \multicolumn{20}{c}{\textbf{Social Recommenders}} \\
%    \midrule
%    
%    
%    
%    \textbf{SBPR~\cite{sbpr}} & 
%      0.271 & 0.138 & 0.446 & 0.185 &
%    0.217 & 0.140 & 0.439 & 0.174 &
%    0.381 & 0.292 & 0.625 & 0.362 &
%    0.368 & 0.206 & 0.528 & 0.287 &
%    0.230 & 0.143 & 0.449 & 0.196 \\
%    
%    
%    \textbf{SNCF} & 
%      0.306 & 0.189 & 0.468 & 0.202 &
%    0.284 & 0.151 & 0.478 & 0.196 &
%    0.520 & 0.296 & 0.747 & 0.380&
%    0.414 & 0.371 & 0.541 & 0.403 &
%    0.198 & 0.103 & 0.493 & 0.202 \\
%    
%    
%    \textbf{SGCN~\cite{sgcn}} & 
%      0.318 & 0.153 & 0.481 & 0.198 &
%    0.275 & 0.142 & 0.470 & 0.179 &
%    0.546 & 0.295 & 0.718 & 0.401 &
%    0.397 & 0.343 & 0.526 & 0.395 &
%    0.288 & 0.160 & 0.492 & 0.176 \\
%      
%     \textbf{CB~\cite{cb}} & 
%      0.337 & 0.171 & 0.436 & 0.202 &
%    0.288 & 0.153 & 0.491 & 0.180 &
%    0.572 & 0.287 & 0.753 & 0.384 &
%    0.399 & 0.365 & 0.559 & 0.382 &
%    0.282 & 0.154 & 0.471 & 0.196 \\   
%    
%    \textbf{SEREC~\cite{serec}} & 
%      0.348 & 0.167 & 0.496 & \hspace{1.5mm}\underline{0.213} &
%    0.303 & 0.158 & 0.513 & 0.202 &
%    0.589 & 0.314 & 0.762 & 0.398 &
%    0.415 & 0.362 & 0.584 & 0.414 &
%    \hspace{1.3mm}\underline{0.306} &\hspace{1.6mm}\underline{0.173} & \hspace{1.5mm}\textbf{0.508} & 0.211 \\
%    
%    
%    \midrule
%     & \multicolumn{20}{c}{\textbf{Adversarial Social Recommenders (Ours)}} \\
%    \midrule
%    
%    
%    \textbf{Asr-DAE} & 
%      0.339 & \hspace{1.3mm}\underline{0.168} & 0.513 & 0.207 &
%    0.301 & 0.144 & 0.519 & 0.189 &
%    0.603 & 0.322 & 0.784 & 0.418 &
%    \hspace{2.7mm}\underline{0.434} & 0.347 & \hspace{1.3mm}\underline{0.585} & 0.412 &
%    0.272 & 0.158 & 0.489 & 0.201 \\
%    
%    \textbf{Asr-VAE} & 
%      \hspace{1.3mm}\textbf{0.358} & \hspace{1.3mm}\underline{0.173} & \hspace{1.3mm}\underline{0.532} & \hspace{1.3mm}\underline{0.216} &
%    0.312 & 0.138 & 0.528 & 0.196 &
%    \hspace{1.3mm}\textbf{0.617} & \hspace{1.3mm}\textbf{0.379} & \hspace{1.3mm}\textbf{0.797} & \hspace{1.3mm}\textbf{0.442} &
%    \hspace{2.7mm}\underline{0.431} & 0.350 & \hspace{1.3mm}\underline{0.592} & 0.401 &
%    \hspace{1.3mm}\underline{0.298} & 0.161 & 0.496 & 0.218 \\
%    
%    \textbf{Asr-LRML} & 
%      0.340 & 0.166 & \hspace{1.3mm}\underline{0.527} & \hspace{1.3mm}\underline{0.220} &
%    \hspace{1.3mm}\textbf{0.328} & 0.160 & \hspace{1.3mm}\textbf{0.544} & \hspace{1.3mm}\textbf{0.214} &
%    0.495 & 0.357 & 0.743 & 0.426 &
%    \hspace{2.7mm}0.411 & \hspace{1.3mm}\textbf{0.375} & 0.578 & \hspace{1.3mm}\textbf{0.419} &
%    0.287 & \hspace{1.6mm}\underline{0.172} & 0.481 & \hspace{1.3mm}\textbf{0.233} \\
%    
%%      \cmidrule(lr){1-1}\cmidrule(lr){2-11}\cmidrule(lr){12-21}
%%    RF~\cite{BurelMA16, TianZL13} & 70.91 & 0.7035 & 72.83 & 0.6832 & 75.04 & 0.5066 & 70.33 & 0.6284 & 69.27 & 0.5798 & 63.74 & 0.7165 & 65.05 & 0.7013 & 70.90 & 0.5965 & 63.13 & 0.7290 & 64.63 & 0.6674\\
%%    FF~\cite{JendersKN16} & 72.75 & 0.8243 & 72.69 & 0.8061 & 76.97 & 0.7167 & 76.07 & 0.7729 & 73.66 & 0.7468 & 65.93 & 0.8018 & 68.18 & 0.8030 & 73.14 & 0.7299 & 68.09 & 0.8014 & 68.49 & 0.7891\\
%%    %biLSTM & 63.84 & 0.6887 & 64.40 & 0.6772 & 70.65 & 0.5679 & 58.27 & 0.6944 & 58.10 & 0.6939 & 64.31 & 0.5869 \\
%%    %biLSTM+CNN & 67.86 & 0.7115 & 68.95 & 0.7009 & 73.08 & 0.6253 & 61.15 & 0.7050 & 59.15 & 0.7279 & 66.75 & 0.5997 \\
%%    DGCN~\cite{DualGCN} & 77.62 & 0.8389 & 76.73 & 0.8098 & 76.79 & 0.7480 & 76.81 & 0.7853 & 75.78 & 0.7522 & 71.14 & 0.8102 & 70.32 & 0.8056 & 75.16 & 0.7487 & 71.34 & 0.8087 & 70.25 & 0.7944\\
%%    RGCN~\cite{relationalGCN} & 61.97 & 0.6490 & 63.21 & 0.6612 & 62.97 & 0.5782 & 53.95 & 0.6135 & 56.12 & 0.6235 & 60.86 & 0.6960 & 64.60 & 0.6906 & 64.14 & 0.6104 & 51.00 & 0.7035 & 55.24& 0.6358\\
%%    \cmidrule(lr){1-1}\cmidrule(lr){2-11}\cmidrule(lr){12-21}
%%    AS-GCN & 74.02 & 0.8359 & 74.14 & 0.8051 & 78.56 & 0.7198 & 76.62 & 0.7902 & 74.60 & 0.7512 & 66.91 & 0.7907 & 68.95 & 0.7953 & 74.90 & 0.7494 & 69.63 & 0.7998 & 70.15 & 0.7737\\
%%    TS-GCN & 72.40 & 0.8308 & 74.08 & 0.7913 & 77.96 & 0.7044 & 76.96 & 0.7842 & 74.19 & 0.7267 & 65.67 & 0.7894 & 68.46 & 0.7985 & 73.95 & 0.7484 & 69.11 & 0.8048 & 69.49 & 0.7818\\
%%    C-GCN & 78.25 & 0.8433 & 76.90 & 0.8154 & 78.91 & 0.7513 & 77.23 & 0.7940 & 76.88 & 0.7574 & 69.48 & 0.8107 & 72.70 & 0.8103 & 76.44 & 0.7609 & 73.09 & 0.8123 & 72.27 & 0.7921\\
%%    B-IR-GCN & \bfseries 80.27 & \bfseries 0.8495 & \bfseries 80.22 & \bfseries 0.8206 & \bfseries 81.61 & \bfseries 0.7710 & \bfseries 79.39 & \bfseries 0.8075 & \bfseries 78.26 & \bfseries 0.7697 & \bfseries 72.4& \bfseries 0.8160 & \bfseries 74.61 & \bfseries 0.8241 & \bfseries 78.75 & \bfseries 0.7654 & \bfseries 74.29 & \bfseries 0.8205 & \bfseries 75.25 & \bfseries 0.7976\\
%    \bottomrule
%  \end{tabular}
%  \begin{tablenotes}
%    \footnotesize
%    \item[*] The Asr variants denote the DAE, VAE-CF and LRML base models integrated as the generator in our adversarial framework. Our model can substitute recommender (generator) and discriminator architectures owing to the modular formulation. The performance numbers in bold numerals indicate statistically significant gains over the second best model at $p =0.05$. When there are two or more strong performers under a specific metric, we underline them. Our adversarial variants exhibit strong gains over competing social recommenders as well as their respective base models.
%  \end{tablenotes}
%  %\subcaption{Non-Tech StackExchanges}
%%  \bigskip
%%  \begin{subtable}{1\textwidth}
%%    \centering
%%  \begin{tabular}{lS[round-mode=places,round-precision=2]SS[round-mode=places,round-precision=2]SS[round-mode=places,round-precision=2]SS[round-mode=places,round-precision=2]SS[round-mode=places,round-precision=2]S}
%%    \toprule
%%    \multirow{2}{*}{Method} &
%%      \multicolumn{2}{c}{arduino} &
%%      \multicolumn{2}{c}{bitcoin} &
%%      \multicolumn{2}{c}{unix} &
%%      \multicolumn{2}{c}{cypto} &
%%      \multicolumn{2}{c}{askUbuntu} \\
%%      & {Acc (\%)} & {MRR} & {Acc(\%)} & {MRR} & {Acc(\%)} & {MRR} & {Acc(\%)} & {MRR} & {Acc(\%)} & {MRR} \\
%%      \midrule
%%    RF & 63.74 & 0.7165 & 65.05 & 0.7013 & 70.90 & 0.5965 & 63.13 & 0.7290 & 64.63 & 0.6674\\
%%    MLP & 65.93 & 0.8018 & 68.18 & 0.8030 & 73.14 & 0.7299 & 68.09 & 0.8014 & 68.49 & 0.7891\\
%%    DGCN & 71.14 & 0.8102 & 70.32 & 0.8056 & 75.16 & 0.7487 & 71.34 & 0.8087 & 70.25 & 0.7944\\
%%    RGCN & 60.86 & 0.6960 & 64.60 & 0.6906 & 64.14 & 0.6104 & 51.00 & 0.7035 & 55.24& 0.6358\\
%%    \hline
%%    AS-GCN & 66.91 & 0.7907 & 68.95 & 0.7953 & 74.90 & 0.7494 & 69.63 & 0.7998 & 70.15 & 0.7737\\
%%    TS-GCN & 65.67 & 0.7894 & 68.46 & 0.7985 & 73.95 & 0.7484 & 69.11 & 0.8048 & 69.49 & 0.7818\\
%%    C-GCN & 69.48 & 0.8107 & 72.70 & 0.8103 & 76.44 & 0.7609 & 73.09 & 0.8123 & 72.27 & 0.7921\\
%%    B-IRGCN & 72.4& 0.8160 & 74.61 & 0.8241 & 78.75 & 0.7654 & 74.29 & 0.8205 & 75.25 & 0.7976\\
%%    \bottomrule
%%  \end{tabular}
%%    \subcaption{Tech StackExchanges}
%%\end{subtable}
%        %\subcaption{}
%  \caption{\small \label{tab:mainresults} $R@K$ and $N@K$ denote the Recall and NDCG metrics for all models. Our models outperform competing baselines by upto 35\% Recall@50 and 25\% NDCG@50. Asr-VAE was found to be the best overall model.}
%  \end{threeparttable}
%\vspace{-0.2in}
%\end{table*}
%
%
%To evaluate the performance of the recommender models listed above, we compute the $NDCG@K$ (\emph{N@K}) and $Recall@K$ (\emph{R@K}) metrics \cite{metric@k}. $Recall@K$ is a measure of the percentage of relevant items in the top-$K$ recommendations to each user; it considers true and false positives in the list and is thus more descriptive than Precision. The $NDCG@K$ metric is position sensitive and considers the order of the ranked list against the ideal case (only relevant items placed at the top). We evaluate each ranked list at $K=20,50$ (\Cref{tab:mainresults}).
%
%We randomly split each dataset into Training (80\%), Validation (10\%) and Test (10\%). We tune the baselines with parameter ranges centered at the author provided values, to obtain the best performance on our datasets. For fair comparison, we set the representation dimensions to $128$ for all models. For our model, adversary weight $\lambda$, balance $\mu$ were both tuned in the range $(0, 10]$ and we set Hadamard projectors $N=10$ across all experiments.
%
%\textbf{Comparative Analysis :} We make several observations from the experimental results obtained with the baseline recommenders and our adversarial variants (\Cref{tab:mainresults}). First, conventional social recommenders are outperformed by social-agnostic neural methods that efficiently leverage the rating information. Non-linear transformations of ineterest representations are more expressive than linear or bi-linear operations \cite{ncf}.
%
%Second, expressive interest spaces (like in \textbf{DAE}~\cite{dae}) benefit more from social regularization than conventional interest representations. The gains achieved by integrating neural models in our framework are stronger than those adding social information to older methods (e.g., \emph{R@50} gains of \textbf{SBPR} vs \textbf{BPR} are smaller on average than those of \textbf{Asr-VAE} vs \textbf{VAE}). Also, note that a direct integration of pre-trained embeddings (as in \textbf{SNCF}) does not produce a noticeable gain in performance. Pre-trained graph embeddings cannot contextually distinguish the influence of a user's neighbors by their interests. 
%
%We find our adversarial variants and \textbf{SEREC} to outperform older social recommender baselines by significant margins. While \textbf{SEREC} permits for the exposed item set to be prioritized differently, \textbf{CB}~\cite{cb}  flexibly attributes puchases, however picking a single factor (interest vs social) instead of a contextual combination.  \textbf{Asr-VAE} was found to achieve the best overall performance. The \textbf{VAE} user representations are inherently stochastic unlike \textbf{DAE} and \textbf{LRML}, we also observed greater recommendation diversity (less interest space collapse) with \textbf{Asr-VAE} (\Cref{subsec:Model Robustness and Mode-Collapse}).
%
%
%\textbf{Neighbor Diversity: } Unlike exposure models, we condition each item on the specific social context i.e., a phone exposed by an android expert has a greater effect than from other social contacts. To verify this, we measure the diversity of each user's friends. As an example, if a user's four friends have 5, 10, 15, and 20 items, their item distribution is $({5}/{50}, {10}/{50}, {15}/{50}, {20}/{50})$. We estimate the KL-divergence of this distribution against the uniform case to measure diversity. We then split all users into four quartiles based on their neighbor diversity (Q4 has users with high neighbor diversity), and compare \textit{R@50} relative gains of \textbf{Asr-VAE} over \textbf{SEREC} on samples from each quartile. Ideally, we expect our model to make gains on later quartiles since context is more important to distinguish diverse social contacts.
%
%\vspace{-6pt}
%
%\begin{table}[!htbp]
% \centering
% \begin{tabular}{@{}p{0.56\linewidth}p{0.069\linewidth}p{0.069\linewidth}p{0.069\linewidth}p{0.069\linewidth}@{}}
%  \toprule
%  \textbf{Neighbor Diversity Quartile} & \textbf{Q1\hspace{-2pt}}       & \textbf{Q2\hspace{-2pt}}          & \textbf{Q3\hspace{-2pt}}        & \textbf{Q4}             \\
%  \midrule
%  \textbf{\% Gain R@50 (Asr-VAE vs SEREC)} & 3.82\% & 3.16\% & 3.45\% & 4.23\% \\
%  \bottomrule
% \end{tabular}
%%  \vspace{1.5pt}
% \label{tab:neighbor_diversity}
% \vspace{-1pt}
% \caption{Performace gains of \textbf{Asr-VAE} against \textbf{SEREC} on user neighbor diversity. We see stronger gains for Q4 (high neighbor item-count diversity)}
% \vspace{-15pt}
%\end{table}
%
%
%
%
%
%%that methods incorporating social links obtain superior results to similar social-agnostic methods. Specifically, the SNCF version outperforms NCF, SBPR outperforms BPR (although by a tiny margin). Social GCN, which incorporate a BPR like loss, outperforms both of these by a small margin. Similar observations have been made in past work \cite{}, this is hardly surprising since social links can regularize the interest representations of sparse users and provide complementary knowledge for other users.
%
%%Second, although social methods 
%
%\subsection{Interpreting our Results}
%\label{subsec:Interpreting our Results}
%We now study our results more closely to understand the source of \textbf{Asr-VAE}'s gains over base recommender \textbf{VAE}. We observe the \emph{R@50} performance values of \textbf{Asr-VAE} against the base recommender \textbf{VAE} to observe the source of our gains. We analyze users along three axes - 
%\begin{description}
%\item [Item Count Quartile:] We separate the test users into 4 quartiles based on the number of items in their histories. 
%\item [Social Links Quartile:] We again separate test users into 4 quartiles depending on their social link counts.
%\item [User Coherence Quartile:] We define user coherence as the mean pair-wise correlation of item categories purchased by the user. Thus if a user were to purchase items that are often bought together, he receives greater coherence. We partition test users
%in 4 quartiles by coherence scores. We can compute coherence only for the \emph{Epinions} and \emph{Ciao} datasets.
%\end{description}
%
%We first study the overall performance variations and performance gains for users in different social and item count quartiles.
%
%\begin{figure}
%\hfill
%\subfigure[Asr-VAE $Recall@50$]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/performance/small_data_avg_perf_perf.pdf}}
%\hfill
%\subfigure[\% Gain Asr-VAE vs VAE $R@50$]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/performance/small_data_avg_perf_diff.pdf}}
%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}
%\vspace{-15pt}
%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across social link count and item count user quartiles (Q1 = lowest values, Q4 = highest values). Heatmap values are averaged over the smaller datasets (\textit{Ciao}, \textit{Epinions}, \textit{Delicious})}
%\vspace{-25pt}
%\label{heatmap:small_overall_diff}
%\end{figure}
%
%
%%\begin{figure}
%%\hfill
%%\subfigure[$Recall@50$]{\includegraphics[clip, trim=0.4cm 0.53cm 0.53cm 1.15cm, width=0.485\linewidth]{images/heatmaps/performance/delicious_perf_perf.pdf}}
%%\hfill
%%\subfigure[$Recall@50$ \textbf{(Asr-VAE - VAE)}]{\includegraphics[clip, trim=0.4cm 0.53cm 0.53cm 1.15cm, width=0.485\linewidth]{images/heatmaps/performance/delicious_perf_diff.pdf}}
%%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), averaged across the two larger datasets (Yelp, Ask-Ubuntu)}
%%\label{heatmap:delicious_overall_diff}
%%\end{figure}
%
%
%\begin{figure}
%\hfill
%\subfigure[Asr-VAE $Recall@50$]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/performance/big_data_avg_perf_perf.pdf}}
%\hfill
%\subfigure[\% Gain Asr-VAE vs VAE $R@50$]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/performance/big_data_avg_perf_diff.pdf}}
%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}
%\vspace{-15pt}
%\caption{Overall Performance and Percentage Gains of Asr-VAE (R@50), mean over larger datasets (\textit{Ask-Ubuntu}, \textit{Yelp})}
%\vspace{-17pt}
%\label{heatmap:big_overall_diff}
%\end{figure}
%
%
%%\begin{figure}
%%\hfill
%%\subfigure[$Recall@50$]{\includegraphics[clip, trim=0.4cm 0.53cm 0.53cm 1.15cm, width=0.485\linewidth]{images/heatmaps/performance/ciao_perf_perf.pdf}}
%%\hfill
%%\subfigure[$Recall@50$ \textbf{(Asr-VAE - VAE)}]{\includegraphics[clip, trim=0.4cm 0.53cm 0.53cm 1.15cm, width=0.485\linewidth]{images/heatmaps/performance/ciao_perf_diff}}
%%\hfill
%%\caption{Overall Performance and Gains over Base Model, Ciao Dataset}
%%\label{heatmap:ciao_overall_diff}
%%\end{figure}
%
%\textbf{Overall Results:} The heatmaps on the left in \Cref{heatmap:small_overall_diff}, \Cref{heatmap:big_overall_diff} indicate the performance (\emph{R@50}) achieved by Asr-VAE for users grouped under each quartile (Q1 - Lower values), averaged over the smaller and larger datasets respectively. We observe weaker performance for users at the bottom-left of the plot (i.e., users with sparse links and items). For the small datasets, stronger results appear at the other three corners (i.e., users who have either have a long item history, or several social connections). On the large datasets, results are concentrated towards users with greater link counts (social link quartiles Q3 and Q4). These gains are consistent with our intuitions, users with a large item history obtain accurate interest representations while those with more social links can socially regularize their interest embeddings.
%
%\textbf{Difference between Asr-VAE and VAE-CF:} The heatmaps on the right of each figure (\Cref{heatmap:small_overall_diff}, \Cref{heatmap:big_overall_diff}) indicate the relative performance gains of \textbf{Asr-VAE} against its base recommender \textbf{VAE} for users in the respective quartiles. We observe stronger performance gains in the bottom half of each heatmap, indicating improvements for users in the 25\% and 50\% item quartiles (i.e., users with sparse interest representations). As expected, social regularization benefits users with limited purchase histories. Surprisingly, we also see gains in the bottom left corner for the smaller datasets. It is feasible that users in these quartiles have fewer informative social links (since the datasets are smaller), making gains in \textbf{Asr-VAE} vs \textbf{VAE}.
%
%%\begin{figure}[htpb]
%%  \centering
%%  \subcaptionbox{Some subfigure\label{first-subfig}}{%
%%    % What you would typically have here is something like:
%%    % \includegraphics[width=0.2\textwidth]{some-file.pdf}
%%    % but for this example, let's go with a placeholder instead:
%%    \includegraphics[width=0.45\linewidth]{images/heatmaps/ciao_pairweight_item}
%%  }
%%  \subcaptionbox{Another subfigure\label{second-subfig}}{%
%%    \includegraphics[width=0.45\linewidth]{images/heatmaps/ciao_pairweight_item}
%%  }
%%  \caption{A caption for the single-column figure with two subfigures}
%%  \label{first-figure-with-subfigures}
%%\end{figure}
%
%
%\subsection{Pair-Weight Allocations}
%\label{subsec:Pair-Weight Allocations}
%The Hadamard projection vectors in our weighting function $w(u,v)$ are hard to interpret, since we do not know what each latent dimension is, however pair weights assigned to pair samples can be aggregated to analyze the training process. 
%
%
%\begin{figure}
%\hfill
%\subfigure[Smaller Datasets (\emph{Ciao, Epinions, Del})]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/small_pw_link.pdf}}
%\hfill
%\subfigure[Large Datasets (\emph{Ask-Ubuntu, Yelp})]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/big_pw_link.pdf}}
%\hfill
%%\caption{Overall Performance and Percentage Gains of Asr-VAE (by R@50), measured across user quantiles. Clearly, users in the third or fourth quartiles of either axis receive better overall recommendations. However, performance gains are mostly observed for users in the first and second item count quartiles (sparse histories)}
%\vspace{-15pt}
%\caption{We measure the Pair-Weight allocations to sampled pairs of users by our weight module. The x and y-axis denote the social link count quartiles of each user in pair (User-1, User-2), Q1 contains the lower values. E.g., The top-right box of the heatmap is the average weight alloted to samples where both users have many social links (Q4, Q4)}
%\label{heatmap:link_pw}
%\vspace{-7pt}
%\end{figure}
%
%
%\begin{figure}
%\hfill
%\subfigure[Small Datasets (\emph{Ciao, Epinions, Del})]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/small_pw_item.pdf}}
%\hfill
%\subfigure[Large Datasets (\emph{Ask-Ubuntu, Yelp})]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/big_pw_item.pdf}}
%\hfill
%\vspace{-5pt}
%\caption{We create these heatmaps similar to \Cref{heatmap:link_pw} with user item count quartiles, i.e., Q4 denotes long item histories}
%\vspace{-8pt}
%\label{heatmap:item_pw}
%\end{figure}
%
%%\begin{figure}
%%\hfill
%%\subfigure[Link-Count vs Link-Count]{\includegraphics[width=0.45\linewidth]{images/heatmaps/pw/epinions_pw_link.pdf}}
%%\hfill
%%\subfigure[Item-Count vs Item-Count]{\includegraphics[width=0.45\linewidth]{images/heatmaps/pw/epinions_pw_item.pdf}}
%%\hfill
%%\caption{The x and y axes in the above plots denote a specific user attribute for the two users in a pair (hence the plots are symmetric), User vs User link counts (left) and User vs User item counts (right) for the Epinions Dataset respectively.}
%%\label{heatmap:epinions_pw_link_item}
%%\end{figure}
%%
%%\begin{figure}
%%\hfill
%%\subfigure[Link-Count vs Link-Count]{\includegraphics[width=0.45\linewidth]{images/heatmaps/pw/delicious_pw_link.pdf}}
%%\hfill
%%\subfigure[Item-Count vs Item-Count]{\includegraphics[width=0.45\linewidth]{images/heatmaps/pw/delicious_pw_item.pdf}}
%%\hfill
%%\caption{User vs uUer link counts (left) and User vs User item counts (right) for the Delicious Dataset respectively.}
%%\label{heatmap:delicious_pw_link_item}
%%\end{figure}
%
%\begin{figure}
%\hfill
%\subfigure[\emph{Ciao} dataset]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/ciao_pw_coherence.pdf}}
%\hfill
%\subfigure[\emph{Epinions} dataset]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/epinions_pw_coherence.pdf}}
%\hfill
%\vspace{-10pt}
%\caption{Pair weights against user coherence for pair samples in the \emph{Ciao} and \emph{Epinions} datasets}
%\vspace{-10pt}
%\label{heatmap:ciao_pw_coherence}
%\end{figure}
%
%We observe from \Cref{heatmap:link_pw}, \Cref{heatmap:item_pw} that our model prioritizes pairs of users where both users have numerous social connections or longer item histories to regularize their neighborhoods. Intuitively, pair samples where both users are influencers or prolific consumers, are likely to be regularize their social and interest neighborhoods respectively (they may act as cluster centers). We observe a similar trend against user coherences in the \emph{Ciao} dataset (\Cref{heatmap:ciao_pw_coherence}). In \emph{epinions}, the model also prioritizes quartiles where one user in a pair has more coherent purchases than the other (note that we can only compute coherence for the \emph{Ciao, Epinions} datasets using their item category labels).
%
%Finally, we also analyze pair weights by considering differences within user pairs. We look at the difference in the number of social counts and length of item histories of the two users. \Cref{heatmap:asymm} indicates a slight drop in pair weights at the extreme right of each plot (large difference in social link count). Such connections are unlikely to represent friend-friend links and hence may not effectively regularize preferences. However, in \emph{Yelp}, \emph{Ask-Ubuntu} we observe a more uniform distribution of pair weights, potentially due to the information-seeking requirements of users on these websites.
%
%\begin{figure}
%\hfill
%\subfigure[Small Datasets (\emph{Ciao, Epinions, Del})]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/small_pw_asymm.pdf}}
%\hfill
%\subfigure[Large Datasets (\emph{Ask-Ubuntu, Yelp})]{\includegraphics[clip, trim=0.2cm 0.48cm 0.53cm 0cm, width=0.49\linewidth]{images/heatmaps/pw/big_pw_asymm.pdf}}
%\hfill
%\vspace{-12pt}
%\caption{Each pair sample (User 1, User 2) is binned in quartiles by item and social link count differences between the two users. We then plot the average pair weights assigned to the pair samples within the respective quantiles.}
%\label{heatmap:asymm}
%\vspace{-10pt}
%\end{figure}
%
%\subsection{Robustness and Interest Space Collapse}
%\label{subsec:Model Robustness and Mode-Collapse}
%We study the robustness of each adversarial model to lossy data by separately sub-sampling the social links and item ratings of each user in the respective training sets (\Cref{fig:robustness}). Performance is measured as a fraction of the peak performance (e.g., $0.98$ indicates the model degraded by 2\%). We observe an average performance degradation $\leq$ 3\% by \emph{R@50} with 10\% item ratings dropped and $\leq$ 6\% at 20\% drop, indicating our models are fairly robust to lossy item ratings. Asr-LRML shows a slightly steeper drop compared to the auto-encoder variants. Further, we observe our models are highly robust to social link drop, degrading by $5\%$ \emph{R@50} even with 50\% social links dropped, owing to their stochastic pair sample based gradient updates.
%%
%%\begin{figure}
%%\hfill
%%\subfigure[Performance with Data Drop]{\includegraphics[width=0.49\linewidth]{images/robustness-plot.pdf}}
%%\hfill
%%\subfigure[Recommendation Diversity]{\includegraphics[width=0.49\linewidth]{images/lambda-plot.pdf}}
%%\hfill
%%\caption{Our models are fairly robust at 10,20\% data drop (left); Greater recommendation diversity is observed for smaller $\lambda$ multiples, VAE appears more resistant to mode collapse}
%%\label{fig:robustness}
%%\end{figure}
%
%\begin{figure}
%\hfill
%\subfigure[Performance with Item Drop]{\includegraphics[width=0.49\linewidth]{images/robustness-item-plot.pdf}}
%\hfill
%\subfigure[And Social Link Drop]{\includegraphics[width=0.49\linewidth]{images/robustness-social-plot.pdf}}
%\hfill
%\vspace{-5pt}
%\caption{We observe $\leq 6\%$ \emph{R@50} degradation at 20\% item drop indicating our models are fairly robust in practice. Dropping social links results in much smaller performance drops, indicating the effectiveness of stochastic user pair sampling. Performance values are averaged across datasets.}
%\label{fig:robustness}
%\vspace{-10pt}
%\end{figure}
%%
%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{images/mode-collapse-plot.pdf}
%\vspace{-3pt}
%\caption{Recommendation diversity is observed to drop on either side of $\lambda_{opt}$, but due to different causes. The smaller $\lambda$ multiples result in overfitting to the supervised term $\mathcal{O}_{\mathbf{G}}$, while larger multiple result in interest space collapse, i.e., less diverse recommendations to socially clustered users. Diversity values are averaged across datasets.}
%\label{fig:modecollapse}
%\vspace{-14pt}
%\end{figure}
%
%We also analyze the effect of adversary weight $\lambda$ on the diversity of items recommended to users (\Cref{fig:modecollapse}). Specifically, we apply $k$-means clustering to the GAE \cite{graphae} embeddings for each social network, pick the median user cluster by average degree and measure recommendation diversity as the union of their top-50 recommendations. $\lambda_{opt}$ indicates the optimal $\lambda$ setting by \emph{R@50} for each dataset. As $\lambda$ is varied, the variation in diversity is measured as a percentage of the largest union set obtained (i.e., less diversity implies a smaller union set and hence lower percentage).
%
%In general, larger values of $\lambda$ result in less diverse recommendations. \textbf{Asr-VAE}'s recommendations are slightly more diverse at greater values of $\lambda$ owing to the stochasticity of the user representations in the \textbf{VAE} generator. On the opposite end, smaller multiples of $\lambda$ also produce lower recommendation diversity by over-fitting to the supervised loss term $\mathcal{O}_{\textbf{G}}$ in the generator objective in \Cref{eq:gen_obj}. Values close to $\lambda_{opt}$ produce the most diverse set of top-50 recommendations.
%
%\subsection{Parameter Sensitivity}
%\label{subsec:Parameter Sensitivity}
%
%
%
%
%In this section, we study the sensitivity of our model to two key parameter values, first the adversary weight $\lambda$, and second the user pair sample count $\epsilon$ (\Cref{fig:sensitivity2}) measured as a fraction of the total number of unique user pairs (e.g., 5\% denotes $0.05 \times \mathcal{U}^{2}$). 
%
%\begin{figure}
%\label{fig:sensitivity2}
%\includegraphics[width = \linewidth]{images/model_performance.pdf}
%\vspace{-2pt}
%\caption{Asr-VAE is fairly robust in a wide range of values ($\leq 2.5\%$ \emph{R@50} variation). $\lambda$ is varied as multiples of the best performing value $\lambda_{opt}$, larger multiples result in a performance drop. Robust performance is obtained for user pair sample count $\epsilon = 0.02 \mathopen | \mathcal{U} \mathclose |^2$, further samples provide small gains ($\leq$ 1\%). \emph{R@50} values are averaged across datasets.}
%\vspace{-9pt}
%\end{figure}
%
%Varying the adversary weight $\lambda$ results in a performance drop on either side of the optimal value. We find $\epsilon = 0.02 \times \mathcal{U}^{2}$ to provide an efficient tradeoff between compute-cost and performance. In practice $\epsilon$ does not significantly change the overall compute time, since the pair weight module is inexpensive. Also note that $\lambda_{opt}$ varies across datasets, with values on either side of $\lambda_{opt}$ resulting in weaker and less diverse recommendations (\Cref{fig:modecollapse}).
%
%\subsection{Limitations}
%\label{subsec:Limitations}
%We identify a few key limitations of our model. First, although the model performance is stable around multiples of the optimal values of $\lambda_{opt}$, the optimal weight varies across datasets and applications. The optimal strength of social regularization depends on the data semantics as well the generator and discriminator architectures. Second, the pair-weighting strategy performs best when the provided context features are meaningfully correlated to the interests and social indicators of users. Thus, depending on the application, context features should be picked to enhance social inference and prevent loss of diversity in the generated recommendations.
%
%


==> SIGIR 2020 copy/inference.tex <==
% !TEX Root=draft.tex

\section{Model Inference}
\label{sec:Model Inference}
%\input{datadesc}
In this section, we describe an efficient Gibbs-sampling approach for model inference, analyze its computational complexity and propose a parallel batch-sampling approach for speed-up. In each iteration of Gibbs-sampling, we unseat users one at a time and re-sample their seating as in ~\Cref{eq:updatedCRP}. Profile and Action-topic distributions are simultaneously updated, while hyper-parameters are modified between Gibbs iterations. We factor the seating sampler (\Cref{ul}) for efficiency since the number of tables is not fixed. We speed-up convergence times with coherent initial seating based on similar action distributions and content tags.\vspace{-20pt}
% We iteratively sample user seating and update profile parameters to reflect the seating until mutual convergence as illustrated in \cref{crpmap}.
%\subsection{Inference via Gibbs Sampling}
%\label{subsec1}
% \subsubsection{Tables Initialization:}

% \subsubsection{Sampling Seating Arrangements:}
\begin{center}

 \begin{figure}[b]
 \vspace{-10pt}
  \includegraphics[width=0.86\linewidth, trim={4.25cm 1.9cm 6.1cm 0cm},clip]{images/image_intro.pdf}
 \caption{Our Gibbs-sampler simultaneously samples the seating arrangement of users (eq. 13) and learns profiles to describe the seated users (eq. 9, 10, 11). Users are grouped by behavioral similarity to overcome sparsity.}
  % \caption{Illustration of our Skew-aware Partitioning and Profiling Approach, Note that profiles are learned at the partition level to tackle inactive users. Our seating process simultaneously samples user partitions and learns profiles.}
  \label{crpmap}
 \end{figure}
\end{center}


\begin{center}
 \begin{table}[t]
%  \vspace{10pt}
  \begin{tabular}{lp{0.7\linewidth}}
   \toprule
   \textbf{Symbol}                         & \textbf{Description}                                                                            \\
   \midrule
   $n_{k}^{(w)}, n_{k}^{(a)}, n_{k}^{(.)}$ & Number of times word $w$, action $a$ were assigned to topic k, and respective marginals         \\
   $n_r^{(k)}, n_r^{(.)}$                  & Number of times interactions of users served profile $r$ was assigned topic k and marginal      \\
   $n_{r,r'}^{(\ell)}, n_{r,r'}^{(.)}$     & Number of $\ell$-labeled exchanges, all exchanges between users in tables serving $r$ with $r'$ \\
   \bottomrule
  \end{tabular}
  \label{gibbsnotation}
%   \vspace{-10pt}
  \caption{Gibbs-sampler count variables}
  \vspace{-15pt}
 \end{table}
\end{center}



The likelihood of generating a user interaction $d = (a,W,t) \in \mathcal{D}_{u}$ conditional on action-topic $k \in K$ is:
\begin{equation}
 p(a,W \mid k) \propto  \frac{n_{k}^{(a)} + \alpha_{\mathcal{A}}}{n_{k}^{(.)} + |\mathcal{A}|\alpha_{\mathcal{A}}} \times \prod_{w \in W}\frac{n_{k}^{(w)} + \alpha_{\mathcal{V}}}{n_{k}^{(.)} + |\mathcal{V}|\alpha_{\mathcal{V}}}.
 \label{dk}
\end{equation}
Thus, the likelihood $p(d \mid r)$ of interaction $d = (a,W,t)$ for a user  served activity profile $r \in R$,~\Cref{eqx} is:
\begin{equation}
 p(d \mid r) \propto \sum_{k \in K} \frac{n_{r}^{k} + \alpha_K}{n_{r}^{(.)} + |K|\alpha_K} \times p(a,W,t \mid k,r).
 \label{dr}
\end{equation}
The likelihood that knowledge exchange occurs between profile pairs $(r, r')$ on type $\ell$ is:
\begin{equation}
 \phi_{r,r'}^{\mathcal{L}}(\ell) = \frac{n_{r, r'}^\ell + \alpha_{\mathcal{L}}}{n_{r, r'}^{(.)} + |\mathcal{L}|\alpha_{\mathcal{L}}}.
 \label{lr}
\end{equation}
Thus, the conditional likelihood in~\Cref{upfinal} can be obtained via~\Cref{dr} over $\mathcal{D}_u$ and~\Cref{lr} over $L_u$ respectively. We can seat a user $u$ either on an existing table $x \in \{1, \ldots, \chi\}$ serving profile $r_x$ or on a new table $\chi+1$; \Cref{eq:updatedCRP}, conditioned on the seating of all other users, denoted by $x_{-u}$. To avoid likelihood computation over all tables, we perform the draw in two factored steps. We first sample the profile served to $u$ by marginalizing over tables via~\Cref{eq:profiledist-eq2},


\begin{equation}
 P( r \mid u, x_{-u}) \sim \left ( \frac{N_{r} - \chi_{r} \delta}{N+\gamma}  + \frac{\gamma+\chi\delta}{|R|(N+\gamma)}   \right ) p(u \mid r),
 \label{ul}
\end{equation}
and then sample from the set of tables serving the sampled profile (including the possibility of a new table with this profile draw),
\begin{equation}
 P(x \mid r, u, x_{-u}) \sim
 \begin{cases}
  \frac{n_{x}-\delta}{N+\gamma} \times \mathbbm{1}(r_x = r), & x \in \{1,\ldots, \chi \}, \\
  \frac{\gamma+\chi\delta}{N+\gamma} \times \frac{1}{|R|},   & x = \chi+1                 \\
 \end{cases}
 \label{user_seat}
\end{equation}
Note that $N = |\mathcal{U}|-1$, i.e. all users except $u$. If we draw a new table $\chi+1$, we assign the sampled profile variable $r$. We update all counts (~\Cref{gibbsnotation}) corresponding to prior profile and action-topic assignments for $u$.

% Given $p(u \mid r)$ we can sample profile $r_u$ for user $u$ as in \cref{eq:profiledist},
%
%where $a_{-u},r_{-u},k_{-u}$ indicate the seating and profile assignments of all other users, and the behavior assignments for their interactions. Behavior assignments for each interaction $d \in \mathcal{D}_u$ are sampled in proportion to \cref{dr} with $r = r_u$, the chosen profile for $u$, and the user is seated either on an existing table $a \in [1, A]$ serving $r_u$, or new table $A+1$ with $r_{A+1} = r_u$,


% \subsubsection{Parameter Estimation: }\label{parameter}
We use well known techniques to update parameters. At the end of each sampling iteration, we update Multinomial-Dirichlet priors $\alpha_{\mathcal{V}}$, $\alpha_{\mathcal{A}}$, $\alpha_{K}$ and $\alpha_{\mathcal{L}}$ by Fixed point iteration~\cite{fpi}. We update Beta parameters $(\alpha_{r,k}, \beta_{r,k})$ by the method of moments~\cite{tot}. We round all time-stamps to double-digit precision and we cache probability values $p(t \mid r,k)$ $\forall$ $t \in [0,1], r \in R, k \in K$ at the end of each sampling iteration, thus avoiding $R \times K$ scaling for $p(u \mid r)$ in~\Cref{ul}. While we fix the Pitman-Yor parameters in our experiments for simplicity, if needed, we can estimate them via auxiliary variable sampling~\cite{pytm, teh}.

\subsubsection*{\textbf{Computational Complexity}}
Our inference is linear in the number of users $|\mathcal{U}|$ and interactions $|\mathcal{D}|$ , scaled by $R + K$ (see empirical results in~\Cref{fig:memtime}). To see this, notice that in each Gibbs iteration, computing~\Cref{dk,dr} involves $|\mathcal{D}| \times (K+R)$ computations.~\Cref{ul} requires an additional $|\mathcal{U}| \times R$ computations. We prevent $R \times K$ scaling for $p(u\mid r)$ in~\Cref{ul} by caching. We cache the first product term of~\Cref{ul} for each $r \in R$, and update it only when there is a change in the seating arrangements on tables serving profile $r$.

\subsubsection*{\textbf{Parallelization with Batch Sampling}}
We scale to massive datasets by parallelizing inference via batch-sampling. The Gibbs sampler described above samples each user's seating $P( x_u \mid u, x_{-u})$ in \Cref{user_seat}, conditioned on all other users. This necessitates iteration over $\mathcal{U}$. Instead, seating arrangements could be simultaneously sampled in batches $U \subset \mathcal{U}$ conditioned on all users outside the batch, i.e. $P( x_{U} \mid U, x_{\mathcal{U}-U})$ where $x_{U}$ denotes the table assignments to users in batch $U$. For efficiency, batches must be chosen with comparable computation. We approximate computation for $u \in \mathcal{U}$ $\propto$ $|\mathcal{D}_u| + |\mathcal{L}_u|$ to decide apriori batch splits for sampling iterations. Note that when batch sampling, we can only exploit knowledge exchange links between users in the batch and users \textit{not} in the batch. In practice, since $|U| \ll |\mathcal{U}|$, the impact of not using knowledge exchanges between users in the same batch turns out to be negligible.


==> SIGIR 2020 copy/introduction.tex <==
%!TEX root = main.tex
\vspace{-7pt}
\section{Introduction}
\label{sec:introduction}

% Recommender systems are a ubiquitous part of our lives today, affecting our interactions with products, services, and content across varied domains. The rapid proliferation of users and items in the social web has aggravated the grey-sheep user/long-tail item challenge in recommendation. Traditional collaborative filtering, as well as the more scalable neural collaborative filtering (NCF) approaches~\cite{vaecf, ncf} continue to suffer from sparse interaction data. In fact, sparsity challenges have become more pronounced \cite{longtail-neural}, motivating us to \textit{learn-to-learn neural embeddings}, i.e., 

The focus of this paper is to learn to build expressive neural collaborative representations of users and items with sparse interaction data. The problem is essential: neural recommender systems are crucial to suggest useful products, services, and content to users online. Sparsity, or the long tail of user interaction, remains a central challenge to traditional collaborative filtering, as well as new neural collaborative filtering (NCF) approaches~\cite{ncf}. Sparsity challenges have become pronounced in neural models~\cite{longtail-neural} owing to generalization and overfitting challenges, motivating us to \textit{learn-to-learn} effective embedding spaces in such a scenario.
Cross-domain transfer learning is a well-studied paradigm to address sparsity in recommendation. However, how recommendation domains are defined plays a key role in deciding the algorithmic challenges. In the most common pairwise cross-domain setting, we can employ cross-domain co-clustering via shared users or items~\cite{wsdm19, ijcai17}, latent structure alignment~\cite{ecmlpkdd13}, or hybrid approaches using both~\cite{www19tmh, www19cngan}. However, recommendation domains with limited user-item overlap are pervasive in real-world applications, such as geographic regions with disparities in data quality and volume (e.g., restaurant recommendation in cities vs. sparse towns). Historically, there is limited work towards such a \textit{few-dense-source}, \textit{multiple-sparse-target} setting, where entity overlap approaches are ineffective. Further, sharing user data entails privacy concerns~\cite{ncf-privacy}. 


Simultaneously, context-aware recommendation has become an effective alternative to traditional methods owing to the extensive multi-modal feedback from online users~\cite{cikm18context}. Combinations of contextual predicates prove critical in \textit{learning-to-organize} the user and item latent spaces in recommendation settings. For instance, an \textit{Italian wine restaurant} is a good recommendation for a \textit{high spending} user on a \textit{weekend evening}. However, it is a poor choice for a \textit{Monday afternoon}, when the user is at work. The intersection of restaurant type (an attribute), historical patterns (historical context), and interaction time (interaction context) jointly describe the likelihood of this interaction. 
Our key intuition is to infer such \textit{behavioral invariants} from a \textit{dense-source} domain where we have ample interaction histories of users with wine restaurants and apply (or adapt) these learned invariants to improve inference in \textit{sparse-target} domains. Clustering users who interact under covariant combinations of contextual predicates in different domains lets us better incorporate their behavioral similarities, and analogously, for the item sets as well. The user and item representations in sparse domains can be significantly improved when we combine these transferrable covariances.

%Thus, there is an innate need to design recommendation systems that address data sparsity issues in practice.

%The long-tail challenge has been an enduring practical consideration in the design and application of real-world recommender systems~\cite{longtail1, longtail2}. In recent times, profiling and recommendation models rely on high-volume online behavioral data, exacerbating the presence of the sparse tail and its extent of interaction sparsity. Neural Collaborative Filtering (NCF) architectures have proven significantly more scalable and effective in comparison to Matrix-Factorization models~\cite{vaecf, ncf}. However, the long-tail challenge persists, or even becomes more pronounced \cite{longtail-neural}. Thus there is a need to \textit{learn-to-learn neural embeddings}, i.e., learn to build expressive neural representations of users and items with sparse interaction data, to effectively leverage behavioral data for recommendation.

% Cross-domain recommendation is known in the literature to alleviate data sparsity~\cite{cross-domain-sparse, codebook}. Transfer learning has employed co-clustering via shared entities~\cite{wsdm19, ijcai17}, latent structure transfer~\cite{ecmlpkdd13}, or a hybrid approach involving both~\cite{www19tmh, www19cngan}. Depending on the definition of a recommendation domain, the challenge presents itself in different forms. In the pairwise user-shared (or item-shared) cross-domain setting, the interaction structure in the dense domain is leveraged to improve recommendations in the sparse domain, grounded upon the shared entities~\cite{codebook, ijcai17}. However, the non-pairwise setting is pervasive in real-world applications, such as geographic region based domains, where we must alleviate regional disparities in data quality and volume (e.g., restaurant recommendation in densely populated cities vs. sparsely populated towns). In such a challenging \textit{few-dense-source}, \textit{many-sparse-target} setting, the shared entity approach (shared users, items, external context) is unlikely to prove effective. Further, there are significant privacy concerns with sharing user data across domains~\cite{ncf-privacy}. 

Guiding neural representations is also a central theme in gradient-based meta-learning. Recent work~\cite{maml, meta-learn-similar} measures the plasticity of a base-learner via gradient feedback for few-shot adaptation to multiple semantically similar tasks. However, the base-learner is often constrained to simpler architectures (such as shallow neural networks) to prevent overfitting~\cite{DBLP:journals/corr/abs-1812-02391} and requires multi-task gradient feedback at training time~\cite{maml}. This strategy does not scale to the embedding learning problem in NCF, especially in the \textit{many sparse-target} setting. 

Instead, we propose to incorporate the core strengths of meta-learning and transfer learning by defining transferrable neural layers (or meta-layers) via contextual predicates, working in tandem with and guiding domain-specific representations. Further, we develop a novel adaptation approach via regularized residual learning to incorporate new target domains with minimal overheads. Only residual layers and user/item embeddings are learned in each domain while transferring meta-layers, thus also limiting sparse domain overfit. In summary, we make the following contributions:

%We propose a novel, cross-domain, meta-transfer learning problem grounded on contextual invariants to organize embedding spaces (i.e., \textit{learn-to-learn embedding representations}) with an aim of addressing target domain sparsity.  




%In recommendation settings, we typically observe three different modes of context: \textit{Interactional} (Describes the conditions of a specific user-item interaction, e.g., time/day of the interaction); \textit{Historical} (Describes past interactions, historical patterns for the interacting user or item); \textit{Attributional} (Time-invariant attributes, e.g., item descriptions).

%\begin{itemize}
% \vspace{-5pt}    
%  \noindent \textbf{Interactional Context:} Describes the conditions of a specific user-item interaction, e.g., time/day of the interaction. 
%     %They can vary across interactions of the same user-item pair.
%     %Interactional context variables are neither dependent on the user, nor the item. Examples of such context include the time and day of the interaction, the location of the interaction, etc. 
%     %the value of the transaction or the spend (spend may be an item attribute in some cases rather than a transactional aspect, it is transactional in user-merchant interactions) etc.
    
%    \noindent \textbf{Historical Context:} Describes past interactions and historical patterns for the interacting user or item.
    
%     %, e.g., user's interaction pattern for an item (or, item category).
% %    Examples of historical context include movie watching or restaurant spending habits of the user, and conversely, popularity of the movie or book, average tip amounts at a restaurant etc. 
    
%    \noindent \textbf{Attributional Context:} Encapsulates time-invariant attributes, e.g., item descriptions. 
    
    %They do not vary across interactions of the same user-item pair.
    %Item descriptions fall under this category, as does demographic descriptors of users such as age-group, gender, etc.
%\vspace{-2pt}  
%\end{itemize}

% Transferrable recommendation domains provide us semantically related context. We can leverage context to develop deeper insights into user-item interactions than black-box latent representations~\cite{ncf}. 



% While the user and item embeddings are domain-specific, 


% We are motivated by the presence of contextual/behavioral invariants describing users' choices, and their application to generate more descriptive representations, especially with sparse data.

%Further, a similar organization of the embedding spaces also enables uniform mapping functions for recommendation to be transferred across domains.

%This knowledge can be effectively leveraged to understand user motivations for each interaction better, and hence organize the user and item embedding spaces by their requirements and characteristics respectively (i.e., \textit{learn to learn latent space representations}). Sharing a context-driven meta-learner provides a data-efficient solution to profile users and items across several sparse domains sharing the interaction characteristics of the source domain. 

% Further, we propose a novel adaptation approach via regularized residual learning to effectively incorporate new target domains with minimal overheads. Only the residual layers and user/item embeddings are learned on a per-domain basis while transferring the source model layers directly, thus controlling for overfitting to sparse data. 


%A central application of our framework is to address regional disparities in data availability and quality. Most existing related efforts in the literature are only applicable to settings where users or items or their subsets are shared across the different domains, and second, when there is external content associated with each item. 

\begin{description}[leftmargin=0pt, labelindent=\parindent]
%\begin{itemize}
    \item[Contextual invariants for disjoint domains:] We identify the shared task of \textit{learning-to-learn} NCF embeddings via cross-domain contextual invariances. We develop a novel class of pooled contextual predicates to learn descriptive representations in sparse recommendation domains without sharing users or items.
    
%     While invariants are intuitive and well-defined for computer vision tasks, it is harder to unify latent collaborative representations across recommendation domains.
    \item[Tackling the \textit{one-dense}, \textit{many-sparse} scenario:] Our model infers invariant contextual associations via user-item interactions in the dense source domain. Unlike gradient-based meta-learning, we do not sample all domains at train time. We show that it suffices to transfer the source layers to new target domains with an inexpensive and effective residual adaptation strategy. 
    \item[Modular Architecture for Reuse:] Contextual invariants describing user-item interactions are geographically and temporally invariant. Thus we can reuse our meta-layers while only updating the user and item spaces with new data, unlike black-box gradient strategies~\cite{maml}. This also lets us embed new users and items without retraining the model from scratch.
    \item[Strong Experimental Results:] We demonstrate strong experimental results with transfer between dense and sparse recommendation domains in three different datasets - % two publicly available datasets 
    (Yelp Challenge Dataset\footnote{\url{https://www.yelp.com/dataset/challenge}}, Google Local Reviews\footnote{\url{http://cseweb.ucsd.edu/~jmcauley/datasets.html}}) for benchmarking purposes and a large financial transaction dataset from Visa, a major global payments technology company. 
    %massive corporate dataset of financial transactions across multiple regions in the United States. 
    We demonstrate performance and scalability gains on multiple sparse target regions with low interaction volumes and densities by leveraging a single dense source region. 
    %user or item overlaps constraints.
%end{itemize}
\end{description}
%Our work is particularly significant in comparison to previous transfer-learning efforts since it enables adaptation to several sparse target domains with a single dense source-learned meta-model while tackling the constraints of pure gradient-based meta-learning.
 We now summarize related work, formalize our problem, describe our approach, and evaluate the proposed framework.




%\begin{itemize}
%\item 
% \vspace{-2pt}
% \begin{enumerate}[label=\Roman*]
% \item \noindent \textbf{Tackling the sparsity challenge without sharing constraints:} We propose the meta-problem of \textit{learning-to-learn} NCF embeddings via cross-domain contextual invariances. While invariants are intuitive and well-defined for computer vision tasks, it is harder to unify latent collaborative representations across recommendation domains. We propose and evaluate a novel class of pooled contextual predicates to learn descriptive representations in data-sparse recommendation domains, without relying on shared users or items.
% %user or item overlaps constraints.
% %shared users, items, or external content. 

% \item \noindent \textbf{Addressing the challenging \textit{one-dense}, \textit{many-sparse} domain setting:} We learn a central meta-model on the dense source domain to infer invariant associations of contextual factors, describing user-item interactions. In contrast to past work, we do not rely on shared entities or expensive gradient co-training across domains. We demonstrate that it is sufficient to learn a meta-model on the source data, and scale to many target domains with an inexpensive and effective residual adaptation strategy. 
% %Cardholder and restaurant embeddings, as well as a residual/distributional adaptation component of the target domains,  accommodate the underlying differences across the different pockets. For example, restaurants in a major city like San Francisco in California will have a different pricing range than restaurants in a small town Elko in Nevada. It is known that restaurant pricing is an important contextual factor defining cardholders eating out activities. The central meta-learner will capture the importance of pricing, while the residual/distributional alignment will balance the region-specific variations.

% %A related argument is to fit a joint model that simultaneously trains on both the source and target domains. Through extensive experimental results, we show that such an approach results in an inferior fit compared to meta-learner transfer followed by regional customization. 
% %$$M_{T+S} \leq M_{T \rightarrow S}$$ In retrospect, joint training of source and target domains ($M_{T+S}$) is expected to be biased to the rich source data and thus less effective on the target domain compared to meta-transfer followed by annealing ($M_{T \rightarrow S}$).


% %\item 
% \item \noindent \textbf{Modular Construction for Prototyping:}  Contextual invariants describing user-item interactions are geographically and temporally invariant, enabling us to reuse our meta modules and transformation layers with minimal effort, unlike black-box latent models. We can thus perform inexpensive updates to our learned user embeddings, and rapidly incorporate for new users and items with limited data.

% %Furthermore, the generated models require updates to leverage recent interaction activity and the evolution of user preferences. The contextual factors that underly user-item interactions are temporally and geographically invariant (except for residual adaptation), thereby enabling the majority of our model not to require updates.


% %Our approach is specifically suited to such a setting. We experimentally demonstrate that a small number of annealing epochs with the transferred meta-model can rapidly generate a high-performance recommender model for a new region or cardholder/restaurant embedding updates. Intuitively, the contextual factors that are important to the restaurant recommendation model do not change (e.g., pricing), thereby enabling the majority of our model not to require updates. On the other hand, a specific cardholder's financial situation may change, as evident from her recent transactions, and annealing on the new data is enough to capture this.


% %\item 

% \item \noindent \textbf{Strong Experimental Results:} We demonstrate strong experimental results, both within and across recommendation domains on three different datasets - % two publicly available datasets 
% (Yelp Challenge Dataset\footnote{\url{https://www.yelp.com/dataset/challenge}}, Google Local Reviews\footnote{\url{http://cseweb.ucsd.edu/~jmcauley/datasets.html}}) for benchmarking purposes, 
% as well as a large financial transaction dataset from a major payments technology company. 
% %massive corporate dataset of financial transactions across multiple regions in the United States. 
% We demonstrate performance and scalability gains across multiple sparse target regions with low interaction volumes and densities, by leveraging a single dense source domain in each dataset.
% \end{enumerate}



%\noindent $\textbf{IV.}$ \textbf{Dealing with Skew and Sparsity in Massive Volumes of Real-World data} Our solution has the ability to adapt to data pockets or regions with low volumes and/or low density. Recommender systems are known to be sensitive to two conditions - the overall volume of training data and per-user data density. These often limit a recommendation model from fitting to new data. In our solution, the meta-learner captures the most important combinations of context that dictate cardholder eating out decisions. This enables us to deal with low density of cardholder data. If a cardholder has a single transaction, the meta-learner knows what important combinations to look for to build a suitable representation for that cardholder, thus using her data more efficiently. We generate a heatmap that demonstrates how the tolerance of our model to low density and low volume targets is significantly improved by transferring the meta-model from the dense source domain.


%Our approach enables horizontal scaling without user or item sharing constraints across several sparse target domains.

%We emphasize two key observations from past work - First, an effective strategy to tackle sparsity is the notion of cross-domain transfer learning, wherein data-rich domains are leveraged to improve recommendations in a data-sparse recommendation domain. Although there are numerous definitions of domain in the past literature, diverse methods have proven effective in these cross-domain settings.





%Recommender systems are a ubiquitous part of our lives today. They affect how users interact with products, services, and content in a wide variety of domains. The past decade has witnessed significant efforts from both academia and industry in developing recommender systems that are personalized, scalable, online, trust-aware, context-aware, etc. Most of these systems necessitate the underlying algorithm to mine interesting patterns from large volumes of rich user-item interaction data. However, owing to the presence of millions of users and items in a domain, practical recommender systems face two primary challenges - data sparsity and scalability. Conventional collaborative filtering methods like matrix factorization and their sparsity-aware extensions do not scale to the massive volumes of data generated by users today. The humongous volume of user-item interaction data further exacerbates the long-tail and the overall data skew concerns, thereby generating low quality inferences for majority of users and items. Recent years have witnessed the rise of cross-domain recommendation techniques that handle data sparsity by assuming the presence of shared users/items or other forms of auxiliary content across dense source that is transferred to improve recommendation quality in sparse target domains~\cite{codebook, DBLP:reference/sp/CantadorFBC15, ijcai17, volkovs2017content, wsdm19}. It is hard to quantify the volume of shared content or entities (i.e., users/items) that can effectively facilitate such transfer learning. Additionally, it is also not reasonable to assume availability of auxiliary information or overlap of users/items between the source and target domains in today's privacy-conscious world. 
%
%Meta-learning has been proposed as a framework to address the challenging few-shot learning problem that learns a model with a small amount of data~\cite{DBLP:journals/corr/abs-1812-02391}. The key idea is to leverage a large number of similar tasks that share a lot in common with a common base learner that is adapted to specialize to each task via few-shot learning. We observe similar challenges in the latent factor collaborative filtering setting where the different recommendation domains constitute the related tasks. A domain is a particular field of thought, activity, or interest. Recommendation literature has different definitions for domain such as different types of items (e.g., movies vs. books), different types of users (e.g., pay-per-view users vs. users with yearly subscription), different distributions of data (e.g., dense and rich data vs. sparse and long-tail data), etc. Our framework defines domain as dense source region and sparse target region, much akin efforts in cross-domain recommendation literature. We draw parallel between few-shot learning task and recommendation task and propose a meta-transfer learning framework that improves the quality of recommendation under limited (sparse and skew) data conditions. Meta-transfer learning is different from transfer-learning in which a model trained on one task is re-purposed on a second related task. Meta-transfer learning transfers knowledge too, but aims to meta-learn what and how to transfer effectively from one domain to another. Sun {\em et al}~\cite{DBLP:journals/corr/abs-1812-02391} provides a detailed comparison between meta-learning, transfer learning, and meta-transfer learning.
%
%
%Our meta-transfer learning paradigm offers numerous advantages over standard transfer learning techniques for cross-domain recommendations. It empowers us to learn a central base learner from rich dense source domain that can be eventually few-shot adapted or transferred to multiple target domains. It also offers flexibility to define the shared aspects captured by the base learner and the advantages of rapid prototyping via adaptation to new users and/or items. As mentioned above, our framework defines domain as dense source region and sparse target region. All existing related efforts in the literature are only applicable to one of two settings - first, where the same set of users or items or their subsets are shared across the different domains, and second, when there is external content associated with each item. However, we relax the assumption of shared users/items or other forms of auxiliary content since it is unrealistic in practice. For example, a framework that transfers knowledge learnt from a restaurant recommendation model built on dense and rich San Francisco Bay Area data (source) to improve the quality of restaurant recommendation in a small town Elko in Nevada (target) cannot assume shared users between the source and target domain in reality. Even if the source and target domain share some common users, the percentage is miniscule. 
%
%%While transfer learning is a well-studied problem in the machine learning community, all transfer learning techniques in the literature are only applicable to one of two settings - first, where the same set of users or items or their subsets are shared across the different domains, and second, when there is external content associated with each item. In most real world recommender systems, we do not observe an adequate proportion of shared users or items to anchor the transferred recommendation models. Further, textual descriptions of items provide us a limited understanding of users and their motivations for engaging in a specific user-item interaction, limiting the utility of the transferred knowledge. 
%
%Meta-learning or meta-transfer learning has been popularly employed by researchers in Computer Vision and Natural Language Processing~\cite{DBLP:journals/corr/abs-1812-02391, DBLP:conf/iclr/WolfCD18}.
%%Unlike research areas such as Computer Vision, most existing collaborative filtering methods cannot leverage meta-learning to adapt a versatile base learner across recommendation domains.  
%Unlike learning tasks in Computer Vision where there are geometric invariants facilitating the transfer process (or, Natural Language Processing where semantic similarity between source and target drive the transfer), latent factor models for recommender systems are not readily amenable to the meta-transfer setting.  
%Vartak {\em et al}~\cite{nips17} transfer a function across users as in content-based filtering methods, thereby enabling a meta-level shared model across sparse and dense users. However, the effort is not grounded on a principled set of invariants and is applicable specifically for new item cold-start recommendation problem. 
%
%In this work, we propose a novel approach to leverage the versatility and strength of meta-learning for collaborative filtering based recommendation. We observe that the proposed solution addresses a wide range of issues typically faced by practical recommender systems. Our proposed recommender system framework is amenable to meta-learning while:
%\begin{itemize}
%\item retaining the core embedding representations of users and items that are common to all collaborative filtering algorithms
%\item learning a meta component to guide the embedding learning process, that is transferrable across recommendation domains, grounded on a novel set of contextual invariants
%\end{itemize}
%
%The goal of any recommender system is to understand how users interact with items. The best predictors of user-item interactions often lie at the intersection of their context information. For example, a user with greater than average spending habits is likely to visit an expensive restaurant for dinner. A user with kids at home is likely to watch a children's movie on a weekend afternoon. These contexts are true and indepedent of the underlying domain. This motivates us to propose contextual invariants for meta-transfer learning in recommendation. Context variables are predicates of a specific user-item interaction. We typically observe three different types of context variables that are critical to recommendation:
%
%\begin{itemize}
%    \item \textbf{Interactional Context:} These predicates describe the conditions under which a specific user-item interaction or transaction occurs. Interactional context variables are neither dependent on the user, nor on the item. Examples of such context include the time and day of the interaction, the location of the interaction, etc. 
%    %the value of the transaction or the spend (spend may be an item attribute in some cases rather than a transactional aspect, it is transactional in user-merchant interactions) etc.
%    
%    \item \textbf{Historical Context:} Historical predicates describe the past interactions associated with the user or item of interest. Examples of historical context include movie watching or restaurant spending frequency of the user, and conversely, total number of views of the movie or total number of purchases at the restaurant. 
%    
%    \item \textbf{Attributional Context:} Attributional context encapsulates the time-invariant attributes of users and items. Item descriptions fall under this category, as does demographic descriptors of users such as age-group, gender, etc.
%\end{itemize}
%
%Some of these contexts or a combinations of contexts provide us a lens or perspective to analyze and draw inferences about the interacting users and items. Users who engage in interactions with items under similar combinations of contextual predicates should be clustered in the user embedding spaces and recommended the appropriate clusters of items that cater to their tastes. While the user and item embeddings are specific to each domain, we propose a novel meta-learning component that learns to organize these spaces based on the observed contextual predicates, and describes the mapping between suitable clusters of users and items in the respective spaces.
%
%
%\vspace{0.10in}
%\noindent \textbf{Motivation and Problem {\em wrt} Visa:} There is growing interest inside Visa to personalize cardholder and merchant experience with advanced AI technologies. Visa intends to build data-driven solutions that recommend restaurants, generates itineraries for travel, predicts cardholder's next purchase, etc. There are several challenges associated with building such systems for Visa such as data scalability, data sparsity, cold-start cardholders and merchants, model updation, etc. Additionally, a recommender engine built for Visa using Visa's transaction data need to learn cardholder and merchant embeddings, i.e., feature vectors, in order to return high quality personalized recommendation. It must also leverage the rich contextual information associated with cardholder-merchant interaction in its solution.
%
%In this work, we design a novel recommendation model, namely a restaurant recommendation system, that addresses data sparsity and data scalability challenges seamlessly by meta-transfer learning from dense source domain to sparse target domain\footnote{We explain our idea using restaurant recommendation. However, the solution works for any user-item/cardholder-merchant application.}. Unlike previous efforts, our solution does not assume shared users/items or other forms of auxiliary content between the source and the target. Specifically, we build a restaurant recommendation model for rich dense data (i.e., US cardholders eating at US restaurants), and meta-transfer the learnt knowledge to generate high quality restaurant recommendations for sparse data (i.e., cardholder from Country X eating at restaurants in Country X). Note that, it is known that Visa data outside the US has poor quality. Our model can also be employed for learning high-quality restaurant recommendations in dense data pockets in the US (e.g., San Francisco Bay Area in California) and generating better quality restaurant recommendations in sparse data pockets in the US (e.g., Alpine County in California). Thus, our work supports restaurant recommendation in the US, restaurant recommendation globally, as well as cross-border restaurant recommendation.  
%
%%Data sparsity is a challenging problem for recommender systems. Broadly we identify two sources of sparsity. First, the reviews or purchase activity per user, namely the transaction density and second, the overall volume of review or purchase activity. Note that while the first is important to build descriptive user profiles, the second is equally important to build item profiles and learn the space of features that are critical to make suitable recommendations.
%%A promising and well-studied solution to this problem is cross-domain recommendation, wherein data from multiple recommendation domains can be leveraged to collectively improve recommendation quality. Broadly, existing efforts in cross-domain recommendation literature can be partitioned into three buckets: 
%%\noindent (i)user-shared setting (i.e., US cardholders traveling to Country X and receiving recommendations for restaurants in Country X), 
%%\noindent (ii) item-shared setting (i.e., cardholders from Country X traveling to the US and receiving recommendations for restaurants in the US), and 
%%\noindent (iii) linked domain setting with no user/item sharing. 
%
%%In our work, we handle the generic scenario, i.e., the linked domain setting where source and target domains focus on restaurant recommendation without assuming cardholder and/or restaurants in common between the two domains.   
%%\begin{itemize}
%%    \item User or Item-Shared Setting 
%%    \item Shared Content Setting
%%    \item Linked Domain Setting with No-Sharing (Ours)
%%\end{itemize}
%
%%In this work, we propose a novel class of invariants grounded on contextual predicates that can be effectively leveraged for linked-domain recommendation independent of the above assumptions.
%
%%Different from these existing approaches, we propose a novel class of invariants grounded on contextual predicates that can be effectively leveraged for linked-domain recommendation independent of the above assumptions. 
% 
%%While research areas such as Computer Vision have benefited from latent feature transfer for cross-domain problems owing to the presence of geometric invariants or motifs, it is much harder to find an accurate mapping of latent features across recommendation domains. While the shared content models ignore the similarities of the latent spaces, the shared user and item models rely on the existence of informative users and items respectively to map the latent factors of the source to the target domains. Co-ordinate transfer approaches, while not assuming any sharing, severely restrict the learned embedding spaces thereby reducing model learning capacity. In this work, we propose a novel class of invariants grounded on contextual predicates that can be effectively leveraged for linked-domain recommendation independent of the above assumptions.
%%Different from these existing approaches, we propose a novel class of invariants grounded on contextual predicates that can be effectively leveraged for linked-domain recommendation independent of the above assumptions. 
%
%\vspace{0.10in}
%\noindent \textbf{Solution Idea:} 
%Consider the task of restaurant recommendation for Visa cardholders. Consider the presence of a rich and dense source data (e.g., San Francisco Bay Area cardholder-restaurant transaction data) and a sparse target data (e.g., US cardholder-China restaurant transaction cross-border data or Californian Alpine County cardholder-restaurant transaction domestic data). Note that, Visa data has two kinds of data sparsity - transaction {\em density} that measures the number of transactions per cardholder, and transaction {\em volume} that captures the overall volume of cardholder-merchant transactions. While the first is important to build descriptive cardholder profiles, the second is equally important to build merchant profiles and learn the space of features that are critical for making suitable recommendations. We observe that each each restaurant visit of a cardholder is predicated on: 
%
%\noindent (i) transactional context (e.g., weekday or weekend, lunch or dinner, at home or at work, etc.), 
%
%\noindent (ii) historical context (e.g., budget-conscious or spendthrift cardholder, highly-rated or poorly rated restaurant, etc.), and 
%
%\noindent (iii) attributional context (e.g., restaurant cuisine type, cardholder's age group). 
%
%Our key hypothesis is the presence of critical combinations of these diverse contextual factors in both source and target domain, which, in turn, dictates where a cardholder eats. It enables us to cluster restaurants (e.g., restaurants that are generally visited for lunch, restaurants that serve Mexican food and are affordable, restaurants that are expensive and generally visited on weekend nights, etc.), as well as cardholders (e.g., cardholders who like to visit affordable Mexican restaurants for lunch, cardholders who like to visit expensive steak restaurants for dinner, etc.) by their specific values under these contextual combinations of these factors. Such an organization of the cardholder and restaurant spaces help us return high quality recommendations to cardholders, even when their data is sparse. The main linked-domain invariant for restaurant recommendation is the knowledge of which context combinations we should employ to cluster the cardholder and restaurant spaces, as well as the mapping of suitable restaurant clusters to cardholder clusters for recommendation.
%% Context-aware recommendation has attracted a lot of attention because of the impact of context on user behavior. The same user makes different choices with very different motivations depending on the contextual predicates, such as the spatio-temporal aspect (is it a weekday vs weekend, is the user at home or work etc.). Further restaurants are suited to certain types of context, for instance a bar is not suited for a midday meal when the user is at work. Our key hypothesis is that there critical combinations of contextual factors (such as time of the day and restaurant type) which dictate how a user behaves, and what restaurants are likely to be chosen under one specific combination (such as mid-day and bar) of these factors. 
%
%Although the clustering solution appears simple, there are an intractable number of such combinations to consider in reality. For example, restaurant cuisine is an important piece of contextual information. In the absence of well-defined restaurant cuisine data, as observed in Visa data, the name of a restaurant often provides clues to the restaurant cuisine. Since there may be over hundred such common words (e.g., {\em `pizza'}, {\em `taco'}, {\em `sushi'}, {\em `kobe'}, etc.) indicating the restaurant cuisine, the presence or absence of each of these words is a contextual factor in itself. Similarly, cardholder's spending behavior, restaurant's tip-receiving patterns, cardholder's preferred geographical locations at different times of the week, etc. all play an important role. Thus, a standard approach considering each combination separately is not feasible since the permutational space of these factors is massive.
%
%This motivates us to adopt a data-driven approach to learn which combinations of contexts are the driving factors behind restaurant visits, as well as to organize the cardholders and restaurants by their preferred values of these context combinations. The contextual factors are learned from the dense source domain while the cardholder-restaurant organization must be performed separately for both the source and target domains. Clearly, the former requires high volumes of dense and rich cardholder-restaurant interaction transaction data to facilitate the learning process. In order to determine the importance of a specific contextual combination, our model must observe these combinations manifest in the real data and hence form the necessary associations to extract and organize the cardholder-restaurant spaces with these factors. To this end, a highly dense, rich and refined dataset must be leveraged to fit the context learner, namely the source model which learns the set of important associations that form the key invariants in our application. This forms the core transfer aspect of our formulation. Additionally, we recognize and address the presence of differences across regions owing to cultural and geo-social factors using residual and distributional alignment. 
%
%%\vspace{10pt}
%%\textbf{NOTE} - The meta-model refers to the transferred set of layers which learn how to transform and extract the critical context combinations, and how to leverage these combinations to organize the user and restaurant embedding spaces (this constitues the overwhelming majority of the non-embedding model parameters, thus most of the learned aspects are reused across source and all target domains).
%
%
%\vspace{10pt}
%\noindent
%Our contributions can be summarized as follows:
%\vspace{5pt}
%%\begin{itemize}
%%\item 
%
%
%\noindent $\textbf{I.}$ \textbf{Contextual Invariance:} To the best of our knowledge, we are the first to consider contextual invariants for transfer learning in recommendation. While invariants are intuitive and well-defined for computer vision and other visual application tasks, it is not obvious what an accurate mapping of latent features across recommendation domain should embody. We propose a novel class of invariants grounded on contextual predicates that can be effectively leveraged for cross-domain recommendation. 
%
%\noindent $\textbf{II.}$ \textbf{Meta-Transfer Learning with Residual and Distributional Alignment:} Our main solution idea is to learn a single central meta-model which forms the key associations between different contextual factors that contribute to a restaurant visit. This central model cannot be learned separately for different data pockets since all of them do not provide the high quality dense data that is required to extract the important associations. We demonstrate that it is sufficient to learn the central model for the rich and dense source data only.   
%Cardholder and restaurant embeddings, as well as a residual/distributional adaptation component of the target domains accommodate the underlying differences across the different pockets. For example, restaurants in a major city like San Francisco in California will have a different pricing range than restaurants in a small town Elko in Nevada. It is known that restaurant pricing is an important contextual factor defining cardholders eating out activities. The central meta-learner will capture the importance of pricing, while the residual/distributional alignment will balance the region-specific variations.
%
%A related argument is to fit a joint model that simultaneously trains on both the source and target domains. Through extensive experimental results, we show that such an approach results in an inferior fit compared to meta-learner transfer followed by regional customization. 
%$$M_{T+S} \leq M_{T \rightarrow S}$$ In retrospect, joint training of source and target domains ($M_{T+S}$) is expected to be biased to the rich source data and thus less effective on the target domain compared to meta-transfer followed by annealing ($M_{T \rightarrow S}$).
%
%
%%\item 
%\noindent $\textbf{III.}$ \textbf{Rapid Prototyping via Annealing} A primary necessity of any industrial application is the ease of rapid prototyping for new data (data pockets or regions). Furthermore, models must also be updated at regular intervals in order to leverage recent cardholder and restaurant transaction activities, as well as to leverage the evolution of preferences of specific cardholders. Our approach is specifically suited to such a setting. We experimentally demonstrate that a small number of annealing epochs with the transferred meta-model can rapidly generate a high-performance recommender model for a new region or for cardholder/restaurant embedding updates. Intuitively, the contextual factors that are important to restaurant recommendation model do not change (e.g., pricing), thereby enabling the majority of our model to not require updates. On the other hand, a specific cardholder's financial situation may change, as evident from her recent transactions, and annealing on the new data is enough to capture this.
%
%
%%\item 
%\noindent $\textbf{IV.}$ \textbf{Dealing with Skew and Sparsity in Massive Volumes of Real-World data} Our solution has the ability to adapt to data pockets or regions with low volumes and/or low density. Recommender systems are known to be sensitive to two conditions - the overall volume of training data and per-user data density. These often limit a recommendation model from fitting to new data. In our solution, the meta-learner captures the most important combinations of context that dictate cardholder eating out decisions. This enables us to deal with low density of cardholder data. If a cardholder has a single transaction, the meta-learner knows what important combinations to look for to build a suitable representation for that cardholder, thus using her data more efficiently. We generate a heatmap that demonstrates how the tolerance of our model to low density and low volume targets is significantly improved by transferring the meta-model from the dense source domain.


==> SIGIR 2020 copy/model.tex <==

\section{Our Approach}
\label{sec:Model Description}

In this section, we describe a scalable, modular architecture to extract pooled contextual invariants and employ them to guide the learned user and item embedding spaces.

%In this section, we formalize cross-domain behavioral invariants via pooled contextual features and describe a scalable, modular architecture to extract and integrate them with the user and item embedding spaces. We predict likely interactions with the resulting context conditioned representations. Our formalization provides an automatic separation between the domain-specific embeddings and shared transformations grounded on context (meta). Subsequently, we develop meta transfer algorithms to adapt the shared components to sparse target domains in \Cref{subsec:Meta-Transfer}. 
\vspace{-4pt}
\subsection{Modular Architecture}
\label{subsec:Meta-Problem Formulation}

We achieve context-guided embedding learning via four synchronized neural modules with complementary semantic objectives:
%Our crucial intuition is the presence of behavioral invariants at the intersection of multiple contextual indicators, i.e., changing a single feature could drastically alter the likelihood of interaction, even with all other features held constant. Additive or linear models struggle to learn interaction effects \cite{nfm, mult-google}. Inspired by the past success of low-rank pooling models \cite{bilinear, mult-google}, we propose a low-rank multi-linear context representation to capture behavioral invariants.

%We leverage the contextual features of user interactions to describe these behavior patterns and learn representative user and item embedding spaces. This forms the core of our \textit{learn-to-learn} formulation, whereby we learn invariants on the dense source domain where they manifest in the observed user-item interactions. Critical invariants often appear at the intersection of multiple contextual indicators, e.g., changing a single context feature such as time of the day could drastically alter the likelihood of interaction even with other features held constant. Additive models struggle to learn interaction effects \cite{nfm}. Past work has even shown deep neural networks driven by linear transforms struggle to infer pooled or multiplicative factors \cite{mult-google}. Inspired by the past success of low-rank pooling models \cite{bilinear, mult-google}, we propose a multi-linear low rank pooled representation to capture invariant context transforms describing user behavior. Our architecture broadly consists of four components:
\begin{itemize}
\item \textbf{Context Module $\mathcal{M}^{1}$: } Extracts contextual invariants driving user-item interactions in the dense source domain.
\item \textbf{Embedding Modules $\mathcal{M}^{2}_{\mathcal{U}}, \mathcal{M}^{2}_{\mathcal{V}}$: } Domain-specific user and item embedding spaces ($\mathcal{U}$, $\mathcal{V}$ denote users and items).
\item \textbf{Context-conditioned Clustering Modules $\mathcal{M}^{3}_{\mathcal{U}}, \mathcal{M}^{3}_{\mathcal{V}}$:\\} $\mathcal{M}^{3}_{\mathcal{U}}$ and $\mathcal{M}^{3}_{\mathcal{V}}$ reorient the user and item embeddings with the contextual invariants extracted by $\mathcal{M}^{1}$ respectively.
\item \textbf{Mapping/Ranking Module $\mathcal{M}^{4}$: } Generate interaction likelihoods with the context-conditioned representations of $\mathcal{M}^{3}$.
\end{itemize}
Context-driven modules $\mathcal{M}^{1}$, $\mathcal{M}^{3}$, and $\mathcal{M}^{4}$ contain the meta-layers that are transferred from the dense to the sparse domains (i.e., shared or meta-modules), while $\mathcal{M}^{2}$ contains the domain-specific user and item representations. Our architecture provides a separation between the domain-specific $\mathcal{M}^{2}$ module and shared context-based transforms in the other modules (\Cref{fig:neural_1}).

%\noindent \textbf{The importance of low-rank pooling: } We extract the most informative contextual combinations to describe each interaction. Specially, the output of the context transform component is composed of \textit{n}-variate combinations of the contextual features. We enable data-driven selection of pooled \textit{n}-variate factors to address combinatorial explosion with growing context. Further, a tiny proportion of pooled combinations are expected to play a crucial role in the user-item interactions. Our approach facilitates their discovery by adaptive weighting the chosen set of multi-linear factors.
\vspace{-4pt}
\subsection{Module Description}
\label{subsec:Arch}
We now detail each module in our overall architecture.
%\begin{itemize}
%\item 

\subsubsection{Context Module $\mathcal{M}^1$} 

User-item interactions are driven by context feature intersections that are inherently \textit{multiplicative} (i.e., assumptions of independent feature contributions are insufficient), and are often missed in the Naive-Bayes assumption of additive models such as feature attention~\cite{nfm, mult-google}. Inspired by the past success of low-rank feature pooling~\cite{bilinear, mult-google}, our context module extracts low-rank multi-linear combinations of context to describe interactions and build expressive representations.
   % $$\mathcal{M}^1$ contains $n$ stacked layers, with each layer transforming an interaction $(u, \mathbf{c}, v)$ as follows$
The first layer in $\mathcal{M}^1$ transforms context $\mathbf{c}$ of an interaction $(u, \mathbf{c}, v)$ as follows: 
    \begin{equation}
    \mathbf{c}^{2} = \sigma(\underbrace{\mathbf{W}^2\mathbf{c} \oplus (\mathbf{b}^{2} \otimes \mathbf{c})}_{\text{Weighted linear transform}}) \hspace{10pt} \otimes \hspace{-20pt} \underbrace{ \mathbf{c}}_{\text{Element-wise interaction}}
    \end{equation}
   where $\oplus, \otimes$ denote element-wise product and sum, i.e.,
    \begin{equation}
    \mathbf{c}^{2}_{i} \propto \mathbf{c}_i \times \sigma(\mathbf{b}^2_{i}\mathbf{c}_i  + \sum_{j}\mathbf{W}^2_{ij} \mathbf{c}_j) 
    \vspace{-8pt}
    \end{equation}  
    Thus, $\mathbf{c}^{2}_{i}$ ($i^{th}\text{-component}$ of $\mathbf{c}^{2}$) incorporates a weighted bivariate interaction between $\mathbf{c}_{i}$ and other context factors $\mathbf{c}_j$, including itself. We then repeat this transformation over multiple stacked layers with each layer using the previous output:
	\begin{equation}    
    \mathbf{c}^{n} = \sigma(\mathbf{W}^{n}\mathbf{c}^{n-1} \oplus (\mathbf{b}^{n} \otimes \mathbf{c}^{n-1})) \otimes \mathbf{c}
    \label{cn}
    \end{equation}
 Each layer interacts \textit{n-variate} terms from the previous layer with $\mathbf{c}$ to form \textit{n+1-variate} terms. However, since each layer has only $|\mathbf{C}|$ outputs (i.e., low-rank), $\mathbf{W}^{n}$ prioritizes the most effective \textit{n-variate} combinations of $\mathbf{c}$ (typically, a very small fraction of all combinations is useful). We can choose the number of layers $n_{\mathbf{C}}$ depending on the required order of the final combinations $\mathbf{c}^{n_{\mathcal{C}}}$.
%     $$\mathbf({c}_{2})_{i} = \mathbf{c}_{i} \times \sum_{j = 1}^{|\mathbf{c}|}\mathbf{W}_{i,j}^{1} \mathbf{c}_{j} = \sum_{j = 1}^{|\mathbf{c}|}\mathbf{W}_{i,j}^{1} \mathbf{c}_{i}\mathbf{c}_{j}$$
    
    
 \begin{figure}[t]
    \centering
    \vspace{-4pt}
    \caption{Our overall recommender architecture, highlighting all four modules, $\mathcal{M}^1 \text{ to } \mathcal{M}^4$}
    \vspace{-3pt}
    \includegraphics[clip, trim=1cm 0.1cm 17cm 3.5cm, width=0.82\linewidth]{images/arch.png}
    \vspace{-28pt}
    \label{fig:neural_1}
    \end{figure}    
    
    
%    \textit{Hadamard Projector Pooling :} We propose a novel Hadamard Memory Network (HMN) to achieve low-rank multi-linear pooling with a more expressive projection strategy. We learn a set of \textit{k} memory blocks (each row or block is a Hadamard projector with the same length as the context vector, $|\mathbf{c}|$), given by $\mathbf{M} \in \mathbb{R}^{k \times |\mathbf{c}|}$. The first order transform of $\mathbf{c}$ is given by the concatentation of its $\mathit{k}$ Hadamard projections along each projector $\mathbf{M}_{i}$, followed by a feedforward operation to reduce the dimension of the concatenated projections to $|\mathbf{c}|$. The first-order transform is then element wise multiplied with the context vector to obtain the second order context vector. 
%    $$\mathbf{c}^{2} = \sigma(\mathbf{W}^{1}(\mathbf{c} \otimes \mathbf{M}_{1} \cdot \mathbf{c} \otimes \mathbf{M}_{2} \cdots \mathbf{c} \otimes \mathbf{M}_{k}) + \mathbf{b}^{1}) \otimes \mathbf{c}$$
%    where $\cdot$ denotes concatenation and $\otimes$ is the Hadamard product.
%    
%    The second order transform is now obtained by projecting and concatenating the second order context, and reduced to $|\mathbf{c}|$ dimensions by a second feedforward operation. The thid order context $\mathbf{c}^{3}$ is obtained by the element wise product of the second order transform with the first order context $\mathbf{c}$. 
%    
%    $$\mathbf{c}^{3} = \sigma(\mathbf{W}^{2}(\mathbf{c}^{2} \otimes \mathbf{M}_{1} \cdot \mathbf{c}^{2} \otimes \mathbf{M}_{2} \cdots \mathbf{c}^{2} \otimes \mathbf{M}_{k}) + \mathbf{b}^{2}) \otimes \mathbf{c}$$
%    
%    The resulting multi-linear pooling incorporates $\mathit{k}$-times the expressivity of the previous strategy, but also incurs a $k$-fold increase in computation and parameter costs. Note however, that the training costs are one-time (only on the dense source domain).
%    
    
    \textit{Multimodal Residuals for Discriminative Correlation Mining:}
  In addition to discovering the most important context combinations, we incorporate the information gain associated with pairwise interactions of context features \cite{featurepool}. For instance, the item cost feature is more informative in interactions where users deviate from their historical spending patterns. Specifically, pairs of signals (e.g., cost \& user history) enhance or diminish each other's impact, i.e.,
  \begin{equation}
   \mathbf{c}_{i} = \mathbf{c}_{i} + \Sigma_{j}\delta_{\mathbf{c}_i | \mathbf{c}_j}
   \label{mm1}
   \end{equation}
     We simplify \Cref{mm1} by only considering cross-modal effects across interactional, historical and attributional context, i.e., 
\begin{equation}
\delta_{\mathbf{c}_{\mathbf{I}}|\mathbf{c}_{\mathbf{H}}, \mathbf{c}_{\mathbf{A}}} = \underbrace{\mathbf{s_{\mathbf{I}}}}_{\text{Scaling factor}}  \hspace{-5pt}\otimes\hspace{7pt} \underbrace{\textit{tanh}(\mathbf{W}_{\mathbf{IH}} \times \mathbf{c}_{\mathbf{H}} + \mathbf{W}_{\mathbf{IA}} \times \mathbf{c}_{\mathbf{A}} + \mathbf{b}_{\mathbf{I}})}_{\text{Info gain/loss}}
\label{multimodal}
\end{equation}
 and likewise for $\delta_{\mathbf{c}_{\mathbf{H}}}$, $\delta_{\mathbf{c}_{\mathbf{A}}}$. Information gains are computed before $\mathbf{c}^{2}$ to cascade to further layers.
    
    
%    Note that we learn a scaling parameter $\mathbf{s}$ and weight $\mathbf{W}$  for each context mode. The above residual transforms are applied to raw context $\mathbf{c}$ before the first transformation layer to enable a cascading effect over the other layers.
    
    
% \noindent \textbf{Organize the User Embedding Space: }    
    
    
    
\begin{table}[t]
 \centering
 \caption{Modules and Learned Parameter Notations}
 \vspace{-12pt}
 \begin{tabular}{@{}p{0.32\linewidth}p{0.66\linewidth}@{}}
  \toprule
\textbf{Modules} & \textbf{Learned Parameters}\\  
  \midrule
     \multirow{1}{*}{\textbf{Domain-Specific} } &  \textbf{Embeddings} $\mathbf{e}_u \forall u \in \mathcal{U}_{\mathbf{D}}$, $\mathbf{e}_{v} \forall v \in \mathcal{V}_{\mathbf{D}}$\\
     ($\mathcal{M}^{2}_{\mathcal{U}}, \mathcal{M}^{2}_{\mathcal{V}}$) & \textbf{Biases} (only under explicit feedback) $s, s_u  \forall u \in \mathcal{U}_{\mathbf{D}}, s_{v} \forall v \in \mathcal{V}_{\mathbf{D}}$ \\
     \midrule
     
  \multirow{2}{*}{\textbf{Shared Modules}} &  $\mathcal{M}^{1}$ \hspace{2pt} \cref{cn} \hspace{3pt} $(\mathbf{W}^{i}, \mathbf{b}^{i}) \forall i = [1, \cdots , n_{\mathbf{C}}]$ \\
  
 &  $\mathcal{M}^{1}$ \hspace{2pt} \cref{multimodal} \hspace{3pt} $\mathbf{s}_{\mathbf{I}},  \mathbf{s}_{\mathbf{H}},  \mathbf{s}_{\mathbf{A}}; \mathbf{W}_{\mathbf{I}},  \mathbf{W}_{\mathbf{H}},  \mathbf{W}_{\mathbf{A}}$ \\
 \multirow{2}{*}{($\mathcal{M}^{1}$, $\mathcal{M}^{3}, \mathcal{M}^4$)} & $\mathcal{M}^{3}$ \hspace{2pt} \cref{link} \hspace{3pt} $\mathbf{W}_{\mathbf{C}\mathcal{U}}, \mathbf{W}_{\mathbf{C}\mathcal{V}}$\\
 
 & $\mathcal{M}^{3}_{\mathcal{U}}$ \cref{eq:ccr} \hspace{3pt}  $(\mathbf{W}^{i}_{\mathcal{U}}, \mathbf{b}^{i}_{\mathcal{U}}) \forall i = [1, \cdots , n_{\mathcal{U}}]$ \\
 
 & $\mathcal{M}^{3}_{\mathcal{V}}$ \cref{eq:ccr} \hspace{3pt}  $(\mathbf{W}^{i}_{\mathcal{V}}, \mathbf{b}^{i}_{\mathcal{V}}) \forall i = [1, \cdots , n_{\mathcal{V}}]$\\
 
 & $\mathcal{M}^{4}$ \hspace{2pt} \cref{sc} \hspace{3pt} $\mathbf{W}_{\mathbf{C}}, \mathbf{b}_{\mathbf{C}}$\\
  \bottomrule
 \end{tabular}
 \label{notation-table}
 \vspace{-14pt}
\end{table}    
    
    
    
    
    
    
    
    
    
\subsubsection{Context Conditioned Clustering $\mathcal{M}^3$}
We combine domain-specific embeddings $\mathcal{M}^2$ with the context combinations extracted by $\mathcal{M}^1$ to generate context-conditioned user and item representations. Specifically, we introduce the following bilinear transforms,
 \begin{align}
    \widetilde{\mathbf{e}_{u}} = \mathbf{e}_{u} \otimes  \sigma(\mathbf{W}_{\mathbf{C}\mathcal{U}} \times \mathbf{c}^{n_\mathbf{C}}) \\
    \widetilde{\mathbf{e}_{v}} = \mathbf{e}_{v} \otimes  \sigma(\mathbf{W}_{\mathbf{C}\mathcal{V}} \times \mathbf{c}^{n_\mathbf{C}})
    \label{link}
   \end{align}

%To achieve this organization of the embeddings, we backpropagate the extracted multi-linear context embeddings $\mathbf{c}^{n_\mathbf{C}}$ into the user embedding space and create context conditioned clusters of users for item ranking.

%   The user embedding space, $\mathbf{e}_u, u \in \mathcal{U}_{D}$, is organized to reflect the contextual preferences of users. The same motivation holds good for the item embedding space as well. 
 

%    The bilinear layers eliminate the irrelevant dimensions of the user and item embeddings to generate the conditioned representations $\widetilde{\mathbf{e}_{u}}$ and $\widetilde{\mathbf{e}_{v}}$. Further, bilinear transforms enable cross-domain \textit{dimensional-uniformity} of embeddings. Context features are analogously transformed and backpropagated into their user and item spaces.
    
%     The vectors $\widetilde{\mathbf{e}_{u}}$ and $\widetilde{\mathbf{e}_{i}}$ represent the context based clusters of users and items, based upon the $\mathit{n}$-variate context combinations in $\mathbf{c}^{n_\mathbf{C}}$.
    
%    \noindent $\textbf{D.}$ \textbf{Cluster Mapping - } 
    
where, $\mathbf{W}_{\mathbf{C}\mathcal{U}} \in \mathbb{R}^{{|\mathbf{e}_u| \times |\mathbf{C}}|}$, $\mathbf{W}_{\mathbf{C}\mathcal{V}} \in \mathbb{R}^{{|\mathbf{e}_v| \times |\mathbf{C}}|}$ are learned parameters that map the most relevant context combinations to the user and item embeddings. We further introduce $n_\mathcal{U}$ feedforward \textit{RelU} layers to cluster the representations,
\begin{align}
    \widetilde{\mathbf{e}_{u}}^{2} = \sigma(\mathbf{W}_{\mathcal{U}}^{2}\widetilde{\mathbf{e}_{u}} + \mathbf{b}_{\mathcal{U}}^{2})\\
    \widetilde{\mathbf{e}_{u}}^{n} = \sigma(\mathbf{W}_{\mathcal{U}}^{n}\widetilde{\mathbf{e}_{u}}^{n-1} + \mathbf{b}_{\mathcal{U}}^{n})
    \label{eq:ccr}
    \end{align}
Analogously, we obtain context-conditioned item representations $\widetilde{\mathbf{e}_{v}}^{2}, \cdots, \widetilde{\mathbf{e}_{v}}^{n_\mathcal{V}}$ with $n_\mathcal{V}$ feedforward \textit{RelU} layers. 

The bilinear transforms in \cref{link} introduce \textit{dimension alignment} for both $\widetilde{\mathbf{e}_{u}}^{n_\mathcal{U}}$ and $\widetilde{\mathbf{e}_{v}}^{n_\mathcal{V}}$ with the context output $\mathbf{c}^{n_{\mathbf{C}}}$. Thus, when $\mathcal{M}^3$ and $\mathcal{M}^1$ layers are transferred to a sparse target domain, we can directly backpropagate to guide the target domain user and item embeddings with the target domain interactions. 
    

    
%    The score for $u, v$ under context $\mathbf{c}$ (i.e., module $\mathcal{M}^4$) is reduced to just the dot product:
%        $$\hat{s}_{u, \mathbf{c}, v} = \widetilde{\mathbf{e}_{u}}^{n_\mathcal{U}} \cdot \widetilde{\mathbf{e}_{v}}^{n_\mathcal{V}}$$
%However in practice, the above loss function results in uninteresting low-variance samples dominating the learning process, resulting in slower convergence, less novelty and inaccurate user representations. In the next subsection, we tackle this challenge.
    
   

 
 \vspace{-3pt}
\subsection{Source Domain Training Algorithm}    
\label{subsec:Train}
In the source domain, we train all modules and parameters (\Cref{notation-table}) with ADAM optimization~\cite{adam} and dropout regularization~\cite{dropout}.

\subsubsection{Self-paced Curriculum via Contextual Novelty}
Focusing on harder data samples accelerates and stabilizes stochastic gradients \cite{hardsample1, active_bias}. Since our learning process is grounded on context, novel interactions display uncommon or \textit{interesting} context combinations. Let $\mathcal{L}_{(u, \mathbf{c}, v)}$ denote the loss function for an interaction $(u, \mathbf{c}, v)$. We propose an inverse novelty measure referred as the context-bias, $s_{\mathbf{c}}$, which is self-paced by the context combinations learned by $\mathcal{M}^1$ in \Cref{cn},
\begin{equation} 
   s_{\mathbf{c}} = \mathbf{w}_{\mathbf{C}} \cdot \mathbf{c}^{n_\mathbf{C}} + b_{\mathbf{C}}
   \label{sc}
\end{equation}
We then attenuate the loss $\mathcal{L}_{(u, \mathbf{c}, v)}$ for this interaction as,
\begin{equation}
	 \mathcal{L}_{(u, \mathbf{c}, v)}^{\mathbf{'}} =  \mathcal{L}_{(u, \mathbf{c}, v)} - s_{\mathbf{c}}
	 \label{eq:context_bias}
\end{equation}
The resulting novelty loss $\mathcal{L}_{(u, \mathbf{c}, v)}^{\mathbf{'}}$ decorrelates interactions \cite{decorrelate, var_reduction} by emulating variance-reduction in the \textit{n-variate} pooled space of $\mathbf{c}^{n_\mathbf{C}}$. $\mathcal{L}_{(u, \mathbf{c}, v)}^{\mathbf{'}}$ determines the user and item embedding spaces, inducing a novelty-weighted training curriculum focused on harder samples as training proceeds. We now describe loss $\mathcal{L}_{(u, \mathbf{c}, v)}$ for the explicit and implicit feedback scenarios.

%The novelty factor is self-paced by the $\mathbf{c}^{n_\mathbf{C}}$ transform generated by module $\mathcal{M}^1$. 
% 
%A practical example could be users visiting inexpensive restaurants in proximity to their common locations. Such examples can be predicted from context alone, and thus exhibit a stronger variance These examples constitute a large proportion of the training samples; fewer examples exhibit novel or diverse interests of users and the corresponding context. 



%\noindent $\textbf{E.}$ \textbf{Learn the Context Bias Component - } Finally,  The key intuition for this term is that some contexts are universally more likely to result in a restaurant visit in comparison to others. For instance, the bias to visit a highly rated restaurant in proximity to the user is expected to be significantly more than that of an average restaurant that is inaccessible to the user. To obtain this context bias score, we learn a simple dot-product layer,
%    $$s_{\mathbf{c}} = \mathbf{w}_{\mathbf{c}} \cdot \mathbf{c}^{n_\mathbf{C}} + b_{\mathbf{c}}$$


\subsubsection{Ranking our Recommendations}
In the \textit{implicit feedback setting}, predicted likelihood $\hat{s}_{(u, \mathbf{c}, v)}$ is computed with the context-conditioned embeddings (\Cref{eq:ccr}) and context-bias (\Cref{eq:context_bias}) as,
\begin{equation}
 \hat{s}_{(u, \mathbf{c}, v)} = \widetilde{\mathbf{e}_{u}}^{n_\mathcal{U}} \cdot \widetilde{\mathbf{e}_{v}}^{n_\mathcal{V}} + s_{\mathbf{c}}
 \end{equation}
 The loss for all the possible user-item-context combinations in domain $\mathbf{D}$ is,
 \begin{equation}
 \mathcal{L}_{\mathbf{D}} = \sum_{u \in \mathcal{U}_{\mathbf{D}}} \sum_{v \in \mathcal{V}_{\mathbf{D}}} \sum_{\mathbf{c} \in \mathbb{R}^{|\mathbf{c}|}} || \mathbb{I}_{(u, \mathbf{c}, v)} - \hat{s}_{(u, \mathbf{c}, v)} ||^{2}
 \label{basic_loss}
 \end{equation}
        where $\mathbb{I}$ is the binary indicator $(u, \mathbf{c}, v) \in \mathcal{T}_{\mathbf{D}}$. $\mathcal{L}_{\mathbf{D}}$ is intractable due to the large number of contexts $\mathbf{c} \in \mathbb{R}^{|\mathbf{c}|}$. We develop a negative sampling approximation for implicit feedback with two learning objectives - identify the likely item given the user and interaction context, and identify the likely context given the user and the item. We thus construct two negative samples for each $(u, \mathbf{c}, v) \in \mathcal{T}_{\mathbf{D}}$ at random: Item negative with the true context, $(u, \mathbf{c}, v^{-})$ and context negative with the true item, $(u, \mathbf{c}^{-}, v)$. $\mathcal{L}_{\mathbf{D}}$ then simplifies to,
\begin{equation}        
        \mathcal{L}_{\mathbf{D}} = \sum_{\mathcal{T}_{\mathbf{D}}} || 1 - \hat{s}_{(u, \mathbf{c}, v)} ||^{2} + \sum_{(u, \mathbf{c}, v^{-})} ||\hat{s}_{(u, \mathbf{c}, v^{-})} || + \sum_{(u, \mathbf{c}^{-}, v)} ||\hat{s}_{(u, \mathbf{c}^{-}, v)} || 
        \label{negsample_loss}
\end{equation}
        
\textit{In the explcit feedback setting}, we introduce two additional bias terms, one for each user, $s_{u}$ and one for each item, $s_v$. These terms account for user and item rating eccentricities (e.g., users who always rate well), so that the embeddings are updated with the relative rating differences. Finally, global bias $s$ accounts for the rating scale, e.g., 0-5 vs. 0-10. Thus the predicted rating is given as,

        \begin{equation}
        \hat{r}_{(u, \mathbf{c}, v)} = \widetilde{\mathbf{e}_{v}}^{n_\mathcal{V}} \cdot \widetilde{\mathbf{e}_{u}}^{n_\mathcal{U}} + s_{\mathbf{c}} + s_{u} + s_{v} + s
        \label{explicit_rating}
        \end{equation}
        Negative samples are not required in the explicit feedback setting,
        
        \begin{equation}
        \mathcal{L}_{\mathbf{D}}^{explicit} = \sum_{(u, \mathbf{c}, v, r_{uv}) \in \mathcal{R}_{\mathbf{D}}}  || r_{uv} - \hat{r}_{(u, \mathbf{c}, v)} ||^{2}
        \label{explicit_loss}
        \end{equation}
    
We now detail our approach to transfer the shared modules from the source domain to sparse target domains.
       
        
        
        
%        \begin{itemize}
%            \item \textbf{Merchant Negatives: } To avoid location bias in the learned embedding space, and explicitly capture the preferences of the user, we draw the negatives for each user in the spatial neighborhood of his positives, i.e., restaurants he could have visited but chosen not to. We construct a spatial index based on quad-trees to facilitate inexpensive sampling of negative merchant samples.
%            
%            \item \textbf{Context Negatives: } The context vector $\mathbf{c}$ is a binary vector denoting the attributional, historical and transactional context variables. Numerical attributes such as tip, spend, and distance are converted to quantile representations (\textit{1 of k-quantile}) to normalize for regional variations. To generative negative context samples, we hold the merchant and user constant, while varying the context vector in one of two ways - 
%%            \begin{itemize}
%%                \item\textit{A} \textit{Random Samples: } Each context value is randomly sampled among the set of transactional context variables such as time of interaction. Note that historical and attributional context is left unchanged since the merchant and user are fixed across negative context samples.
%%                
%%                \item\textit{B} \textit{Dirichlet Mixture Model: } Random sampling often results in unrealistic context variables that do not train the model since they are easy to distinguish. We propose a topic modeling approach to capture the co-occurrence patterns of the different transactional context variables across all users. Note that the value of each context variable in the transactional context represents a word (since each context is discretized with the \textit{1 of k-quantile} approach, there is a finite number of words), and a specific combination of transactional contexts is a short sentence, adopting the DMM terminology \cite{dmm}. Let us denote this set of \textit{'context topics'} by $\mathbf{T}_{\mathbf{c}}$.
%%                
%%                Each context vector $\mathbf{c}$ can then be denoted by a distribution $\textbf{P}_{\mathbf{c}}$ over the topics $\mathbf{T}_{\mathbf{c}}$. Our proposal is to then create an orthagonal projection of $\textbf{P}_{\mathbf{c}}$ in the context topic space and sample a random negative context from the resulting mixture of context topics.
%%            \end{itemize}
%        \end{itemize}
        
%        Loss function $\mathcal{L}_u$ is then given by the sum over the positive samples (transactions $\mathbf{T}_u$) and negative samples (sampled with the above procedure) corresponding to each user with a suitable scaling component $\mu$.  
%        
%        \item Explicit Feedback Scenario - 
%        $$
%        \hat{r}_{u, \mathbf{c}, v} = \widetilde{\mathbf{e}_{v}}^{n_\mathcal{V}} \cdot \widetilde{\mathbf{e}_{u}}^{3} + \mathbf{w}_{\mathbf{c}} \cdot \mathbf{c}^{n_\mathbf{C}} + b_{\mathbf{c}} + s_{u} + s_{v} + s
%        $$
%        
%        $$\mathcal{L}_u = \sum_{v \in \mathbf{R_{u}}}  || R_{u, \mathbf{c}, v} - \hat{r}_{u, \mathbf{c}, v} ||^{2}$$
%    \end{itemize}
%    
    
%\end{itemize}


==> SIGIR 2020 copy/model_adaptation.tex <==
\section{Transfer to Target Domains}
\label{subsec:Meta-Transfer}
Our formulation enables us to train the shared modules $(\mathcal{M}^1)_{\mathbf{S}}, (\mathcal{M}^3)_{\mathbf{S}}$ and $(\mathcal{M}^4)_{\mathbf{S}}$ on a dense source domain $\mathbf{S}$, and transfer them to a sparse target domain $\mathbf{T}$ to guide its embedding module $(\mathcal{M}^2)_{\mathbf{T}}$. Each shared module $\mathcal{M}$ encodes inputs $\mathbf{x}_{\mathcal{M}}$ to generate output representations $\mathbf{y}_{\mathcal{M}}$. In each domain $\mathbf{T}$, module $(\mathcal{M})_{\mathbf{T}}$ determines the joint input-output distribution, 
\begin{equation}
p_{\mathbf{T}}(\mathbf{y}_{\mathcal{M}}, \mathbf{x}_{\mathcal{M}}) = p_{\mathbf{T}}(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}}) \times p_{\mathbf{T}}(\mathbf{x}_{\mathcal{M}})
\label{joint}
\end{equation}
where the parameters of $(\mathcal{M})_{\mathbf{T}}$ determine the conditional $p_{\mathbf{T}}(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}})$ and $p_{\mathbf{T}}(\mathbf{x}_{\mathcal{M}})$ describes the inputs to module $(\mathcal{M})_{\mathbf{T}}$ in domain ${\mathbf{T}}$.
\textbf{Adaptation: }There are two broad strategies to adapt module $\mathcal{M}$ to a new target domain ${\mathbf{T}}$:
\begin{itemize}
\item \textbf{Parameter Adaptation:} We can retrain the parameters of module $\mathcal{M}$ for target domain $\mathbf{T}$ thus effectively changing the conditional $p_{\mathbf{T}}(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}})$ in \cref{joint}, or, 
\item \textbf{Input Adaptation:} Modify the input distribution $p_{\mathbf{T}}(\mathbf{x}_{\mathcal{M}})$ in each domain $\mathbf{T}$ without altering the parameters of $\mathcal{M}$.
\end{itemize}
We now explore module transfer with both types of adaptation strategies towards achieving three key objectives. First, the transferred modules must be optimized to be effective on each target domain $\mathbf{T}$. Second, we aim to minimize the computational costs of adapting to new domains by maximizing the reuse of module parameters between the source $\mathbf{S}$ and target domains $\mathbf{T}$. Finally, we must take care to avoid overfitting the transferred modules to the samples in the sparse target domain $\mathbf{T}$.
%\begin{itemize}
%\item \textbf{Target Domain Fit:} 
%\item \textbf{Minimize computational overheads per target:} 
%\item \textbf{Maximize shared parameters:} Maximize direct source-to-target parameter reuse for simplicity and efficiency.
%\item \textbf{Prevent Overfitting:} 
%\end{itemize}
\vspace{-4pt}
\subsection{Direct Layer-Transfer}
\label{subsec:DLT}
We first train all four modules on the source $\mathbf{S}$ and each target domain $\mathbf{T}$ in isolation. We denote these pre-trained modules as $(\mathcal{M}^i)_{\mathbf{S}}$ and $(\mathcal{M}^i)_{\mathbf{T}}$ for source domain $\mathbf{S}$ and a target domains $\mathbf{T}$ respectively. We then replace the shared modules in all the target domain models with the source-trained version, i.e., $(\mathcal{M}^{1})_{\mathbf{T}} = (\mathcal{M}^{1})_{\mathbf{S}}$,  $(\mathcal{M}^{3})_{\mathbf{T}} = (\mathcal{M}^{3})_{\mathbf{S}}$, $(\mathcal{M}^{4})_{\mathbf{T}} = (\mathcal{M}^{4})_{\mathbf{S}}$, while the domain-specific embeddings $(\mathcal{M}^{2})_{\mathbf{T}}$ are not changed in the target domains. Clearly, direct layer-transfer involves no overhead and trivially prevents overfitting. However, we need to adapt the transferred modules for optimal target performance, i.e., either adapt the parameters or the input distributions for the transferred modules in each target $\mathbf{T}$. We now develop these adaptation strategies building on layer-transfer.
%We replicate the domain-independent parameters and meta-modules in \Cref{notation-table} in the target domain, while the domain-specific parameters are pre-trained on the target data before layer-transfer. We can then obtain recommendation with the pre-trained user parameters and the transferred meta-layers.
% While direct layer-transfer has produced impressive results across a range of Computer Vision tasks \cite{layer-transfer-empirical},
%Our key objectives are two-fold - avoid overfitting to the sparse target domain while adapting the transferred layers, and scale laterally, i.e., adapt to new sparse target domains with minimal computational/storage overheads.
%
%While direct layer-transfer is highly scalable; there is significant scope to adapt the layers to the eccentricities of the target domain and optimize performance. We begin by introducing simulated annealing as a feasible adaptation strategy, and proceed to address its scalability concerns. 
%Note that the primary goal in the target domain is to learn representative user and merchant embeddings with a relatively low volume and density of transactional data. The key strength of our approach is to adapt the pre-determined contextual combinations, user and merchant clustering layers and  This enables our model to efficiently leverage the smaller volume of transactional data in the target domain. 
\begin{table*}[t]
 \centering
 \caption{Comparing the objectives in \Cref{subsec:Meta-Transfer} addressed by our meta-transfer approaches for sparse target domains}
 \vspace{-12pt}
 \begin{tabular}{@{}p{0.18\linewidth}p{0.16\linewidth}p{0.155\linewidth}p{0.21\linewidth}p{0.22\linewidth}@{}}
  \toprule
     \textbf{Adaptation Method} & \textbf{Target Adaptation} & \textbf{Resists Overfitting} & \textbf{Extra compute per target} & \textbf{Extra parameters per target}  \\
  \midrule
\textbf{Layer-Transfer} & No adaptation & Yes, trivially & None & None, module params reused\\
%\midrule
\textbf{Simulated Annealing} & Yes, module params & Yes, stochastic & All parameter updates & All module params (~\Cref{notation-table})\\
%\midrule
%\textbf{} & Yes, adapts module inputs & No & Residual layer updates & Residual layers only\\
\textbf{Regularized Residuals} & Yes, module inputs & Yes, via distributional consistency & Residual layer updates with distributional regularization & Residual layer parameters\\
  \bottomrule
 \end{tabular}
 \label{methods}
 \vspace{-12pt}
\end{table*}
\vspace{-4pt}
\subsection{Simulated Annealing}
\label{subsec:anneal}
Simulated annealing is a stochastic local-search algorithm, that implicitly thresholds parameter variations in the gradient space by decaying the gradient learning rates~\cite{anneal}. As a simple and effective adaptation strategy, we anneal each transferred module $\mathcal{M}$ in the target domain $\mathbf{T}$ with exponentially decaying learning rates to stochastically prevent overfitting: 
\begin{equation}
(m)_{b+1} = (m)_{b} + \eta_{b}\frac{\partial\mathcal{L}_{b}}{\partial m}, \hspace{3pt} \eta_{b} = \eta_{0}e^{-\lambda b}
\label{eq:anneal}
\end{equation}
where $m$ denotes any parameter of transferred module $\mathcal{M}$ (\Cref{notation-table}), $b$ is the stochastic gradient batch index in the target domain and $\mathcal{L}_b$ is the batch loss for batch $b$. Our annealing strategy stochastically generates a robust parameter search schedule for transferred modules $\mathcal{M}^{1}, \mathcal{M}^{3}, \mathcal{M}^{4}$, with $\eta_{b}$ decaying to zero after one annealing epoch. While annealing the transferred modules, domain-specific module $\mathcal{M}^2$ is updated with the full learning rate $\eta_{0}$.
Clearly, annealing modifies the conditional $p_{\mathbf{T}}(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}})$ in \cref{joint} via parameter adaptation. However, annealing transferred modules in each target domain is somewhat expensive, and the annealed parameters are not shareable, thus causing scalability limitations in the one-to-many transfer scenario. We now develop a lightweight residual adaptation strategy to achieve input adaptation without modifying any shared module parameters in the target domains to overcome the above scalability challenges.
%We highlight a few relevant insights regarding layer perturbation- 
%
%\begin{itemize}
%    \item \textit{Residual Shifting of Context Combinations} - The notion of residual learning was provided impetus by the landmark ResNet approach to image representation \cite{resnet}. We learn a perturbation function on the latent representation of transferred layers, rather than a direct transformation. This is a particularly intuitive approach in our setting since user preferences and context-sensitivity vary across regions by small margins, although we broadly expect similar combinations to play a critical role in determining user-item interactions. Thus residual learning is applied to adapt the meta layers and enable cross-domain user preference variations.
%    
%    \item \textit{Hadamard Scaling} - Our approach is predicated on maintaining embedding consistency across domains of recommendation. Note from our earlier equations that both, the transformed user $\widetilde{\mathbf{e}_{u}}$ and item embeddings $\widetilde{\mathbf{e}_{i}}$ are obtained via element-wise combinations with the transformed context $\mathbf{c}^n$. 
    
%    Thus to maintain dimensional consistency, we restrict the scaling method to Hadamard-based transforms. Effectively, this permits different dimensions to be re-weighted but not to be changed, i.e., the semantics of dimensions are consistent though their importance may vary depending on the domain.
%    
%    \item \textit{Adversarial Learning for Distributional Regularization} - We view the distributional regularization problem as one of cluster-level consistency across domains. While the residual shifting and hadamard scaling of embeddings ensure flexible adaptation, it is necessary to maintain the same broad overall set of user and merchant clusters. Note the key distinction between older work and our proposal, we do not restrict the joint distribution of users with varying preferences, but rather the conditional, i.e., given a user has a certain preference which matches that of some set of users in the source domain, her embedding representation matches the corresponding cluster or dense patch of the source embedding space. Applying regularization ensures smooth transfers of cross-cluster mapping while also smoothing (regularizing) noisy embedding spaces in sparse domains.
%\end{itemize}
\vspace{-4pt}
\subsection{Distributionally Regularized Residuals}
\label{subsec:DRR}
% \subsubsection{adapt:anneal}%Adaptation approaches that modify $p(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}})$ must alter module parameters in each new target domain, resulting in scalability challenges. Instead, w
We now develop an approach to reuse the source modules with target-specific input adaptation, thus addressing the scalability concerns of parameter adaptation methods.
\subsubsection{Enabling Module Reuse with Residual Input  Adaptation}
In \cref{joint}, module $\mathcal{M}$ implements the conditional $p(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}})$. To maximize parameter reuse, we share these modules across the source and target domains (i.e., $p_{\mathbf{T}}(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}}) = p_{\mathbf{S}}(\mathbf{y}_{\mathcal{M}} | \mathbf{x}_{\mathcal{M}})$) and introduce target-specific residual perturbations to account for their eccentricities~\cite{classifier-adap} by modifying the input distributions $p_{\mathbf{T}}(\mathbf{x}_{\mathcal{M}})$. Target-specific input adaptation overcomes the need for an expensive end-to-end parameter search. Our adaptation problem thus reduces to learning an input modifier for each target domain $\mathbf{T}$ and shared module $\mathcal{M} \in [\mathcal{M}^1, \mathcal{M}^3, \mathcal{M}^4]$, i.e., for each $\mathcal{M}, \mathbf{T}$.
%\begin{equation}
%x_{\mathcal{M}}^{\mathbf{T}} = f_{\mathcal{M}}^{\mathbf{T}}(x_{\mathcal{M}})
%\end{equation}
Residual transformations enable the flow of information between layers without the gradient attenuation of inserting new non-linear layers, resulting in numerous optimization advantages~\cite{resnet}. Given the module-input $\mathbf{x}_{\mathcal{M}}$ to the shared module $\mathcal{M}$ in target domain $\mathbf{T}$, we learn a module and target specific residual transform:
\begin{equation}
\mathbf{x}_{\mathcal{M}} = \mathbf{x}_{\mathcal{M}} + \delta_{\mathcal{M}, \mathbf{T}}(\mathbf{x}_{\mathcal{M}})
\end{equation}
%In this subsection, we describe the residual adaptation of each context transformation layer.
%In the most general form (since we have multiple approaches to perform multi-linear context pooling),
%
%$$\mathbf{c}^{n} = \mathit{f}^{n}(\theta_{c}^{n-1}, \Theta_{c}; \mathbf{c}^{n-1})$$
%
%where $\theta_{c}^{n-1}$ denotes the layer-specific parameters of the $n-1^{th}$ layer while $\Theta_{c}$ denotes the parameters shared by all transform layers, such as the Hadamard memory vectors $\mathbf{M}_{k}$. 
%
%To enable lateral scaling across many domains or regions, we mustn't alter the core layer parameters, since this would result in a model-space explosion. Instead we propose only to perturb the model transforms with a domain-specific residual function, much in the spirit of ResNet \cite{resnet}.
%Consider the above layer transformation for $\mathbf{c}^{n}$, we do not modify the source-learned parameters $\theta_{c}^{n}, \Theta_{c}$ (let us denote the source domain by $\mathbb{S}$ and the target domain by $\mathbb{T}$). We learn a target specific residual function $\delta_{f}^{n}$ corresponding to the $n^{th}$ layer as a function of the layer transformed output $\mathit{f}^{n}$. Thus the adapted version is as follows,
%
%$$\mathbf{c}^{n} = \mathit{f}^{n}(\theta_{c}^{n}, \Theta_{c}; \mathbf{c}^{n-1}) + \delta_{f}^{n}(\mathit{f}^{n}(\theta_{c}^{n-1}, \Theta_{c}; \mathbf{c}^{n-1}))$$
%Note that context shortcut connections are not modified in the adaptation process. Shortcut connections of the form $\mathbf{c}^{n} \oplus g(\mathbf{c})$ should be interpreted as part of the source-learned transform, i.e., $$\mathbf{c}^{n} = \mathit{f}^{n}(\theta_{c}^{n-1}, \Theta_{c}; \mathbf{c}^{n-1}, \mathbf{c})$$ and provided as input to the residual function $\delta_{f}^{n}$. 
The form of the residual function $\delta$ is flexible. We chose a single non-linear residual layer, $\delta(\mathbf{x}) = tanh(\mathbf{W}\mathbf{x} + \mathbf{b})$. We can intuitively balance the complexity and number of such residual layers.
Note that the above residual strategy involves learning the $\delta_{\mathcal{M}, \mathbf{T}}$ layers with feedback from only the sparse target domain samples. To avoid overfitting, we need a scalable regularization strategy to regularize $p_{\mathbf{T}}(\mathbf{x}_{M})$ in each target domain. We propose to leverage the source input distribution as a common baseline for all the target domains, i.e., intuitively, $p_{\mathbf{S}}(\mathbf{x}_{M})$ provides a common center for each $p_{\mathbf{T}}(\mathbf{x}_{M})$ in the different target domains. This effectively anchors the residual functions and prevents overfitting to noisy samples.
%. We also note that a residual perturbation need not be learned for each context transform layer. Instead 
%
% We now revisit the two embedding transform equations responsible for organizing the target user and merchant embedding spaces,
% 
% $$\widetilde{\mathbf{e}_{u}} = \mathbf{e}_{u} \otimes \mathbf{c}^{n}$$
% $$\widetilde{\mathbf{e}_{i}} = \mathbf{e}_{i} \otimes \mathbf{c}^{n}$$
% 
%Hadamard scaling and shifting operations are applied to the feedforward layers on $\widetilde{\mathbf{e}_{u}}$, $\widetilde{\mathbf{e}_{i}}$ which jointly compute the outputs $\widetilde{\mathbf{e}_{u}}^{2}$ and $\widetilde{\mathbf{e}_{i}}^{2}$ respectively. The residual shift is identical to the context residuals and can be applied to one or both feedforward outputs $\widetilde{\mathbf{e}_{u/i}^{n}}$. The Hadamard transform requires an additional scaling vector $\mathbf{w}_{\otimes}^{n}$. The overall transform is as follows - 
%
%$$\widetilde{\mathbf{e}_{u/i}^{n}} = \sigma(\widetilde{\mathbf{W}_{\mathcal{U}/\mathcal{I}}^{n}} \hspace{2pt} (\widetilde{\mathbf{e}_{u/i}^{n-1}} \otimes \mathbf{w}_{\otimes}^{n}) + \widetilde{\mathbf{b}^{n}}) + \delta^{n}(.)$$
%\begin{algorithm}
%\caption{DRR Algorithm}\label{alg:inference}
%\begin{algorithmic}[1]
%%\Require{Nodes $x_1 \ldots x_n$, Class labels $y_1 \ldots y_n$, $y_i \in \{-1,1\}$, Adjacency matrix of each induced GCN $A_c, A_{ts}, A_{as}, A_r$}
%%\Ensure{boosted score $h_b(x_i) \forall i \in [1, n]$}
%\Function{Forward}{$\mathbf{X}, \mathbf{Y}, \{A_i\}_{S_i \in \mathbf{S}}$}
%  \State $\mathbf{H}_{b} \gets \mathbf{0} $
%    \For{$\mathbf{R} \in \mathcal{R}$}
%    \State $\{ \mathbf{Z}_i^K \}_{S_i \in \mathbf{R}} \gets Conv(\mathbf{X}, \{ A_i \}_{S_i \in \mathbf{R}})$
%    
%    %\State \Comment{Equation  \ref{eq:contrast}, \ref{eq:similar}, \ref{eq:reflexive}}
%
%    \State $\mathbf{H}_\mathbf{R} =\sum_{{S_i} \in \mathbf{R}} \mathbf{Z}_i^{K} \times \widetilde{\mathbf{W}}_i$  % \Comment{Equation \ref{eq:score}}
%    %\State $h_s = merge(h_{as}, h_{ts})$ \Comment{Equation \ref{eq:merge}}
%    \State $ \mathbf{e}_{\mathbf{R}} \gets \exp({-\mathbf{Y} \odot \mathbf{H}_{b}})$
%    \State \Comment{ $\odot \rightarrow \textit{Hadamard Product}$}
%  \State $\alpha_\mathbf{R} \gets \dfrac{1}{2} \ln{\dfrac{\sum \mathbf{e}_{\mathbf{R}} \odot \mathbbm{1}\left((\mathbf{Y} \odot \mathbf{H}_{\mathbf{R}}\right) > 0)}{\sum \mathbf{e}_{\mathbf{R}} \odot \mathbbm{1}\left((\mathbf{Y} \odot \mathbf{H}_{\mathbf{R}}) < 0 \right) }}$
%    \State \Comment{$\sum \rightarrow \textit{reduce-sum}$}
%      \State \Comment{$\mathbbm{1}(.) \rightarrow \textit{element-wise Indicator function}$}
%  \State    $\mathbf{H}_{b} \gets \mathbf{H}_{b} + \alpha_\mathbf{R} * \mathbf{H}_{\mathbf{R}}$ \Comment{Update boosted GCN}
%%    \State $ w_{i,r} \gets \exp^{-y_i * h_{cs}(x_i)}$
%%  \State    $\alpha_r \gets \dfrac{1}{2} \lnb{\dfrac{\sum\limits_{y_i = h_s(x_i)} w^{i,c}}{\sum\limits_{y_i \neq h_s(x_i)} w_{i,c} }}$
%%    \State $h_{b}(x_i) \gets h_{cs}(x_i) + \alpha_r * h_{cs}(x_i)$\Comment{Final Boosted GCN}
%    \EndFor
%    \State \Return $\mathbf{H}_{b}$, $ \{ \mathbf{H}_{R} \}_{\mathbf{R} \in \mathcal{R}}$, $\{ \mathbf{Z}_{i}^{K} \}_{S_i \in \mathbf{S}}$
%    %\State \Comment{Boosted scores, Relation level scores,}
%    %\State \Comment{Each GCN vertex representations}
%\EndFunction
%\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}[tbh]
%\caption{MMT-Net Training}\label{alg:training}
%\begin{algorithmic}[1]
%\Require{Input Context Features, Acceptance labels for each sample, $\mathbf{Y}$ }
%\Ensure{Trained Model i.e. Weight parameters $W_{i}^{1} \ldots W_{i}^{k}, S_i \in \mathbf{S}, \forall k \in [1, K]$ and transform parameters $\widetilde{W}_i$, $S_i \in \mathbf{S}$ }
%%\Ensure{Trained Model i.e. Weight parameters $W_{\mathbf{S}}^{1} \ldots W_{\mathbf{S}}^{k}, \mathbf{S} \in %\mathbb{S} $ and transform parameters $\widetilde{W}_v$, $v \in \mathbf{V}$ }
%%\While{ $not$ $converged$}
%%\For{$t\gets0 to \textit{num_epochs}$ }
%\For{$t \gets 1$ to $\textit{num-epochs}$}
%    \State $\mathbf{H}_b, \{ \mathbf{H}_{R} \}_{\mathbf{R} \in \mathcal{R}}, \{ \mathbf{Z}^{K}_{i} \}_{S_i \in \mathbf{S}}$ $\gets \textsc{Forward}(X, Y, \{ A_i \}_{S_i \in \mathbf{S}})$
%    \State \Comment{\Cref{alg:inference}}
%    \For{ $\mathbf{R} \in \mathcal{R}$}
%
%        \State $\mathcal L_b \gets \sum \exp({-\mathbf{Y} \odot \mathbf{H}_b}) + \gamma_1 \mathcal L_1(.) + \gamma_2 \mathcal L_2(.)$
%    \State \Comment{$\sum \rightarrow \textit{reduce-sum}$}
%  \State \Comment{$\odot \rightarrow \textit{Hadamard Product}$}
%        \State $\mathcal L_{\mathbf{R}} \gets 0$
%        \For{ $S_i \in \mathbf{R}$}
%        \State $\mathcal L_{i} \gets \sum \exp({-\mathbf{Y} \odot \mathbf{H}_\mathbf{R}})$
%                    %\State \Comment{$\sum \rightarrow \textit{reduce-sum}$}
%    \State $\mathcal L_{\mathbf{R}} \gets \mathcal L_{\mathbf{R}} + \mathcal L_{i} + \frac{1}{2}\sum_{S_i' \neq S_i}\lvert\lvert \mathbf{Z}_{i}^K - \mathbf{Z}_{i'}^K \lvert\lvert $
%    \EndFor
%    \State $\mathcal L_b \gets \mathcal L_b + \lambda(t) \mathcal L_{\mathbf{R}}$
%    \State    $W_i^{k} \gets  W_i^{k} + \eta_{\textsc{adam}} \frac{\partial \mathcal L_b}{\partial W_i^{k}} $ \Comment{$\forall k \in [1, K], \forall S_i \in \mathbf{R}$}
%     \State    $\widetilde{W}_i \gets  \widetilde{W}_i +  \eta_{\textsc{adam}} \frac{\partial \mathcal L_b}{\partial \widetilde{W}_i}$ \Comment{$\forall S_i \in \mathbf{S}$}
%    \EndFor
%\EndFor
%\end{algorithmic}
%\end{algorithm}
\subsubsection{Scalable Distributional Regularization for Residual Learning}
\label{subsec:encoder}
Learning pairwise regularizers between each $p_{\mathbf{T}}(\mathbf{x}_{M})$ and the source input distribution $p_{\mathbf{S}}(\mathbf{x}_{M})$ is not a scalable solution. Instead we train a universal regularizer for each module $\mathcal{M}$ on the source $p_{\mathbf{S}}(\mathbf{x}_{\mathcal{M}})$, and apply this pre-trained regularizer when we fit the residual layers $\delta_{\mathcal{M}, \mathbf{T}}$ in each target domain. Our key intuition is to treat the regularizer for the inputs of each module $\mathcal{M}$ as a one-class decision-boundary~\cite{adv-novelty}, described by the dense regions in the source domain, i.e., $p_{\mathbf{S}}(\mathbf{x}_{\mathcal{M}})$. Unlike adversarial models that are trained with both the source and target distributions~\cite{adv-dist}, we propose a novel approach to learn distributional input regularizers for the shared modules with just the source domain inputs.
% $\mathbf{x}_{\mathcal{M}}^{\mathbf{T}} \sim p_{\mathbf{T}}(\mathbf{x}_{\mathcal{M}} + \delta^{\mathbf{T}}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}}))$.
%Maintaining cross-domain distributional consistency of the input representations $\mathbf{x}_{\mathcal{M}}$ to module $\mathcal{M}$ is involves fitting a  While generative adversarial approaches have proven effective at imitating distributions in the generated space~\cite{adv-dist, gan1}, adversarial models are trained jointly with both the source and target representations. In our application, 
For each shared module, the learned regularizer anticipates hard inputs across the target domains without accessing the actual samples. We introduce a variational encoder $\mathcal{E}_{\mathcal{M}}$ with RelU layers to map inputs $\mathbf{x}_{\mathcal{M}} \sim p_{\mathbf{S}}(\mathbf{x}_{\mathcal{M}})$ to a lower-dimensional reference distribution $\mathbf{N}(0, \mathbb{I})$~\cite{vae-tutorial}. Simultaneously, we add poisoning model $\mathcal{P}_{\mathcal{M}}$ to generate sample-adaptive noise $\mathcal{P}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}})$ to generate poisoned samples $\widetilde{\mathbf{x}}_{\mathcal{M}} = \mathbf{x}_{\mathcal{M}} + \mathcal{P}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}})$ with the source domain inputs $\mathbf{x}_{\mathcal{M}} \sim p_{\mathbf{S}}(\mathbf{x}_{\mathcal{M}})$. We define the encoder loss to train $\mathcal{E}_{\mathcal{M}}$ as follows:\vspace{1pt}
% so that $\widetilde{\mathbf{x}}_{\mathcal{M}} \sim \widetilde(p_{\mathbf{S}})$
\begin{equation}
\mathcal{L}_{\mathcal{E}_{\mathcal{M}}} = \infdiv{p(\mathcal{E}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}}))}{\mathbf{N}(0, \mathbb{I})} - \infdiv{p(\mathcal{E}_{\mathcal{M}}(\widetilde{\mathbf{x}}_{\mathcal{M}}))}{\mathbf{N}(0, \mathbb{I})}
\label{e_loss}
\end{equation}
where $\infdiv{p}{q}$ denotes the \textit{KL-Divergence} of distributions $p$ and $q$. The above loss enables $\mathcal{E}_{\mathcal{M}}$ to separate the true and poisoned samples across the $\mathbf{N}(0, \mathbb{I})$ hypersphere in its encoded space. Since $\mathcal{E}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}})$ involves a stochastic sampling step, gradients can be estimated with a \textit{reparametrization trick} using random samples to eliminate stochasticity in the loss $\mathcal{L}_{\mathcal{E}_{\mathcal{M}}}$\cite{vae-tutorial}. Conversely, the loss for our poisoning model $\mathcal{P}_{\mathcal{M}}$ is given by,
\vspace{-2pt}
\begin{equation}
\mathcal{L}_{\mathcal{P}_{\mathcal{M}}} = \infdiv{p(\mathcal{E}_{\mathcal{M}}(\widetilde{\mathbf{x}_{\mathcal{M}}}}{\mathbf{N}(0, \mathbb{I})}  - \log ||\mathcal{P}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}})||
\label{p_loss}
\end{equation}
Note the first term in \Cref{p_loss} attempts to confuse $\mathcal{E}_{\mathcal{M}}$ into encoding poisoned examples $\widetilde{\mathbf{x}_{\mathcal{M}}} = \mathbf{x}_{\mathcal{M}} + \mathcal{P}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}})$ in the reference distribution, while the second term prevents the degenerate solution $\mathcal{P}_{\mathcal{M}}(\mathbf{x}_{\mathcal{M}}) = 0$. \Cref{e_loss} and \Cref{p_loss} are alternatingly optimized, learning sharper decision boundaries as training proceeds. With the above alternating optimization, we pre-train the encoders $\mathcal{E}_{\mathcal{M}}$ for the three shared modules on the source domain $\mathbf{S}$. We now describe how we use these encoders to regularize the residual layers $\delta_{\mathcal{M}, \mathbf{T}}$ in each target domain $\mathbf{T}$.
\subsubsection{Distributionally-Regularized Target Loss}
For each target domain $\mathbf{T}$, we learn three residual layers for the module inputs $\mathbf{c}^{2}$, $\widetilde{\mathbf{e}_{u}}$ and $\widetilde{\mathbf{e}_{v}}$ for $\mathcal{M}_1, \mathcal{M}_3^{\mathcal{U}}, \mathcal{M}_3^{\mathcal{V}}$ respectively. The inputs to $\mathcal{M}_{4}$, $\widetilde{\mathbf{e}_{u}}^{n_{\mathcal{U}}}$,  $\widetilde{\mathbf{e}_{v}}^{n_{\mathcal{V}}}$  are not adapted. Thus, we learn three variational encoders in the source domain as described in \Cref{subsec:encoder}, $\mathcal{E}_{\mathbf{C}}, \mathcal{E}_{\mathcal{U}}$ and $\mathcal{E}_{\mathcal{V}}$ for $\mathbf{c}^{2}$, $\widetilde{\mathbf{e}_{u}}$ and $\widetilde{\mathbf{e}_{v}}$ respectively.
Consider target interactions $(u, \mathbf{c}, v) \in \mathcal{T}_{\mathbf{T}}$. In the absence of distributional regularization, the loss is identical to the first term in \Cref{negsample_loss}. However, we now apply regularizers to $\mathbf{c}^{2}$, $\widetilde{\mathbf{e}_{u}}, \widetilde{\mathbf{e}_{v}}$:
\begin{equation}
\begin{split}
\mathcal{L}^{reg}_{\mathcal{T}_{\mathbf{T}}} &= \mathcal{L}_{\mathcal{T}_{\mathbf{T}}} + \infdiv{p_{\mathbf{T}}(\mathcal{E}_{\mathcal{U}}({\widetilde{\mathbf{e}_{u}}}))}{\mathbf{N}(0, \mathbb{I})} + \\ & \infdiv{p_{\mathbf{T}}(\mathcal{E}_{\mathcal{V}}({\widetilde{\mathbf{e}_{v}}}))}{\mathbf{N}(0, \mathbb{I})} + \infdiv{p_{\mathbf{T}}(\mathcal{E}_{\mathbf{C}}({\mathbf{c}^{2}}))}{\mathbf{N}(0, \mathbb{I})}
\label{regloss}
\end{split}
\end{equation}
Again, the gradients can be estimated with the \textit{reparametrization trick} on the stochastic \textit{KL-divergence} terms\cite{vae-tutorial} as in \Cref{subsec:encoder}. The residual layers are then updated as in \Cref{subsec:Train} with $\mathcal{L}^{reg}_{\mathcal{T}_{\mathbf{T}}}$ replacing the first term in \Cref{negsample_loss}.
%\begin{figure}[hbtp]
%    \centering
%    \includegraphics[width=0.9\linewidth]{adv_image.png}
%    \caption{Our Approach to Efficient Distributional Regularization}
%    \label{fig:neural_1}
%\end{figure}
% The above three components are trained in tandem, the objective of the encoding and decoding layers is to reconstruct the source embedding $\widetilde{{e}_{u}^{n}}$ with the least error, the objective of the poisoning layer is to generate the most confusing variants of the encoded version and finally the objective of the classifier is to distinguish the poisoned and encoded source embedding variants. As training proceeds, the poisoning mechanism generates increasingly harder examples while the classifier learns a sharper decision boundary for the dense source regions. At the end of the training process, the classifier is frozen and used as a distributuional regualizer to penalize the outlier embeddings in each target domain. We thus obtain an inexpensive one-time solution in contrast to adversarial learning on each target domain separately.
%We employ variational encoder $\mathcal{E}$ with RelU layers to fit the source embeddings to the reference distribution $\mathcal{N}(0, I)$ in a lower dimensional space. Our objective is to enable $\mathcal{E}$ to anticipate noise or outlier regions encountered in the target domains and penalize them. Towards this goal, the encoders attempts to diverge poisoned samples away from the reference distribution $\mathcal{N}(0, I)$. Thus the encoder objective is given by,
%
%$$\mathcal{O}_{\mathcal{E}} = \mathbf{KL}(\mathbf{N}|\mathbf{N}(0,1)) - \mathbf{KL}(\mathbf{P}|\mathbf{N}(0,1))$$
%
%$$\theta_{\mathcal{E}} = \argmax_{\theta} \mathcal{O}_{\mathcal{E}}$$
%
%The objective of the poisoning model or corruption model $\mathcal{C}$ follows directly from the above; it adds residual noise to the positive class to produce negative samples. These negative samples must confuse the Variational Encoder and hence minimize KL divergence from the reference distribution $\mathbf{N}(0,1)$. We generate the negative class as follows - 
%
%$$\mathbf{N} = \mathbf{P} + \mathbf{\delta}\mathbf{P} $$
%
%where $\mathbf{\delta}\mathbf{P} = \mathcal{C}(\mathbf{P})$. The corruption model is trained with the following objective, aiming to confuse the encoder into placing poisoned samples in the reference distribution,
%%
%$$\theta_{\mathcal{C}} = \argmin_{\theta} \mathcal{O}_{\mathcal{E}}(\mathbf{N} = \mathbf{P} + \mathcal{C}(\mathbf{P})$$
%%
%An important inference is that the training process may result in the corruption model learning to produce low magnitude noise. We need to explicitly penalize such an outcome -
%
%$$\theta_{\mathcal{C}} = \argmin_{\theta} (\mathcal{O}_{\mathcal{E}} - \log || \mathcal{C}(\mathbf{P})||) $$
%
%As a result the corruption model is incentivized to discover non-zero solutions to corrupt the positive (or source) embeddings.
%
%%\emph{A note on overfitting to small training datasets: }A long-standing challenge in machine learning is the generalization aspect for models that are trained on relatively small volumes of data. In meta-learning, this problem appears in the context of model adaptation. Models adapted to tiny datasets can fit noise to the base learner and thus fail to generalize well. Our adversarial distribution regularizer is a solution to this challenge, since
%
%The receptive regions in the source domain are leveraged to maintain a similar overall structure in the target space for each module input $\mathbf{x}_{\mathcal{M}}$. We thus avoid undesirable residuals that may result from overfitting to sparse target samples and diminish our module reusability.
%\subsection{A Flexible Curriculum for Model Adaptation}
%
%The training curriculum or schedule in our transfer process describes the order of training samples in the target domain when adaptation is performed. A measure of sample hardness can be estimated by using a proxy such as the gradient magnitude \cite{maml} or training loss on each target transaction. The harder samples are then stratified and re-sampled for faster model adaptation.
%\section{System Description}
%
%\begin{figure}[hbtp]
%\centering
%\includegraphics[width=0.9\textwidth]{Overall_Arch.pdf}
%\caption{Overall architecture of the restaurant recommendation}
%\label{fig:arch}
%\end{figure}
%
%
%To understand how our meta-model fits in the overall framework of restaurant recommendation, here, we present an overall architecture.
%On a high level the architecture is divided into three workflows: a) meta-model learning, b) embedding learning, and c) inference. The two learning workflows are offline, whereas inference is online. 
%
%\begin{itemize}
%    \item \textbf{Meta-model learning:}
%    The first offline workflow is training the meta-model. The meta-model is trained using the transactions  from the source domain and aims at understanding the importance of contextual combination. As discussed earlier, this training is the most compute-intensive one, but this is acceptable as training the meta-model is a one-time process.  The trained meta-model is frozen during this workflow and reused in the remaining workflows. 
%
% 
%    \item \textbf{Embedding learning: }
%    In the second offline workflow, we learn the embeddings of the target domain. Here, we use the meta-model trained in the first step and use it to organize the user and merchant embedding spaces for the target domain to reflect their contextual preferences. Compared to training the meta-model, learning the embeddings is computationally lightweight and can be done with relatively sparse data---this ensures the scalability of our method. 
%    
%    
%    \item \textbf{Inference: }
%Finally, using the meta-model learned in step one, and the embeddings learned in the previous step, we perform the inference online. 
%A controller coordinates the entire process. It takes the user details along with location form the user. The location is used to filter restaurants, which the controller ranks by feeding the user and restaurant embeddings to the meta-model, which returns a preference score for each restaurant. 
%
%\end{itemize}


==> SIGIR 2020 copy/problemdef.tex <==
\vspace{-4pt}
\section{Problem Definition}
%\label{sec:Problem Formulation}
%
%In this subsection, we establish a few relevant preliminaries and formalize our context-based cross-domain recommendation setting.
%
%\subsection{Preliminaries}
Consider recommendation domains $\mathbb{D} = \{\mathbf{D}_i\}$ where each $\mathbf{D}_i$ is a tuple $\{\mathcal{U}_{\mathbf{D}_i}, \mathcal{V}_{\mathbf{D}_i}, \mathcal{T}_{\mathbf{D}_i}\}$, with $\mathcal{U}_{\mathbf{D}_i}$, $\mathcal{V}_{\mathbf{D}_i}$ denoting the user and item sets of $\mathbf{D}_i$, and interactions $\mathcal{T}_{\mathbf{D}_i}$ between them. There is no overlap between the user and item sets of any two domains $\mathbf{D}_i$, $\mathbf{D}_j$.

In the implicit feedback setting, each interaction $t \in \mathcal{T}_{\mathbf{D}_i}$ is a tuple $t = (u, \mathbf{c}, v)$ where $u \in \mathcal{U}_{\mathbf{D}_i}, v \in \mathcal{V}_{\mathbf{D}_i}$ and context vector $\mathbf{c} \in \mathbb{R}^{|\mathbf{C}|}$. For the explicit feedback setting, $\mathcal{T}_{\mathbf{D}_i}$  is replaced by ratings $\mathcal{R}_{\mathbf{D}_i}$, where each rating is a tuple $r = (u, \mathbf{c}, v, r_{uv})$, with the rating value $r_{uv}$ (other notations are the same). For simplicity, all interactions in all domains have the same set of context features. In our datasets, the context feature set $\mathbf{C}$ contains three different types of context features, interactional features $\mathbf{C}_{\mathbf{I}}$ (such as time of interaction), historical features $\mathbf{C}_{\mathbf{H}}$ (such as a user's average spend), and attributional features $\mathbf{C}_{\mathbf{A}}$ (such as restaurant cuisine or user age). Thus each context vector $\mathbf{c}$ contains these three types of features for that interaction, i.e., $\mathbf{c} = [\mathbf{c}_{\mathbf{I}}, \mathbf{c}_{\mathbf{H}}, \mathbf{c}_{\mathbf{A}}]$. 

Under implicit feedback, we rank items $v \in \mathcal{V}_{\mathbf{D}}$ given user $u \in \mathcal{U}_{\mathbf{D}}$ and context $\mathbf{c}$.  In the explicit feedback scenario, we predict rating $r_{uv}$ for $v \in \mathcal{V}_{\mathbf{D}}$ given $u \in \mathcal{U}_{\mathbf{D}}$ and $\mathbf{c}$. Our transfer objective is to reduce the rating or ranking error in a set of disjoint sparse target domains $\{\mathbf{D}_t\} \subset \mathbb{D}$ given the dense source domain $\mathbf{D}_s \in \mathbb{D}$.



%The set of interactions of users $u \in \mathcal{U}_{S}$ are given by $\mathbf{T}_{u} = \{(u, \mathbf{c}_{1}, i_{1}), (u, \mathbf{c}_{2}, i_{2}) \cdots (u, \mathbf{c}_{n_{u}}, i_{n_{u}})\}$ where $n_{u}$ is the number of interactions or transactions for user $u$. In contrast, for the explicit feedback setting, we obtain atmost one review value for each user-item pair, $R_{u, i}$. Again, we will denote the set of ratings of each user by $\mathbf{R}_u$. 

 

% We consider the implicit feedback setting with users $\mathcal{U}$, items $\mathcal{I}$ and binary user-item interaction matrix $\mathcal{Z} \in \mathbb{B}^{\mathopen |\mathcal{U} \mathclose | \times \mathopen |\mathcal{I} \mathclose | }$ ($\mathbb{B} = \{0,1\}$). Further, $\mathcal{N} \in \mathbb{B}^{\mathopen |\mathcal{U} \mathclose | \times \mathopen |\mathcal{U} \mathclose | }$ denotes the explicit social link matrix between the users, we abuse $\mathcal{N}$ to denote both, the social network and its user adjacency matrix. Although we assume undirected social links, the extension to the directed case is straightforward. The total number of user-item interactions and social links are denoted $\mathopen | \mathcal{Z} \mathclose |$, $\mathopen | \mathcal{N} \mathclose |$ respectively. Latent-factor social recommenders learn the latent social and item interest representations for each user. Without loss of generality, let us denote the social embedding matrix $\mathbf{S} \in \mathbb{R}^{\mathopen |\mathcal{U} \mathclose | * d_{S}}$ and the interest embeddings $\mathbf{X} \in \mathbb{R}^{\mathopen |\mathcal{U} \mathclose | * d_{X}}$. Note that $\mathbf{X}_u, \mathbf{S}_u$ denote the rows for user $u$. Further, we denote item embeddings $\mathbf{I} \in \mathbb{R}^{\mathopen |\mathcal{I} \mathclose | * d_{I}}$. Given any user embedding matrix $\mathbf{E}$, we can compute user-user similairities in $\mathbf{E}$'s latent space as, \begin{equation} p_{\mathbf{E}}(u,v) \propto \sigma(\mathbf{E}_u\cdot\mathbf{E}_v) \label{user_proximity} \end{equation} where $u,v \in \mathcal{U}$ and $ \sigma(x) = 1/(1+e^{-x})$. The social and interest embedding spaces $\mathbf{S}$, $\mathbf{X}$ model the social neighborhoods and item interactions of users, and thus induce different user-user proximities $p_S, p_X$ when placed in \Cref{user_proximity}. Social regularization of interest space $\mathbf{X}$ is achieved by introducing a shared coordinate structure between $\mathbf{S}$ and $\mathbf{X}$. At the heart of this problem is the choice of a suitable distance metric in the embedding space. Historically metric learning approaches have learned effective distance functions in similarity, distance-based tasks \cite{metric_learning_survey}, and recently in Collaborative Filtering \cite{cml}.

%\subsection{Context-Driven Cross-Domain Setting}

==> SIGIR 2020 copy/related.tex <==

\section{Related Work}
\label{sec:Related Work}
We briefly summarize a few related lines of work that apply to the sparse inference problem in recommendation: 

%\begin{itemize}
%\item 
\noindent \textbf{Sparsity-Aware Cross-Domain Transfer:} Structure transfer methods regularize the user and item subspaces via principal components~\cite{codebook, aaai10}, joint factorization~\cite{joint-factor1, joint-factor2}, shared and domain-specific cluster structure~\cite{ecmlpkdd13, www19cngan} or combining prediction tasks~\cite{infvae, socialrec} to map user-item preference manifolds. They explicitly map correlated cluster structures in the subspaces. Instead, co-clustering methods use user or item overlaps as anchors for sparse domain inference~\cite{ijcai17, wsdm19}, or auxiliary data~\cite{volkovs2017content, fema} or both~\cite{www19tmh}. It is hard to quantify the volume of users/items or shared content for effective transfer. Further, both overlap-based methods and pairwise structure transfer do not scale to \textit{many sparse-targets}.
% It also scales poorly to non-pairwise transfer settings.
    
%\item 
\noindent \textbf{Neural Layer Adaptation: } A wide-array of layer-transfer and adaptation techniques use convolutional invariants on semantically related images~\cite{joint-adaptation-nets, layer-transfer-coral} and graphs~\cite{motif}. However, unlike convolutional nets, latent collaborative representations are neither interpretable nor permutation invariant~\cite{ncf,vaecf}. Thus it is much harder to establish principled layer-transfer methods for recommendation. We develop our model architecture via novel contextual invariants to enable cross-domain layer-transfer and adaptation.
    
%\item 
\noindent \textbf{Meta-Learning in Recommendation: }
Prior work has considered algorithm selection \cite{federated-meta}, hyper-parameter initialization~\cite{metaparam, kdd19}, shared scoring functions across users~\cite{nips17} and meta-curriculums to train models on related tasks~\cite{kdd19, melu}. Across these threads, the primary challenge is scalability in the multi-domain setting. Although generalizable, they train separate models (over users in ~\cite{nips17}), which can be avoided by adapting or sharing relevant components.


==> SIGIR 2020 copy/temp.tex <==

We use standard classifiers and evaluation metrics. Characterization and Recommendation use linear-kernel SVM evaluated with Precision, Recall, F1-Score and Area-Under-Curve (AUC). Future Activity Prediction uses Linear Regression. Both were implemented with default parameters in sklearn \footnote{http://scikit-learn.org/}. For the activity prediction task, we measure the Root Mean Squared Error (RMSE) in predicted activity proportions for $\textit{(topic, action)}$ pairs against actual proportions of users in the held-out future activity. We compute results with 5-fold cross-validation for each dataset. Statistically significant gains (Paired t-test, $p<0.05$) are in bold.


\subsection{Results}
\label{sec:Result Analysis}
We examine the experimental results for each of the three tasks---User characterization, question recommendation and future activity prediction in this section.

% \textbf{User Characterization Tasks (Reputation, Certification)\\}

% \subsubsection{User Characterization Tasks (Reputation, Certification)}
% \label{sub:User Characterization Tasks (Reputation, Certification)}
Our method improves on the baselines in the \textit{reputation prediction task} by 6.26-15.97\% AUC averaged across the Stack-Exchanges; \Cref{tab:reputation prediction} shows the results with statistically significant improvements in bold. LadFG performs slightly better on the overall precision in reputation prediction (not statistically significant), likely due to over-fitting of the embeddings to user-level data resulting in low recall. Our ability to discover more distinct user clusters even with the same latent dimensions as baselines (refer \cref{combined_clusters}) is the main reason for our gains in predicting reputation. Similarly, we improve on \textit{certification prediction} (see~\Cref{tab:certificate prediction}) by 6.65-21.43\% AUC averaged over MOOCs.

\begin{table}[t]
 \caption{Reputed User Prediction ($\mu\pm\sigma$ across Stack-Exchanges). We obtain improvements of 6.65-21.43\% AUC.}
 \vspace{-10pt}
 \centering
 \begin{tabular}{@{}ccccc@{}}
  \toprule
  \textbf{Method} & \textbf{Precision} & \textbf{Recall}          & \textbf{F1-score}        & \textbf{AUC}             \\
  \midrule
  LRC             & 0.73 $\pm$ 0.04    & 0.69 $\pm$ 0.04          & 0.72 $\pm$ 0.03          & 0.73 $\pm$ 0.03          \\
  DMM             & 0.69 $\pm$ 0.05    & 0.65 $\pm$ 0.04          & 0.66 $\pm$ 0.04          & 0.70 $\pm$ 0.04          \\
  LadFG           & 0.86 $\pm$ 0.03    & 0.75 $\pm$ 0.03          & 0.79 $\pm$ 0.02          & 0.80 $\pm$ 0.03          \\
  FEMA            & 0.79 $\pm$ 0.04    & 0.73 $\pm$ 0.03          & 0.77$\pm$ 0.03           & 0.79 $\pm$ 0.04          \\

  BLDA            & 0.75 $\pm$ 0.04    & 0.71 $\pm$ 0.04          & 0.74 $\pm$ 0.03          & 0.74 $\pm$ 0.04          \\
  CMAP            & 0.85 $\pm$ 0.02    & \textbf{0.83 $\pm$ 0.03} & \textbf{0.84 $\pm$ 0.02} & \textbf{0.86 $\pm$ 0.02} \\
  \bottomrule
 \end{tabular}
 \label{tab:reputation prediction}
 \vspace{-2pt}
\end{table}


\begin{table}[b]
\vspace{-4pt}
 \begin{tabular}{@{}ccccc@{}}
  \toprule
  \textbf{Method} & \textbf{Precision}       & \textbf{Recall}          & \textbf{F1-score}        & \textbf{AUC}             \\
  \midrule
  LRC             & 0.76 $\pm$ 0.04          & 0.71 $\pm$ 0.05          & 0.74 $\pm$ 0.04          & 0.72 $\pm$ 0.03          \\
  DMM             & 0.77 $\pm$ 0.03          & 0.74 $\pm$ 0.04          & 0.75 $\pm$ 0.03          & 0.74 $\pm$ 0.03          \\
  LadFG           & 0.81 $\pm$ 0.02          & 0.78 $\pm$ 0.02          & 0.79 $\pm$ 0.02          & 0.79 $\pm$ 0.02          \\
  FEMA            & 0.78 $\pm$ 0.03          & 0.75 $\pm$ 0.04          & 0.76 $\pm$ 0.03          & 0.78 $\pm$ 0.03          \\

  BLDA            & 0.80 $\pm$ 0.04          & 0.75 $\pm$ 0.03          & 0.77 $\pm$ 0.03          & 0.77 $\pm$ 0.04          \\
  CMAP            & \textbf{0.86 $\pm$ 0.02} & \textbf{0.81 $\pm$ 0.03} & \textbf{0.83 $\pm$ 0.02} & \textbf{0.84 $\pm$ 0.02} \\
  \bottomrule
 \end{tabular}
%  \vspace{-2pt}
  \caption{Certificate Earner Prediction ($\mu \pm \sigma$ across MOOCs); CMAP improves upon baselines by 6.65-21.43\% AUC}
 \vspace{-20pt}
 \label{tab:certificate prediction}

\end{table}



%\vspace{-15pt}
% \begin{flushleft}
% \textbf{Question Recommendation Task (Stack-Exchanges)\\}

% \subsubsection{Question Recommendation Task (Stack-Exchanges)}
% \label{sub:Question Recommendation Task (Stack-Exchanges)}

For the \textit{question recommendation task}~\Cref{tab:question recommendation}, we see gains between 6-47\% AUC over the baselines. To do well in this task, we require the model to make finer distinctions between the topical preferences of users; user reputation and action style are also important in this task.
% \end{flushleft}


\begin{table}[!htbp]
 \centering
 \caption{Question Recommendation ($\mu\pm\sigma$ across Stack-Exchanges)with 6.30-47.45\% AUC gains for CMAP. DMM performs quite well owing to importance of content in this task.}
 \vspace{-10pt}
 \begin{tabular}{@{}ccccc@{}}
  \toprule
  \textbf{Method} & \textbf{Precision}       & \textbf{Recall}          & \textbf{F1-score}        & \textbf{AUC}             \\
  \midrule
  LRC             & 0.65 $\pm$ 0.06          & 0.57 $\pm$ 0.08          & 0.60 $\pm$ 0.06          & 0.57 $\pm$ 0.05          \\
  DMM             & 0.72 $\pm$ 0.04          & 0.81 $\pm$ 0.05          & 0.75 $\pm$ 0.04          & 0.74 $\pm$ 0.04          \\
  LadFG           & 0.88 $\pm$ 0.03          & 0.60 $\pm$ 0.02          & 0.71 $\pm$ 0.02          & 0.76 $\pm$ 0.04          \\
  FEMA            & 0.79 $\pm$ 0.05          & 0.73 $\pm$ 0.06          & 0.77$\pm$ 0.05           & 0.79 $\pm$ 0.03          \\

  BLDA            & 0.70 $\pm$ 0.04          & \textbf{0.84 $\pm$ 0.04} & 0.77 $\pm$ 0.03          & 0.75 $\pm$ 0.04          \\
  CMAP            & \textbf{0.89 $\pm$ 0.03} & 0.81 $\pm$ 0.02          & \textbf{0.85 $\pm$ 0.03} & \textbf{0.84 $\pm$ 0.02} \\
  \bottomrule
 \end{tabular}
%  \vspace{1.5pt}
 \label{tab:question recommendation}
 \vspace{-5pt}
\end{table}

%
% \subsubsection{Future Activity Prediction Task :}
% \label{sub:Future Activity Prediction Task :}

%
% \begin{flushleft}
%  \textbf{Future Activity Prediction Task :\\}
%   \end{flushleft}
For the \textit{future activity prediction task}, our method shows gains over baselines in RMSE by 12\%-25\% on MOOCs and between 9.5\%-22\% on Stack-Exchanges; (see~\Cref{tab:future activity prediction}). Gains are explained by our model's ability to make finer distinction on action styles, and to be able to make better distinctions between profiles assigned to users.


\begin{table}[b]
 \vspace{-2pt}
 \centering
 \begin{tabular}{@{}cccccc@{}}
  \toprule
  \textbf{Method} & \textbf{DMM}   & \textbf{LadFG} & \textbf{FEMA}  & \textbf{BLDA}  & \textbf{CMAP}           \\
  \midrule
  MOOC            & 4.9 $\pm$ 0.4  & 4.2 $\pm$0.3   & 4.1 $\pm$ 0.2  & 4.4  $\pm$ 0.4 & \textbf{3.6  $\pm$ 0.2} \\
  Stack-Ex        & 8.6  $\pm$ 0.6 & 7.9  $\pm$ 0.4 & 7.5  $\pm$ 0.3 & 7.4  $\pm$ 0.5 & \textbf{6.7  $\pm$ 0.4} \\
  \bottomrule
 \end{tabular}
%  \vspace{1.5pt}
\caption{Future Activity Prediction (RMSE ($\times 10^{-2}$) $\mu \pm \sigma$), Lower RMSE is better. CMAP ouperforms baselines in MOOCs (12\%-25\%) and Stack-Exchanges (9.5\%-22\%)}
 \label{tab:future activity prediction}
 \vspace{-15pt}
\end{table}

%\subsection{Characterizing Inactive Users}
%\label{sub:Effects of data sparsity}
%In order to study the gains of our algorithm on characterizing users with different levels of activity, we split participants in each dataset into four equal partitions based on their number of interactions (Quartiles 1-4, 1 being least active). We then sample participants from each quartile and evaluate all methods on prediction performance (AUC).
%
%Our model shows magnified gains (\Cref{data_sparsity}) in prediction performance over baseline models in the first and second quartiles which correspond to users with limited activity. BLDA performs the weakest in Quartile-1 since it relies on interaction activity to build user representations. These gains confirm our ability to group inactive users in appropriate paritions.

In this section, we showed impressive performance gains on three types of tasks for our model over state of the art baselines. In the next section, we qualitatively analyze the reasons for it's success.

\vspace{-6pt}
\subsection{Why does CMAP work well?}
\label{sub:Why does CMAP work well?}

To interpret the gains obtained by CMAP, we examine the extracted clusters in~\Cref{sub:The Impact of Profile Driven Seating} and then look at users responsible for the performance gains of our model in~\Cref{sub:Making gains on inactive users}.
\vspace{-2pt}
\subsubsection{\textbf{The Impact of Profile Driven Seating}}
\label{sub:The Impact of Profile Driven Seating}

We now compare clusters obtained through CMAP seating against conventional generative assignments in BLDA~\cite{blda} on Stack-Exchanges. Both models group users best described by the same profile to form clusters. We use average user reputations of the clusters (appropriately normalized) as an external validation metric for cluster quality. We also run our model excluding time and knowledge-exchanges to see the effect on the clusters.~\Cref{ask_ubuntu_clusters} shows the result from the \texttt{Ask-Ubuntu} Stack Exchange, and~\Cref{cmap_clusters} shows the main activities and topics of the top three CMAP clusters. %\hs{is~\Cref{cmap_clusters} the full CMAP?}.
\begin{figure}[b]
 \vspace{6pt}
 %\includegraphics[width=\columnwidth]{./data/qualitative/ask_ubuntu_1.pdf}
 \includegraphics[width=\columnwidth]{./images/foo.pdf}
 \vspace{-10pt}
 \caption{Bubbles denote user clusters discovered by each model in the Ask-Ubuntu dataset (Bubble size $\propto$ Users in Cluster). CMAP discovers fine distinctions of reputed users (Profiles 1,2,3,4) by content preference and activity (\Cref{cmap_clusters}). BLDA clusters are mean-sized and close to the population average in reputation. In contrast, our assignments better reflect the behavior skew of users in the dataset.}
 \label{ask_ubuntu_clusters}
\end{figure}
We make the following key observations from the clusters:
\begin{description}
 \item[The Mean-Shift problem:] The Dirichlet-Multinomial setting in BLDA tends to merge profiles and hence shift cluster sizes and average participant reputation closer to the mean.~\Cref{ask_ubuntu_clusters} shows that 15 of 20 BLDA clusters have nearly the same size and average reputation. Both variants of CMAP show diversity in cluster size and high reputation variability across tables. Our cluster assignments appear to mirror the behavior skew for \texttt{Ask-Ubuntu} (c.f.~\Cref{skew_sparsity}).\\
 \item[Profile Quality:] CMAP learns finer variation in the topic affinities and actions of expert users. We can observe these variations from~\Cref{ask_ubuntu_clusters} and from~\Cref{cmap_clusters}. The top three profiles are of higher reputation, smaller in size, and from~\Cref{cmap_clusters}, each of these clusters shows distinct activities different from the mean activity. CMAP clusters appear to better reflect skewed user activity (c.f.~\Cref{d1}) and content preference (c.f.~\Cref{skew_sparsity}) with flexible profile-driven seating.
\end{description}

\begin{figure*}
 \centering
 \includegraphics[width=\textwidth]{./data/qpwide.pdf}
 \vspace{-22pt}
 \caption{Effects of activity sparsity on prediction tasks (AUC) for Stack Exchanges (datasets 1-10) and MOOCs (datasets 11-14). CMAP has greatest performance gains in Quartile-1 (Sparse users), performance gap reduces for very active users (Quartile-4).}
 \label{data_sparsity}
\end{figure*}

\begin{center}
 \begin{table}[b]


  \vspace{-10pt}
  \begin{tabular}{@{}cp{0.4\linewidth}p{0.4\linewidth}@{}}
   \toprule
   \textbf{Cluster} & \textbf{Action Style}                                & \textbf{Common Topics}                            \\
   \midrule
   1                & +31\% Answer, +24\% Edits, -9\% Questions            & Graphics Drivers, Booting Issues, Disk Partitions \\
   2                & +67\%Answer,	-3\% Edits, \hspace{2cm}-21\% Questions & Gnome, Desktop, Package Install                   \\
   3                & +11\% Answer, -4\% Edits, +47\% Questions            & Script, Application, Sudo Access                  \\
   \bottomrule
  \end{tabular}
    \caption{Action and Content description of users in top-3 clusters discovered by CMAP in Ask-Ubuntu, +/- values of action proportions against the average Ask-Ubuntu user}
  \label{cmap_clusters}
  \vspace{-17.7pt}
 \end{table}
\end{center}
%
% \begin{itemize}
%  \item \textbf{BLDA Clusters are Uninformative due to Mean-Shift: } The Dirichlet-Multinomial setting in BLDA tends to merge profiles and hence shift clusters closer to mean sizes and reputation. Our cluster assignments appear to better reflect the known disparities in the user population (\Cref{skew_sparsity}).
%  \item \textbf{Profile-Driven Seating: } CMAP clusters appear to better reflect uneven/skewed user activity (\Cref{d1}) and content preference (\Cref{skew_sparsity}) with flexible profile-driven seating.
%  \item \textbf{Profile Quality: }The mean-shift effect degrades information content of the learned profile variables in BLDA. For instance, expert users in our clusters (\Cref{cmap_clusters}) are not coherently grouped in the BLDA assignments.
%  \item \textbf{Profile Resolution: } Our assignments appear to discover finer variation in the topic affinities and actions of expert users, which enables fine-grained latent profile learning.
%
%        %This is particularly important in content recommendation and user characterization (\cref{sub:Prediction Tasks}).
%
% \end{itemize}
\begin{figure}[!htbp]
 \vspace{-15pt}
 %\includegraphics[width=\columnwidth]{./data/qualitative/combined_clusters_1.pdf}
 \includegraphics[width=\columnwidth]{images/foo2.pdf}
 \vspace{-16.5pt}
 \caption{Bubbles denote clusters in other Stack-Exchanges (Bubble size $\propto$ Users in Cluster). CMAP discovers highest reputation clusters in all datasets (Thick red dot, Top-left). BLDA clusters tend to mean reputation, size (Mean-Shift) not capturing disparities. In our case, profiles 1,2,3,4 appear to capture niche, highly reputed user behaviors}
 \vspace{1pt}
 \label{combined_clusters}
\end{figure}


\vspace{-13pt}
We observe a similar trend in the aggregated clusters obtained from all the other Stack-Exchange datasets  (c.f.~\Cref{combined_clusters}). The Dirichlet-Multinomial setting in BLDA results in similarly sized clusters which cannot model highly skewed content and action affinities of users. Note the fewer high-reputation clusters of BLDA in comparison to the finer distinctions of reputed users in our model. Our performance in prediction and recommendation reflect these observations, we see significant gains in our ability to characterize reputed users and recommend suitable content (\Cref{sub:Prediction Tasks}).

\subsubsection{\textbf{Making gains on inactive users}}
\label{sub:Making gains on inactive users}

We now investigate the source of our gains. We split users in each Stack-Exchange and MOOC into four quartiles based on interaction count (Quartile 1 is least active, 4 most). Then, we evaluate each method on Reputation and Certificate Prediction AUC in each quartile 
%\hs{reputation AUC, or certificate prediction AUC?}
of Stack Exchange and MOOC datasets respectively.

Our model shows large gains (\Cref{data_sparsity}) in Quartiles 1,2 that contain sparse users. We attribute these gains due to our joint profile learning to describe similar users seated on tables. The decision to address skew and sparsity jointly has two advantages: better profile fits for sparse users; more distinct and informative profiles in skewed scenarios. In contrast, models building representations  at the user level perform weakly in Quartiles-1,2 since these methods rely on interaction volume. We make smaller gains in Quartiles 3,4. %T

\textbf{To summarize: } jointly addressing sparsity and skew by profile driven seating is responsible for our gains. Importantly, the clusters are coherent, the model learns fine distinctions in behavioral profiles and exhibits behavior skew found in the underlying data.

% We re-iterate a few key observations from the high-reputation clusters in the Ask-Ubuntu dataset (\Cref{cmap_clusters}, \Cref{ask_ubuntu_clusters}) with our model:
% \begin{itemize}
%  \item \textbf{Distinct Action-Styles :} The mutual enhancement of user seating and profile learning results in more distinct profiles. Both the topic content and actions of users in \Cref{cmap_clusters} show significant
%  \item \textbf{Size Variations :} This is closely related to the first point. If we require distinctive action styles, the profile sizes must vary owing to behavior skew (very few users display certain trends of activity). Our seating is better suited to such scenarios due to it's exploration of niche profiles and discounting of the common and larger profiles as described with \Cref{eq:profiledist}.
% \end{itemize}
% These improvements aid us in both recommending suitable content (\Cref{tab:question recommendation}) as seen in the question recommendation result, as well as future activity prediction for users (\Cref{tab:behavior prediction}).

% (We are yet to add the content recommendation experiments, currently running them). The below plots indicate our ability to identify and profile niche high reputation user groups within each stack exchange (Blue bubbles indicate users grouped under profiles discovered by BLDA, while red bubbles are ours, bubble size indicates the percentage of the population placed under the profile). Conventional CRP seating cannot account for the details of the latent user model when generating clusters, the resulting clusters thus would not capture latent patterns of user interaction shared by users grouped together. Based on the below plots, our grouping discovers coherent patterns of user interaction with content which result in users possesssing a high or a low reputation. Users seated together share these traits and hence exhibit similar levels of reputation.
%
%Ask-Ubuntu, original dataset vs deskewed version. Our results can be seen to be closely aligned with BLDA in the deskewed version, however diverging in the original dataset to discover niche high reputation groups.
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/skew.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/deskew.pdf}
%\end{figure}
%
%
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/1.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/2.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/3.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/4.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/5.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/6.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/7.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/8.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/9.pdf}
%\end{figure}
\vspace{-3pt}
\subsection{What if there was less Skew?}
\label{b_skew}
In this section, we study a counterfactual: what if the real-world datasets were less skewed?
%
% observed behavioral skew was less than observed?
% What is the effect of reducing the overall behavior skew so that different action styles are more balanced in the dataset?
To study this question, we sub-sample users who predominantly perform the two most common actions in our largest datasets, \texttt{Ask-Ubuntu} (Comments and Questions) and \texttt{Comp Sci-1 MOOC} (Play and Skip). These users are sub-sampled by half while retaining all other users, hence reducing overall action skew in the data. Baseline models are expected to perform better with reduced skew. All models degrade in Ask-Ubuntu owing to significant loss of content.
%Eliminating skew completely is very hard owing to significant content loss and high skew in the original datasets.~\Cref{tab:skew} shows the results of the prediction tasks(in terms of AUC) after partially de-skewing data.
\begin{table}[b]
 \centering
%  \vspace{1pt}
%   \vspace{-10pt}
 \begin{tabular}{@{}rcccc@{} }
  \toprule
  \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{@{}c}{\textbf{Ask-Ubuntu}} & \multicolumn{2}{c@{}}{\textbf{CompSci1 MOOC}}\\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & Original       & Deskewed       & Original       & Deskewed \\
  \midrule
  LRC   & 0.671          & 0.656          & 0.713          & 0.734    \\
  DMM   & 0.647          & 0.611          & 0.684          & 0.672    \\
  LadFG & 0.734          & 0.718          & 0.806          & 0.830    \\
  BLDA  & 0.706          & 0.683          & 0.739          & 0.788    \\
  CMAP  & \textbf{0.823} & \textbf{0.746} & \textbf{0.851} & 0.849    \\
  \bottomrule
 \end{tabular}
%  \vspace{2pt}

 \label{tab:skew}
 \caption{CMAP outperforms baselines (AUC) in the de-skewed datasets, but with smaller gains}
 \vspace{-15pt}
\end{table}

\vspace{3pt}

Table 11 shows that CMAP still maintains a lead owing to inactive users. We also investigate performance gains in a highly skewed and sparse Stack-Exchange (Ask-Ubuntu) vs least skewed (Christianity) in Table 12. On average, we outperform baselines by 13.3\% AUC for Ask-Ubuntu vs 10.1\% for Christianity Stack-Exchange in User Characterization.
\begin{table}[t]
 \centering
%  \vspace{-1pt}

\vspace{-8pt}
 \begin{tabular}{@{}ccccccc@{}}
  \toprule
  \textbf{Method} & \textbf{DMM} & \textbf{LRC} & \textbf{LadFG} & \textbf{FEMA} & \textbf{CMAP}  & \textbf{BLDA} \\
  \midrule
  Ask-Ubuntu      & 0.647        & 0.671        & 0.734          & -             & \textbf{0.823} & 0.706         \\
  Christianity    & 0.684        & 0.720        & 0.842          & 0.818         & \textbf{0.856} & 0.791         \\
  \bottomrule
 \end{tabular}
%  \vspace{1.5pt}
 \label{tab:ubuntu-christianity}
 \caption{We see greater gains for User Characterization in a high-skew dataset (Ask-Ubuntu) vs low-skew (Christianity)}
	\vspace{-6pt}
\end{table}
% skip for wsdm 2018
% The seating arrangement of participants resulting from our model reflects behavior skew. The model distributes participants more evenly across profiles in comparison to the original datasets. The TableSum terms from \cite{eqn} are more uniformly distributed. Our CRP assignment process adapts to the extent of behavioral skew present in the data (c.f.~\Cref{fig:skew}). The figure illustrates the effect of varying the discount parameter $\delta$. A higher value of $\delta$ creates a ``fatter'' tail of activity profiles.
%
% \begin{figure}[htbp]
%  \includegraphics[viewport = .75in 0in 14.25in 6.75in ,clip, width=\columnwidth]{./data/skew.pdf}
%  \caption{Effect of varying the discount parameter $\delta$ on the seating arrangement. A higher value of $\delta$ favors the creation of more tables, thus creating a ``fatter'' activity profile distribution.}
%  \label{fig:skew}
% \end{figure}
\subsection{Scalability Analysis}
\label{sub:Scalability Analysis}
We compared the runtimes and memory consumption of our serial and batch-sampling (with 8 cores) inference algorithms with other models, for different volumes of interaction data obtained from random samples of the Ask-Ubuntu Stack-Exchange. BLDA is the fastest among the set of compared models. Our 8x batch sampler is comparable to BLDA in runtime. FEMA was the least scalable owing to the $O(|\mathcal{U}|^2)$ growth of the User-User regularizer matrix. ~\Cref{fig:memtime} shows the comparisons between the algorithms.
%\begin{figure}[htbp]
% \includegraphics[viewport = .25in 0in 7.5in 5.5in ,clip, width=\columnwidth]{./data/memtime.pdf}
% \caption{Effects of dataset size on algorithm runtime and memory consumption. BLDA is the fastest among the set of compared models. }
% \label{fig:memtime}
%\end{figure}
\begin{figure}[htbp]
\vspace{-9pt}
 \includegraphics[width=\columnwidth]{./data/memtime.pdf}
 \vspace{-24pt}
 \caption{Effects of dataset size on algorithm runtime and memory consumption. BLDA is the fastest among the set of compared models. }
 \vspace{-5pt}
 \label{fig:memtime}
 \vspace{-4pt}
\end{figure}

\vspace{-5pt}
\subsection{Parameter Sensitivity Analysis}
\label{sub:Parameter Sensitivity Analysis}

Our model is primarily impacted by three parameter values: number of profiles $R$, number of Action-Topics $K$ and discount $\delta$. We find results to be stable in a broad range of parameter values indicating that in practice our model requires minimal tuning (\Cref{fig:parameter sensitivity}). It is worth noting that while $R$ primarily impacts the granularity of the discovered activity profiles, K impacts the resolution of content-action associations. Dirichlet and other hyper-parameters have negligible impact on the profiles and seating arrangement learned. Our inference algorithm converges within 1\% AUC in less than 400 sampling iterations across all datasets.
\begin{figure}[!htbp]
\vspace{-9pt}
 \includegraphics[viewport = 1.25in 0in 16.75in 4.55in ,clip, width=\columnwidth]{./data/mp7.pdf}
 \vspace{-18pt}
 \caption{Mean performance(AUC) \& 95\% confidence interval with varying model parameters one at a time: $\delta$, $R$, $K$. Stability is observed in broad ranges of parameter values.}
 
 \label{fig:parameter sensitivity}
\end{figure}


%\begin{figure}[!htbp]
% \includegraphics[height=0.2\textwidth]{./data/gibbs.pdf}
% \caption{Model convergence over sampling iterations}
% \label{fig:gibbs}
%\end{figure}

\subsection{Limitations}
\label{limitations}
We identify two limitations. First, we make no assumptions about the structure of knowledge (e.g. a knowledge of ``probability'' is useful to understand ``statistical models''); incorporating knowledge structure, perhaps in the form of an appropriate prior will help with better understanding participants with low activity. Second, we assume a bounded time range. Development of latent profiles for streaming activity can lead to deployment with real-time data.

It would be an interesting exercise to observe the effect of dynamic updates to Pitman-Yor hyper-parameters over sampling iterations \cite{teh}. Although such an approach has been explored for LDA \cite{wallach}, it is unclear how over-fitting in our approach can be avoided in case of hyper-parameter drift. We plan this study for future work.
% domain ontology  or make use of any external

% Most of our errors arise from sparse users with ambiguous activity, who could be assigned inappropriate profiles. External sources of data could be integrated to aid us in such cases. Our model also assumes a bounded time range and is inapplicable to streaming data. Furthermore, our profiles are purely data-driven and do not provide a way to encode prior beliefs on behavior trends. We plan to address these shortcomings of our approach in future work.
% \begin{figure*}
%  \subfigure[b][]{
%   \centering
%   \includegraphics[width=0.32\linewidth]{plots/varyingR}
%  }
%  \subfigure[b][]{
%   \centering
%   \includegraphics[width=0.32\linewidth]{plots/varyingK}
%  }
%  \subfigure[b][]{
%   \centering
%   \includegraphics[width=0.32\linewidth]{plots/varyingD}
%  }
%
%  \caption{Effects on model performance of  (a) Varying Profiles R  (b) Varying Behaviors K  (c) Varying discount parameter $\delta$}
% \end{figure*}
% \begin{center}
% \begin{table*}
% \begin{tabular}{cp{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}
% p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}
% p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}}
% \toprule
% \multirow{2}{*}{\textbf{Method \textbackslash Data}} & \multicolumn{4}{c}{\textbf{AskUbuntu}} & \multicolumn{4}{c}{\textbf{Android}} & \multicolumn{4}{c}{\textbf{Travel}} & \multicolumn{4}{c}{\textbf{Chemistry}} & \multicolumn{4}{c}{\textbf{Christianity}}\\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
% & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC\\
% \midrule
% LRC & & & & & 0.78 & 0.67 & 0.72 & 0.74 & 0.80 & 0.70 & 0.75 & 0.76 & 0.81 & 0.65 & 0.73 & 0.75 & 0.62 & 0.81 & 0.70 & 0.66\\
% DMM & & & & & 0.84 & 0.61 & 0.70 & 0.74 & 0.75 & 0.84 & 0.79 & 0.78 & 0.65 & 0.77 & 0.71 & 0.68 & 0.62 & 0.92 & 0.74 & 0.68\\
% LadFG & & & & & 0.78 & 0.65 & 0.72 & 0.76 & 0.84 & 0.79 & 0.81 & 0.82 & 0.83 & 0.69 & 0.74 & 0.75 & 0.86 & 0.81 & 0.84 & 0.84\\
% BLDA & & & & & 0.80 & 0.65 & 0.72 & 0.75 & 0.81 & 0.79 & 0.79 & 0.80 & 0.74 & 0.68 & 0.71 & 0.72 & 0.79 & 0.78 & 0.79 & 0.80\\
% FEMA &-&-&-&-& 0.73 & 0.67 & 0.70 & 0.71 &  0.84 & 0.78 & 0.81 & 0.82 & 0.80 & 0.68 & 0.73 & 0.75 & 0.84 & 0.78 & 0.81 & 0.82\\
% Ours & & & & & 0.87 & 0.79 & 0.83 & 0.84 & 0.88 & 0.82 & 0.84 & 0.85 & 0.89 & 0.70 & 0.78 & 0.81 & 0.87 & 0.82 & 0.84 & 0.85\\
% \bottomrule
% \end{tabular}
% \end{table*}
% \end{center}
%
% \begin{center}
% \begin{table*}
% \begin{tabular}{cp{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}
% p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}}
% \toprule
% \multirow{2}{*}{\textbf{Method \textbackslash Data}} & \multicolumn{4}{c}{\textbf{CS1 Mooc}} & \multicolumn{4}{c}{\textbf{CS2 Mooc}} & \multicolumn{4}{c}{\textbf{Science Mooc}} & \multicolumn{4}{c}{\textbf{Math Mooc}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
% & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC \\
% \midrule
% LRC & & & & & 0.83 & 0.74 & 0.78 & 0.79 & 0.82 & 0.68 & 0.75 & 0.77 & 0.80 & 0.76 & 0.78 & 0.79\\
% DMM & & & & & 0.88 & 0.77 & 0.83 & 0.83 & 0.81 & 0.80 & 0.81 & 0.81 & 0.82 & 0.78 & 0.80 & 0.79\\
% LadFG & & & & & 0.84 & 0.78 & 0.81 & 0.82 & 0.82 & 0.79 & 0.80 & 0.80 & 0.79 & 0.73 & 0.76 & 0.78\\
% BLDA & & & & &  0.80 & 0.76 & 0.77 & 0.78 & 0.77 & 0.58 & 0.66 & 0.70 & 0.78 & 0.75 & 0.76 & 0.77\\
% FEMA &-&-&-&-& 0.83 & 0.76 & 0.79 & 0.80 & 0.72 & 0.69 & 0.70 & 0.72 & 0.74 & 0.73 & 0.74 & 0.73\\
% Ours & & & & &  0.87 & 0.83 & 0.85 & 0.86 & 0.85 & 0.82 & 0.83 & 0.84 & 0.85 & 0.82 & 0.84 & 0.84\\
% \bottomrule
% \end{tabular}
% \end{table*}
% \end{center}
\vspace{-7pt}

==> datadesc.tex <==
% !TEX Root=draft.tex
\vspace{-5pt}
\section{Dataset Description}
\label{sec:Platform Description}


\begin{center}
 \begin{table}[b]
  \begin{tabular}{p{0.15\linewidth}lp{0.52\linewidth}}
   \toprule
   \textbf{Platform}                          & \textbf{Action} & \textbf{Description}              \\
   \midrule
   \multirow{7}{2cm}{\textbf{Coursera MOOC}}  & Play            & First lecture segment view        \\
                                              & Rewatch         & Repeat lecture segment view       \\
                                              & Clear Concept   & Back and forth movement, pauses   \\
                                              & Skip            & Unwatched lecture segment         \\
                                              & Create Thread   & Create forum thread for inquiries \\
                                              & Post            & Reply to existing threads         \\
                                              & Comment         & Comment on existing posts         \\
   \midrule
   \multirow{5}{2cm}{\textbf{Stack-Exchange}} & Question        & Posting a question                \\
                                              & Answer          & Authoring answer to a question    \\
                                              & Comment         & Comment on a question/answer      \\
                                              & Edit            & Modify posted content             \\
                                              & Follow          & Following posted content          \\
   \bottomrule
  \end{tabular}
  
  
%   \vspace{-5pt}
	\caption{User Action Description (Coursera/Stack-Exchange)}
  	\vspace{-15pt}
  	\label{t1}
 	\end{table}
	\end{center}
%\begin{center}
%\begin{table}
%\begin{tabular}{llll}
%\toprule
%\textbf{Platform} & \textbf{Link Label} & \textbf{Source Int} & \textbf{Target Int}\\
%\midrule
%\multirow{2}{*}{MOOC} & Commenting & Comment & Post\\
%& Posting & Post & Create Thread\\
%\midrule
%\multirow{3}{*}{Stack Ex.} & Commenting & Comment & Question/Answer\\
%& Answering & Answer & Question\\
%& Editing & Edit & Question/Answer\\
%%\bottomrule
%\bottomrule
%\end{tabular}
%\caption{Interaction Links}
%\label{t11}
%\end{table}
%\end{center}
%\begin{table*}
%\caption{Minimum Requirements for Automatic \textbf{Readmission} into the Commerce Faculty}
%\centering
%\begin{tabular}{ccccc}
%\toprule
%& \multicolumn{2}{c}{BCom} &
%\multicolumn{2}{c}{B.Bus.Sci} \\
%\cmidrule(r{4pt}){2-3} \cmidrule(l){4-5}
%& Number of courses required to pass & Cumulative Total of Courses & Number of courses &         Cumulative Total of Courses\\
%\midrule
%First year & 4 & 8 & 4 & 18 \\
%\bottomrule
%\end{tabular}
%\label{table:mr}
%\end{table*}
%\begin{center}
%\begin{table}
%\begin{tabular}{cp{0.7\linewidth}}
%\toprule
%\textbf{Symbol} & \textbf{Description} \\
%\midrule
%Question & Authoring a question on the stack exchange website\\
%Answer & Authoring an answer to a question on the stack exchange website\\
%Comment & Authoring a comment on a question or answer\\
%Edit & Modifying existing content via addition or deletion of text\\
%Favorite & Liking interesting or relevant content\\
%\bottomrule
%\end{tabular}
%\caption{User Action Set - Stack Exchange}
%\label{t2}
%\end{table}
%\end{center}
%
%\begin{center}
%\begin{table}
%\begin{tabular}{lll}
%\toprule
%\textbf{Link Label} & \textbf{Source Interaction} & \textbf{Target Interaction}\\
%\midrule
%Commenting & Comment & Question/Answer\\
%Answering & Answer & Question\\
%Editing & Edit & Question/Answer\\
%\bottomrule
%\end{tabular}
%\caption{Interaction Links - Stack Exchange}
%\label{t22}
%\end{table}
%\end{center}
% \vspace{-16pt}
% \textbf{Stack-Exchange Q\&A Networks: }
\vspace{-15pt}
We now provide a brief description of the Coursera MOOC and Stack-Exchange datasets that we use in our experiments and characterize them in terms of skew and sparsity.

Stack-Exchanges are community Q\&A websites where participants discuss a wide range of topics. Users interact with each other and perform a range of actions (e.g. post question, answer, comment etc.). We experiment on 10 Stack-Exchanges, chosen for thematic diversity and size variation. Coursera MOOCs feature video lectures for students to watch and a forum where students and instructors can interact. We analyze the actions (e.g. play, skip, rewind etc.) on the videos, lecture content via subtitles, and the forum interaction for four MOOCs, chosen for thematic diversity. The user action types and datasets are summarized in~~\Cref{t1} and~\Cref{d1} respectively.

% exchanges between students and instructors via course forums. Patterns of lecture viewing obtained from video clickstreams provide valuable cues on learning behavior \cite{mooc1, ladfg}, in addition to forum activity \cite{forum1}. We combine these two sources to define the action set of students (\Cref{t1}). Lecture content is extracted from subtitle files. Students engage in exchanges by posting or commenting on forum content. We conduct our experiment with both, technical and non-technical MOOCs (\Cref{d1}).



% domains of public interest. Users interact by asking/answering questions, and editing, following and commenting on content (\Cref{t1}). Users engage in knowledge-exchange by answering questions and editing/commenting each other's content. We conduct our experiments on several Stack-Exchange websites chosen to capture diverse technical and non-technical subjects and differently sized user populations (\Cref{d1}).
%reacting to other users' activity, specifically liking and editing content, favorite, and answering questions hence establishing Editing, Liking and Answering links between pairs of users, indicative of their interests and knowledge
\begin{center}
 \begin{table}
  \caption{Preliminary analysis indicates significant behavior skew and inactive user proportion, although slightly reduced in specialized domains like Christianity}
  \vspace{-10pt}
  \begin{tabular}{@{}p{0.14\linewidth}p{0.19\linewidth}cccc@{}}
   \toprule
   \textbf{Platform}                             & \textbf{Dataset} & \textbf{Users} & \textbf{Interactions} & \textbf{$\eta_t$} & \textbf{$S_N$} \\
   \midrule
   \multirow{4}{2.2cm}{\textbf{Coursera MOOC}} & Comp Sci-1       & 26,542         & 834,439               & -2.51             & 0.67           \\  
   												& Math             & 10,796         & 162,810               & -2.90             & 0.69           \\
                                                 & Nature           & 6,940          & 197,367               & -2.43             & 0.70           \\
                                                 
                                                 & Comp Sci-2       & 10,796         & 165,830               & -2.14             & 0.73           \\
   \midrule
   \multirow{10}{2.2cm}{\textbf{Stack-Exchange}} & Ask-Ubuntu       & 220,365        & 2,075,611             & -2.81             & 0.65           \\
                                                 & Android          & 28,749         & 182,284               & -2.32             & 0.56           \\
                                                 & Travel           & 20,961         & 277,823               & -2.01             & 0.66           \\
                                                 & Movies           & 14,965         & 150,195               & -2.17             & 0.67           \\
                                                 & Chemistry        & 13,052         & 175,519               & -2.05             & 0.63           \\
                                                 & Biology          & 10,031         & 138,850               & -2.03             & 0.71           \\
                                                 & Workplace        & 19,820         & 275,162               & -2.05             & 0.59           \\
                                                 & Christianity     & 6,417          & 130,822               & -1.71             & 0.64           \\
                                                 & Comp Sci         & 16,954         & 183,260               & -2.26             & 0.62           \\
                                                 & Money            & 16,688         & 179,581               & -1.72             & 0.63           \\
   \bottomrule
  \end{tabular}

  \label{d1}
%   \vspace{-5pt}
 \end{table}

\end{center}


% \vspace{-13pt}
% \textbf{Coursera MOOC Platform: } Coursera MOOCs feature a structured learning environment with lecture content and exchanges between students and instructors via course forums. Patterns of lecture viewing obtained from video clickstreams provide valuable cues on learning behavior \cite{mooc1, ladfg}, in addition to forum activity \cite{forum1}. We combine these two sources to define the action set of students (\Cref{t1}). Lecture content is extracted from subtitle files. Students engage in exchanges by posting or commenting on forum content. We conduct our experiment with both, technical and non-technical MOOCs (\Cref{d1}).

% \vspace{2pt}
\vspace{-18pt}
To get a feel for these datasets, let us examine sparsity and behavior skew. To understand sparsity, we compute the power-law ($f_w = c.w^{\eta_t}$) exponent $\eta_t$ that best describes the fraction of users $f_w$ who were active for $w$-weeks. A more negative index indicates that fewer users are consistently active. As a reference point, when $\eta_t=0$, a constant fraction of users are always active. Thus when we notice that $\eta_t=-2.81$ for \texttt{Ask Ubuntu} Stack Exchange in~\Cref{d1}, it means that the number of users who are active for two weeks is just $14\%$ of those active for one week.~\Cref{d1} indicates that larger Stack Exchanges tend to have greater sparsity.

We measure skew by first identifying the dominant action type or style of each user (e.g commenter, editor) and then compute the normalized entropy $S_N$ of the resulting user distribution.
% Activity skew (excluding text content) can be approximated by grouping users by dominant action type (e.g. users who mostly comment or ask questions), and computing the normalized entropy ($S_N$) of the resulting distribution.
In a large Stack-Exchange such as \texttt{Ask-Ubuntu}, while less than 5\% (c.f~\Cref{skew_sparsity})  of the users have `Answer' as their dominant type, over 60\% of the users have `Comment' as their dominant action. This does not consider content topics, which result in even greater skew. When $S_N=1$, all dominant action types are equally likely; in contrast $S_N=0$ indicates a single dominant action type. In MOOCs, 'Play' is the dominant action type with low forum participation (participation rates $\sim$10-15\% in our MOOC forums).




% It is interesting to observe that larger Stack-Exchanges have more inactive users in comparison to more niche domains of discussion. We explicitly compare the effects of skew and sparsity in our prediction results on these datasets (\Cref{sec:Result Analysis} and 7.5).


==> inference.tex <==
% !TEX Root=draft.tex

\section{Model Inference}
\label{sec:Model Inference}
%\input{datadesc}
In this section, we describe an efficient Gibbs-sampling approach for model inference, analyze its computational complexity and propose a parallel batch-sampling approach for speed-up. In each iteration of Gibbs-sampling, we unseat users one at a time and re-sample their seating as in ~\Cref{eq:updatedCRP}. Profile and Action-topic distributions are simultaneously updated, while hyper-parameters are modified between Gibbs iterations. We factor the seating sampler (\Cref{ul}) for efficiency since the number of tables is not fixed. We speed-up convergence times with coherent initial seating based on similar action distributions and content tags.\vspace{-20pt}
% We iteratively sample user seating and update profile parameters to reflect the seating until mutual convergence as illustrated in \cref{crpmap}.
%\subsection{Inference via Gibbs Sampling}
%\label{subsec1}
% \subsubsection{Tables Initialization:}

% \subsubsection{Sampling Seating Arrangements:}
\begin{center}

 \begin{figure}[b]
 \vspace{-10pt}
  \includegraphics[width=0.86\linewidth, trim={4.25cm 1.9cm 6.1cm 0cm},clip]{images/image_intro.pdf}
 \caption{Our Gibbs-sampler simultaneously samples the seating arrangement of users (eq. 13) and learns profiles to describe the seated users (eq. 9, 10, 11). Users are grouped by behavioral similarity to overcome sparsity.}
  % \caption{Illustration of our Skew-aware Partitioning and Profiling Approach, Note that profiles are learned at the partition level to tackle inactive users. Our seating process simultaneously samples user partitions and learns profiles.}
  \label{crpmap}
 \end{figure}
\end{center}


\begin{center}
 \begin{table}[t]
%  \vspace{10pt}
  \begin{tabular}{lp{0.7\linewidth}}
   \toprule
   \textbf{Symbol}                         & \textbf{Description}                                                                            \\
   \midrule
   $n_{k}^{(w)}, n_{k}^{(a)}, n_{k}^{(.)}$ & Number of times word $w$, action $a$ were assigned to topic k, and respective marginals         \\
   $n_r^{(k)}, n_r^{(.)}$                  & Number of times interactions of users served profile $r$ was assigned topic k and marginal      \\
   $n_{r,r'}^{(\ell)}, n_{r,r'}^{(.)}$     & Number of $\ell$-labeled exchanges, all exchanges between users in tables serving $r$ with $r'$ \\
   \bottomrule
  \end{tabular}
  \label{gibbsnotation}
%   \vspace{-10pt}
  \caption{Gibbs-sampler count variables}
  \vspace{-15pt}
 \end{table}
\end{center}



The likelihood of generating a user interaction $d = (a,W,t) \in \mathcal{D}_{u}$ conditional on action-topic $k \in K$ is:
\begin{equation}
 p(a,W \mid k) \propto  \frac{n_{k}^{(a)} + \alpha_{\mathcal{A}}}{n_{k}^{(.)} + |\mathcal{A}|\alpha_{\mathcal{A}}} \times \prod_{w \in W}\frac{n_{k}^{(w)} + \alpha_{\mathcal{V}}}{n_{k}^{(.)} + |\mathcal{V}|\alpha_{\mathcal{V}}}.
 \label{dk}
\end{equation}
Thus, the likelihood $p(d \mid r)$ of interaction $d = (a,W,t)$ for a user  served activity profile $r \in R$,~\Cref{eqx} is:
\begin{equation}
 p(d \mid r) \propto \sum_{k \in K} \frac{n_{r}^{k} + \alpha_K}{n_{r}^{(.)} + |K|\alpha_K} \times p(a,W,t \mid k,r).
 \label{dr}
\end{equation}
The likelihood that knowledge exchange occurs between profile pairs $(r, r')$ on type $\ell$ is:
\begin{equation}
 \phi_{r,r'}^{\mathcal{L}}(\ell) = \frac{n_{r, r'}^\ell + \alpha_{\mathcal{L}}}{n_{r, r'}^{(.)} + |\mathcal{L}|\alpha_{\mathcal{L}}}.
 \label{lr}
\end{equation}
Thus, the conditional likelihood in~\Cref{upfinal} can be obtained via~\Cref{dr} over $\mathcal{D}_u$ and~\Cref{lr} over $L_u$ respectively. We can seat a user $u$ either on an existing table $x \in \{1, \ldots, \chi\}$ serving profile $r_x$ or on a new table $\chi+1$; \Cref{eq:updatedCRP}, conditioned on the seating of all other users, denoted by $x_{-u}$. To avoid likelihood computation over all tables, we perform the draw in two factored steps. We first sample the profile served to $u$ by marginalizing over tables via~\Cref{eq:profiledist-eq2},


\begin{equation}
 P( r \mid u, x_{-u}) \sim \left ( \frac{N_{r} - \chi_{r} \delta}{N+\gamma}  + \frac{\gamma+\chi\delta}{|R|(N+\gamma)}   \right ) p(u \mid r),
 \label{ul}
\end{equation}
and then sample from the set of tables serving the sampled profile (including the possibility of a new table with this profile draw),
\begin{equation}
 P(x \mid r, u, x_{-u}) \sim
 \begin{cases}
  \frac{n_{x}-\delta}{N+\gamma} \times \mathbbm{1}(r_x = r), & x \in \{1,\ldots, \chi \}, \\
  \frac{\gamma+\chi\delta}{N+\gamma} \times \frac{1}{|R|},   & x = \chi+1                 \\
 \end{cases}
 \label{user_seat}
\end{equation}
Note that $N = |\mathcal{U}|-1$, i.e. all users except $u$. If we draw a new table $\chi+1$, we assign the sampled profile variable $r$. We update all counts (~\Cref{gibbsnotation}) corresponding to prior profile and action-topic assignments for $u$.

% Given $p(u \mid r)$ we can sample profile $r_u$ for user $u$ as in \cref{eq:profiledist},
%
%where $a_{-u},r_{-u},k_{-u}$ indicate the seating and profile assignments of all other users, and the behavior assignments for their interactions. Behavior assignments for each interaction $d \in \mathcal{D}_u$ are sampled in proportion to \cref{dr} with $r = r_u$, the chosen profile for $u$, and the user is seated either on an existing table $a \in [1, A]$ serving $r_u$, or new table $A+1$ with $r_{A+1} = r_u$,


% \subsubsection{Parameter Estimation: }\label{parameter}
We use well known techniques to update parameters. At the end of each sampling iteration, we update Multinomial-Dirichlet priors $\alpha_{\mathcal{V}}$, $\alpha_{\mathcal{A}}$, $\alpha_{K}$ and $\alpha_{\mathcal{L}}$ by Fixed point iteration~\cite{fpi}. We update Beta parameters $(\alpha_{r,k}, \beta_{r,k})$ by the method of moments~\cite{tot}. We round all time-stamps to double-digit precision and we cache probability values $p(t \mid r,k)$ $\forall$ $t \in [0,1], r \in R, k \in K$ at the end of each sampling iteration, thus avoiding $R \times K$ scaling for $p(u \mid r)$ in~\Cref{ul}. While we fix the Pitman-Yor parameters in our experiments for simplicity, if needed, we can estimate them via auxiliary variable sampling~\cite{pytm, teh}.

\subsubsection*{\textbf{Computational Complexity}}
Our inference is linear in the number of users $|\mathcal{U}|$ and interactions $|\mathcal{D}|$ , scaled by $R + K$ (see empirical results in~\Cref{fig:memtime}). To see this, notice that in each Gibbs iteration, computing~\Cref{dk,dr} involves $|\mathcal{D}| \times (K+R)$ computations.~\Cref{ul} requires an additional $|\mathcal{U}| \times R$ computations. We prevent $R \times K$ scaling for $p(u\mid r)$ in~\Cref{ul} by caching. We cache the first product term of~\Cref{ul} for each $r \in R$, and update it only when there is a change in the seating arrangements on tables serving profile $r$.

\subsubsection*{\textbf{Parallelization with Batch Sampling}}
We scale to massive datasets by parallelizing inference via batch-sampling. The Gibbs sampler described above samples each user's seating $P( x_u \mid u, x_{-u})$ in \Cref{user_seat}, conditioned on all other users. This necessitates iteration over $\mathcal{U}$. Instead, seating arrangements could be simultaneously sampled in batches $U \subset \mathcal{U}$ conditioned on all users outside the batch, i.e. $P( x_{U} \mid U, x_{\mathcal{U}-U})$ where $x_{U}$ denotes the table assignments to users in batch $U$. For efficiency, batches must be chosen with comparable computation. We approximate computation for $u \in \mathcal{U}$ $\propto$ $|\mathcal{D}_u| + |\mathcal{L}_u|$ to decide apriori batch splits for sampling iterations. Note that when batch sampling, we can only exploit knowledge exchange links between users in the batch and users \textit{not} in the batch. In practice, since $|U| \ll |\mathcal{U}|$, the impact of not using knowledge exchanges between users in the same batch turns out to be negligible.


==> temp.tex <==

We use standard classifiers and evaluation metrics. Characterization and Recommendation use linear-kernel SVM evaluated with Precision, Recall, F1-Score and Area-Under-Curve (AUC). Future Activity Prediction uses Linear Regression. Both were implemented with default parameters in sklearn \footnote{http://scikit-learn.org/}. For the activity prediction task, we measure the Root Mean Squared Error (RMSE) in predicted activity proportions for $\textit{(topic, action)}$ pairs against actual proportions of users in the held-out future activity. We compute results with 5-fold cross-validation for each dataset. Statistically significant gains (Paired t-test, $p<0.05$) are in bold.


\subsection{Results}
\label{sec:Result Analysis}
We examine the experimental results for each of the three tasks---User characterization, question recommendation and future activity prediction in this section.

% \textbf{User Characterization Tasks (Reputation, Certification)\\}

% \subsubsection{User Characterization Tasks (Reputation, Certification)}
% \label{sub:User Characterization Tasks (Reputation, Certification)}
Our method improves on the baselines in the \textit{reputation prediction task} by 6.26-15.97\% AUC averaged across the Stack-Exchanges; \Cref{tab:reputation prediction} shows the results with statistically significant improvements in bold. LadFG performs slightly better on the overall precision in reputation prediction (not statistically significant), likely due to over-fitting of the embeddings to user-level data resulting in low recall. Our ability to discover more distinct user clusters even with the same latent dimensions as baselines (refer \cref{combined_clusters}) is the main reason for our gains in predicting reputation. Similarly, we improve on \textit{certification prediction} (see~\Cref{tab:certificate prediction}) by 6.65-21.43\% AUC averaged over MOOCs.

\begin{table}[t]
 \caption{Reputed User Prediction ($\mu\pm\sigma$ across Stack-Exchanges). We obtain improvements of 6.65-21.43\% AUC.}
 \vspace{-10pt}
 \centering
 \begin{tabular}{@{}ccccc@{}}
  \toprule
  \textbf{Method} & \textbf{Precision} & \textbf{Recall}          & \textbf{F1-score}        & \textbf{AUC}             \\
  \midrule
  LRC             & 0.73 $\pm$ 0.04    & 0.69 $\pm$ 0.04          & 0.72 $\pm$ 0.03          & 0.73 $\pm$ 0.03          \\
  DMM             & 0.69 $\pm$ 0.05    & 0.65 $\pm$ 0.04          & 0.66 $\pm$ 0.04          & 0.70 $\pm$ 0.04          \\
  LadFG           & 0.86 $\pm$ 0.03    & 0.75 $\pm$ 0.03          & 0.79 $\pm$ 0.02          & 0.80 $\pm$ 0.03          \\
  FEMA            & 0.79 $\pm$ 0.04    & 0.73 $\pm$ 0.03          & 0.77$\pm$ 0.03           & 0.79 $\pm$ 0.04          \\

  BLDA            & 0.75 $\pm$ 0.04    & 0.71 $\pm$ 0.04          & 0.74 $\pm$ 0.03          & 0.74 $\pm$ 0.04          \\
  CMAP            & 0.85 $\pm$ 0.02    & \textbf{0.83 $\pm$ 0.03} & \textbf{0.84 $\pm$ 0.02} & \textbf{0.86 $\pm$ 0.02} \\
  \bottomrule
 \end{tabular}
 \label{tab:reputation prediction}
 \vspace{-2pt}
\end{table}


\begin{table}[b]
\vspace{-4pt}
 \begin{tabular}{@{}ccccc@{}}
  \toprule
  \textbf{Method} & \textbf{Precision}       & \textbf{Recall}          & \textbf{F1-score}        & \textbf{AUC}             \\
  \midrule
  LRC             & 0.76 $\pm$ 0.04          & 0.71 $\pm$ 0.05          & 0.74 $\pm$ 0.04          & 0.72 $\pm$ 0.03          \\
  DMM             & 0.77 $\pm$ 0.03          & 0.74 $\pm$ 0.04          & 0.75 $\pm$ 0.03          & 0.74 $\pm$ 0.03          \\
  LadFG           & 0.81 $\pm$ 0.02          & 0.78 $\pm$ 0.02          & 0.79 $\pm$ 0.02          & 0.79 $\pm$ 0.02          \\
  FEMA            & 0.78 $\pm$ 0.03          & 0.75 $\pm$ 0.04          & 0.76 $\pm$ 0.03          & 0.78 $\pm$ 0.03          \\

  BLDA            & 0.80 $\pm$ 0.04          & 0.75 $\pm$ 0.03          & 0.77 $\pm$ 0.03          & 0.77 $\pm$ 0.04          \\
  CMAP            & \textbf{0.86 $\pm$ 0.02} & \textbf{0.81 $\pm$ 0.03} & \textbf{0.83 $\pm$ 0.02} & \textbf{0.84 $\pm$ 0.02} \\
  \bottomrule
 \end{tabular}
%  \vspace{-2pt}
  \caption{Certificate Earner Prediction ($\mu \pm \sigma$ across MOOCs); CMAP improves upon baselines by 6.65-21.43\% AUC}
 \vspace{-20pt}
 \label{tab:certificate prediction}

\end{table}



%\vspace{-15pt}
% \begin{flushleft}
% \textbf{Question Recommendation Task (Stack-Exchanges)\\}

% \subsubsection{Question Recommendation Task (Stack-Exchanges)}
% \label{sub:Question Recommendation Task (Stack-Exchanges)}

For the \textit{question recommendation task}~\Cref{tab:question recommendation}, we see gains between 6-47\% AUC over the baselines. To do well in this task, we require the model to make finer distinctions between the topical preferences of users; user reputation and action style are also important in this task.
% \end{flushleft}


\begin{table}[!htbp]
 \centering
 \caption{Question Recommendation ($\mu\pm\sigma$ across Stack-Exchanges)with 6.30-47.45\% AUC gains for CMAP. DMM performs quite well owing to importance of content in this task.}
 \vspace{-10pt}
 \begin{tabular}{@{}ccccc@{}}
  \toprule
  \textbf{Method} & \textbf{Precision}       & \textbf{Recall}          & \textbf{F1-score}        & \textbf{AUC}             \\
  \midrule
  LRC             & 0.65 $\pm$ 0.06          & 0.57 $\pm$ 0.08          & 0.60 $\pm$ 0.06          & 0.57 $\pm$ 0.05          \\
  DMM             & 0.72 $\pm$ 0.04          & 0.81 $\pm$ 0.05          & 0.75 $\pm$ 0.04          & 0.74 $\pm$ 0.04          \\
  LadFG           & 0.88 $\pm$ 0.03          & 0.60 $\pm$ 0.02          & 0.71 $\pm$ 0.02          & 0.76 $\pm$ 0.04          \\
  FEMA            & 0.79 $\pm$ 0.05          & 0.73 $\pm$ 0.06          & 0.77$\pm$ 0.05           & 0.79 $\pm$ 0.03          \\

  BLDA            & 0.70 $\pm$ 0.04          & \textbf{0.84 $\pm$ 0.04} & 0.77 $\pm$ 0.03          & 0.75 $\pm$ 0.04          \\
  CMAP            & \textbf{0.89 $\pm$ 0.03} & 0.81 $\pm$ 0.02          & \textbf{0.85 $\pm$ 0.03} & \textbf{0.84 $\pm$ 0.02} \\
  \bottomrule
 \end{tabular}
%  \vspace{1.5pt}
 \label{tab:question recommendation}
 \vspace{-5pt}
\end{table}

%
% \subsubsection{Future Activity Prediction Task :}
% \label{sub:Future Activity Prediction Task :}

%
% \begin{flushleft}
%  \textbf{Future Activity Prediction Task :\\}
%   \end{flushleft}
For the \textit{future activity prediction task}, our method shows gains over baselines in RMSE by 12\%-25\% on MOOCs and between 9.5\%-22\% on Stack-Exchanges; (see~\Cref{tab:future activity prediction}). Gains are explained by our model's ability to make finer distinction on action styles, and to be able to make better distinctions between profiles assigned to users.


\begin{table}[b]
 \vspace{-2pt}
 \centering
 \begin{tabular}{@{}cccccc@{}}
  \toprule
  \textbf{Method} & \textbf{DMM}   & \textbf{LadFG} & \textbf{FEMA}  & \textbf{BLDA}  & \textbf{CMAP}           \\
  \midrule
  MOOC            & 4.9 $\pm$ 0.4  & 4.2 $\pm$0.3   & 4.1 $\pm$ 0.2  & 4.4  $\pm$ 0.4 & \textbf{3.6  $\pm$ 0.2} \\
  Stack-Ex        & 8.6  $\pm$ 0.6 & 7.9  $\pm$ 0.4 & 7.5  $\pm$ 0.3 & 7.4  $\pm$ 0.5 & \textbf{6.7  $\pm$ 0.4} \\
  \bottomrule
 \end{tabular}
%  \vspace{1.5pt}
\caption{Future Activity Prediction (RMSE ($\times 10^{-2}$) $\mu \pm \sigma$), Lower RMSE is better. CMAP ouperforms baselines in MOOCs (12\%-25\%) and Stack-Exchanges (9.5\%-22\%)}
 \label{tab:future activity prediction}
 \vspace{-15pt}
\end{table}

%\subsection{Characterizing Inactive Users}
%\label{sub:Effects of data sparsity}
%In order to study the gains of our algorithm on characterizing users with different levels of activity, we split participants in each dataset into four equal partitions based on their number of interactions (Quartiles 1-4, 1 being least active). We then sample participants from each quartile and evaluate all methods on prediction performance (AUC).
%
%Our model shows magnified gains (\Cref{data_sparsity}) in prediction performance over baseline models in the first and second quartiles which correspond to users with limited activity. BLDA performs the weakest in Quartile-1 since it relies on interaction activity to build user representations. These gains confirm our ability to group inactive users in appropriate paritions.

In this section, we showed impressive performance gains on three types of tasks for our model over state of the art baselines. In the next section, we qualitatively analyze the reasons for it's success.

\vspace{-6pt}
\subsection{Why does CMAP work well?}
\label{sub:Why does CMAP work well?}

To interpret the gains obtained by CMAP, we examine the extracted clusters in~\Cref{sub:The Impact of Profile Driven Seating} and then look at users responsible for the performance gains of our model in~\Cref{sub:Making gains on inactive users}.
\vspace{-2pt}
\subsubsection{\textbf{The Impact of Profile Driven Seating}}
\label{sub:The Impact of Profile Driven Seating}

We now compare clusters obtained through CMAP seating against conventional generative assignments in BLDA~\cite{blda} on Stack-Exchanges. Both models group users best described by the same profile to form clusters. We use average user reputations of the clusters (appropriately normalized) as an external validation metric for cluster quality. We also run our model excluding time and knowledge-exchanges to see the effect on the clusters.~\Cref{ask_ubuntu_clusters} shows the result from the \texttt{Ask-Ubuntu} Stack Exchange, and~\Cref{cmap_clusters} shows the main activities and topics of the top three CMAP clusters. %\hs{is~\Cref{cmap_clusters} the full CMAP?}.
\begin{figure}[b]
 \vspace{6pt}
 %\includegraphics[width=\columnwidth]{./data/qualitative/ask_ubuntu_1.pdf}
 \includegraphics[width=\columnwidth]{./images/foo.pdf}
 \vspace{-10pt}
 \caption{Bubbles denote user clusters discovered by each model in the Ask-Ubuntu dataset (Bubble size $\propto$ Users in Cluster). CMAP discovers fine distinctions of reputed users (Profiles 1,2,3,4) by content preference and activity (\Cref{cmap_clusters}). BLDA clusters are mean-sized and close to the population average in reputation. In contrast, our assignments better reflect the behavior skew of users in the dataset.}
 \label{ask_ubuntu_clusters}
\end{figure}
We make the following key observations from the clusters:
\begin{description}
 \item[The Mean-Shift problem:] The Dirichlet-Multinomial setting in BLDA tends to merge profiles and hence shift cluster sizes and average participant reputation closer to the mean.~\Cref{ask_ubuntu_clusters} shows that 15 of 20 BLDA clusters have nearly the same size and average reputation. Both variants of CMAP show diversity in cluster size and high reputation variability across tables. Our cluster assignments appear to mirror the behavior skew for \texttt{Ask-Ubuntu} (c.f.~\Cref{skew_sparsity}).\\
 \item[Profile Quality:] CMAP learns finer variation in the topic affinities and actions of expert users. We can observe these variations from~\Cref{ask_ubuntu_clusters} and from~\Cref{cmap_clusters}. The top three profiles are of higher reputation, smaller in size, and from~\Cref{cmap_clusters}, each of these clusters shows distinct activities different from the mean activity. CMAP clusters appear to better reflect skewed user activity (c.f.~\Cref{d1}) and content preference (c.f.~\Cref{skew_sparsity}) with flexible profile-driven seating.
\end{description}

\begin{figure*}
 \centering
 \includegraphics[width=\textwidth]{./data/qpwide.pdf}
 \vspace{-22pt}
 \caption{Effects of activity sparsity on prediction tasks (AUC) for Stack Exchanges (datasets 1-10) and MOOCs (datasets 11-14). CMAP has greatest performance gains in Quartile-1 (Sparse users), performance gap reduces for very active users (Quartile-4).}
 \label{data_sparsity}
\end{figure*}

\begin{center}
 \begin{table}[b]


  \vspace{-10pt}
  \begin{tabular}{@{}cp{0.4\linewidth}p{0.4\linewidth}@{}}
   \toprule
   \textbf{Cluster} & \textbf{Action Style}                                & \textbf{Common Topics}                            \\
   \midrule
   1                & +31\% Answer, +24\% Edits, -9\% Questions            & Graphics Drivers, Booting Issues, Disk Partitions \\
   2                & +67\%Answer,	-3\% Edits, \hspace{2cm}-21\% Questions & Gnome, Desktop, Package Install                   \\
   3                & +11\% Answer, -4\% Edits, +47\% Questions            & Script, Application, Sudo Access                  \\
   \bottomrule
  \end{tabular}
    \caption{Action and Content description of users in top-3 clusters discovered by CMAP in Ask-Ubuntu, +/- values of action proportions against the average Ask-Ubuntu user}
  \label{cmap_clusters}
  \vspace{-17.7pt}
 \end{table}
\end{center}
%
% \begin{itemize}
%  \item \textbf{BLDA Clusters are Uninformative due to Mean-Shift: } The Dirichlet-Multinomial setting in BLDA tends to merge profiles and hence shift clusters closer to mean sizes and reputation. Our cluster assignments appear to better reflect the known disparities in the user population (\Cref{skew_sparsity}).
%  \item \textbf{Profile-Driven Seating: } CMAP clusters appear to better reflect uneven/skewed user activity (\Cref{d1}) and content preference (\Cref{skew_sparsity}) with flexible profile-driven seating.
%  \item \textbf{Profile Quality: }The mean-shift effect degrades information content of the learned profile variables in BLDA. For instance, expert users in our clusters (\Cref{cmap_clusters}) are not coherently grouped in the BLDA assignments.
%  \item \textbf{Profile Resolution: } Our assignments appear to discover finer variation in the topic affinities and actions of expert users, which enables fine-grained latent profile learning.
%
%        %This is particularly important in content recommendation and user characterization (\cref{sub:Prediction Tasks}).
%
% \end{itemize}
\begin{figure}[!htbp]
 \vspace{-15pt}
 %\includegraphics[width=\columnwidth]{./data/qualitative/combined_clusters_1.pdf}
 \includegraphics[width=\columnwidth]{images/foo2.pdf}
 \vspace{-16.5pt}
 \caption{Bubbles denote clusters in other Stack-Exchanges (Bubble size $\propto$ Users in Cluster). CMAP discovers highest reputation clusters in all datasets (Thick red dot, Top-left). BLDA clusters tend to mean reputation, size (Mean-Shift) not capturing disparities. In our case, profiles 1,2,3,4 appear to capture niche, highly reputed user behaviors}
 \vspace{1pt}
 \label{combined_clusters}
\end{figure}


\vspace{-13pt}
We observe a similar trend in the aggregated clusters obtained from all the other Stack-Exchange datasets  (c.f.~\Cref{combined_clusters}). The Dirichlet-Multinomial setting in BLDA results in similarly sized clusters which cannot model highly skewed content and action affinities of users. Note the fewer high-reputation clusters of BLDA in comparison to the finer distinctions of reputed users in our model. Our performance in prediction and recommendation reflect these observations, we see significant gains in our ability to characterize reputed users and recommend suitable content (\Cref{sub:Prediction Tasks}).

\subsubsection{\textbf{Making gains on inactive users}}
\label{sub:Making gains on inactive users}

We now investigate the source of our gains. We split users in each Stack-Exchange and MOOC into four quartiles based on interaction count (Quartile 1 is least active, 4 most). Then, we evaluate each method on Reputation and Certificate Prediction AUC in each quartile 
%\hs{reputation AUC, or certificate prediction AUC?}
of Stack Exchange and MOOC datasets respectively.

Our model shows large gains (\Cref{data_sparsity}) in Quartiles 1,2 that contain sparse users. We attribute these gains due to our joint profile learning to describe similar users seated on tables. The decision to address skew and sparsity jointly has two advantages: better profile fits for sparse users; more distinct and informative profiles in skewed scenarios. In contrast, models building representations  at the user level perform weakly in Quartiles-1,2 since these methods rely on interaction volume. We make smaller gains in Quartiles 3,4. %T

\textbf{To summarize: } jointly addressing sparsity and skew by profile driven seating is responsible for our gains. Importantly, the clusters are coherent, the model learns fine distinctions in behavioral profiles and exhibits behavior skew found in the underlying data.

% We re-iterate a few key observations from the high-reputation clusters in the Ask-Ubuntu dataset (\Cref{cmap_clusters}, \Cref{ask_ubuntu_clusters}) with our model:
% \begin{itemize}
%  \item \textbf{Distinct Action-Styles :} The mutual enhancement of user seating and profile learning results in more distinct profiles. Both the topic content and actions of users in \Cref{cmap_clusters} show significant
%  \item \textbf{Size Variations :} This is closely related to the first point. If we require distinctive action styles, the profile sizes must vary owing to behavior skew (very few users display certain trends of activity). Our seating is better suited to such scenarios due to it's exploration of niche profiles and discounting of the common and larger profiles as described with \Cref{eq:profiledist}.
% \end{itemize}
% These improvements aid us in both recommending suitable content (\Cref{tab:question recommendation}) as seen in the question recommendation result, as well as future activity prediction for users (\Cref{tab:behavior prediction}).

% (We are yet to add the content recommendation experiments, currently running them). The below plots indicate our ability to identify and profile niche high reputation user groups within each stack exchange (Blue bubbles indicate users grouped under profiles discovered by BLDA, while red bubbles are ours, bubble size indicates the percentage of the population placed under the profile). Conventional CRP seating cannot account for the details of the latent user model when generating clusters, the resulting clusters thus would not capture latent patterns of user interaction shared by users grouped together. Based on the below plots, our grouping discovers coherent patterns of user interaction with content which result in users possesssing a high or a low reputation. Users seated together share these traits and hence exhibit similar levels of reputation.
%
%Ask-Ubuntu, original dataset vs deskewed version. Our results can be seen to be closely aligned with BLDA in the deskewed version, however diverging in the original dataset to discover niche high reputation groups.
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/skew.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/deskew.pdf}
%\end{figure}
%
%
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/1.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/2.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/3.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/4.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/5.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/6.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/7.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/8.pdf}
%\end{figure}
%\begin{figure}[htbp]
% \includegraphics[width=\columnwidth]{./data/qualitative/9.pdf}
%\end{figure}
\vspace{-3pt}
\subsection{What if there was less Skew?}
\label{b_skew}
In this section, we study a counterfactual: what if the real-world datasets were less skewed?
%
% observed behavioral skew was less than observed?
% What is the effect of reducing the overall behavior skew so that different action styles are more balanced in the dataset?
To study this question, we sub-sample users who predominantly perform the two most common actions in our largest datasets, \texttt{Ask-Ubuntu} (Comments and Questions) and \texttt{Comp Sci-1 MOOC} (Play and Skip). These users are sub-sampled by half while retaining all other users, hence reducing overall action skew in the data. Baseline models are expected to perform better with reduced skew. All models degrade in Ask-Ubuntu owing to significant loss of content.
%Eliminating skew completely is very hard owing to significant content loss and high skew in the original datasets.~\Cref{tab:skew} shows the results of the prediction tasks(in terms of AUC) after partially de-skewing data.
\begin{table}[b]
 \centering
%  \vspace{1pt}
%   \vspace{-10pt}
 \begin{tabular}{@{}rcccc@{} }
  \toprule
  \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{@{}c}{\textbf{Ask-Ubuntu}} & \multicolumn{2}{c@{}}{\textbf{CompSci1 MOOC}}\\
  \cmidrule(lr){2-3} \cmidrule(lr){4-5}
        & Original       & Deskewed       & Original       & Deskewed \\
  \midrule
  LRC   & 0.671          & 0.656          & 0.713          & 0.734    \\
  DMM   & 0.647          & 0.611          & 0.684          & 0.672    \\
  LadFG & 0.734          & 0.718          & 0.806          & 0.830    \\
  BLDA  & 0.706          & 0.683          & 0.739          & 0.788    \\
  CMAP  & \textbf{0.823} & \textbf{0.746} & \textbf{0.851} & 0.849    \\
  \bottomrule
 \end{tabular}
%  \vspace{2pt}

 \label{tab:skew}
 \caption{CMAP outperforms baselines (AUC) in the de-skewed datasets, but with smaller gains}
 \vspace{-15pt}
\end{table}

\vspace{3pt}

Table 11 shows that CMAP still maintains a lead owing to inactive users. We also investigate performance gains in a highly skewed and sparse Stack-Exchange (Ask-Ubuntu) vs least skewed (Christianity) in Table 12. On average, we outperform baselines by 13.3\% AUC for Ask-Ubuntu vs 10.1\% for Christianity Stack-Exchange in User Characterization.
\begin{table}[t]
 \centering
%  \vspace{-1pt}

\vspace{-8pt}
 \begin{tabular}{@{}ccccccc@{}}
  \toprule
  \textbf{Method} & \textbf{DMM} & \textbf{LRC} & \textbf{LadFG} & \textbf{FEMA} & \textbf{CMAP}  & \textbf{BLDA} \\
  \midrule
  Ask-Ubuntu      & 0.647        & 0.671        & 0.734          & -             & \textbf{0.823} & 0.706         \\
  Christianity    & 0.684        & 0.720        & 0.842          & 0.818         & \textbf{0.856} & 0.791         \\
  \bottomrule
 \end{tabular}
%  \vspace{1.5pt}
 \label{tab:ubuntu-christianity}
 \caption{We see greater gains for User Characterization in a high-skew dataset (Ask-Ubuntu) vs low-skew (Christianity)}
	\vspace{-6pt}
\end{table}
% skip for wsdm 2018
% The seating arrangement of participants resulting from our model reflects behavior skew. The model distributes participants more evenly across profiles in comparison to the original datasets. The TableSum terms from \cite{eqn} are more uniformly distributed. Our CRP assignment process adapts to the extent of behavioral skew present in the data (c.f.~\Cref{fig:skew}). The figure illustrates the effect of varying the discount parameter $\delta$. A higher value of $\delta$ creates a ``fatter'' tail of activity profiles.
%
% \begin{figure}[htbp]
%  \includegraphics[viewport = .75in 0in 14.25in 6.75in ,clip, width=\columnwidth]{./data/skew.pdf}
%  \caption{Effect of varying the discount parameter $\delta$ on the seating arrangement. A higher value of $\delta$ favors the creation of more tables, thus creating a ``fatter'' activity profile distribution.}
%  \label{fig:skew}
% \end{figure}
\subsection{Scalability Analysis}
\label{sub:Scalability Analysis}
We compared the runtimes and memory consumption of our serial and batch-sampling (with 8 cores) inference algorithms with other models, for different volumes of interaction data obtained from random samples of the Ask-Ubuntu Stack-Exchange. BLDA is the fastest among the set of compared models. Our 8x batch sampler is comparable to BLDA in runtime. FEMA was the least scalable owing to the $O(|\mathcal{U}|^2)$ growth of the User-User regularizer matrix. ~\Cref{fig:memtime} shows the comparisons between the algorithms.
%\begin{figure}[htbp]
% \includegraphics[viewport = .25in 0in 7.5in 5.5in ,clip, width=\columnwidth]{./data/memtime.pdf}
% \caption{Effects of dataset size on algorithm runtime and memory consumption. BLDA is the fastest among the set of compared models. }
% \label{fig:memtime}
%\end{figure}
\begin{figure}[htbp]
\vspace{-9pt}
 \includegraphics[width=\columnwidth]{./data/memtime.pdf}
 \vspace{-24pt}
 \caption{Effects of dataset size on algorithm runtime and memory consumption. BLDA is the fastest among the set of compared models. }
 \vspace{-5pt}
 \label{fig:memtime}
 \vspace{-4pt}
\end{figure}

\vspace{-5pt}
\subsection{Parameter Sensitivity Analysis}
\label{sub:Parameter Sensitivity Analysis}

Our model is primarily impacted by three parameter values: number of profiles $R$, number of Action-Topics $K$ and discount $\delta$. We find results to be stable in a broad range of parameter values indicating that in practice our model requires minimal tuning (\Cref{fig:parameter sensitivity}). It is worth noting that while $R$ primarily impacts the granularity of the discovered activity profiles, K impacts the resolution of content-action associations. Dirichlet and other hyper-parameters have negligible impact on the profiles and seating arrangement learned. Our inference algorithm converges within 1\% AUC in less than 400 sampling iterations across all datasets.
\begin{figure}[!htbp]
\vspace{-9pt}
 \includegraphics[viewport = 1.25in 0in 16.75in 4.55in ,clip, width=\columnwidth]{./data/mp7.pdf}
 \vspace{-18pt}
 \caption{Mean performance(AUC) \& 95\% confidence interval with varying model parameters one at a time: $\delta$, $R$, $K$. Stability is observed in broad ranges of parameter values.}
 
 \label{fig:parameter sensitivity}
\end{figure}


%\begin{figure}[!htbp]
% \includegraphics[height=0.2\textwidth]{./data/gibbs.pdf}
% \caption{Model convergence over sampling iterations}
% \label{fig:gibbs}
%\end{figure}

\subsection{Limitations}
\label{limitations}
We identify two limitations. First, we make no assumptions about the structure of knowledge (e.g. a knowledge of ``probability'' is useful to understand ``statistical models''); incorporating knowledge structure, perhaps in the form of an appropriate prior will help with better understanding participants with low activity. Second, we assume a bounded time range. Development of latent profiles for streaming activity can lead to deployment with real-time data.

It would be an interesting exercise to observe the effect of dynamic updates to Pitman-Yor hyper-parameters over sampling iterations \cite{teh}. Although such an approach has been explored for LDA \cite{wallach}, it is unclear how over-fitting in our approach can be avoided in case of hyper-parameter drift. We plan this study for future work.
% domain ontology  or make use of any external

% Most of our errors arise from sparse users with ambiguous activity, who could be assigned inappropriate profiles. External sources of data could be integrated to aid us in such cases. Our model also assumes a bounded time range and is inapplicable to streaming data. Furthermore, our profiles are purely data-driven and do not provide a way to encode prior beliefs on behavior trends. We plan to address these shortcomings of our approach in future work.
% \begin{figure*}
%  \subfigure[b][]{
%   \centering
%   \includegraphics[width=0.32\linewidth]{plots/varyingR}
%  }
%  \subfigure[b][]{
%   \centering
%   \includegraphics[width=0.32\linewidth]{plots/varyingK}
%  }
%  \subfigure[b][]{
%   \centering
%   \includegraphics[width=0.32\linewidth]{plots/varyingD}
%  }
%
%  \caption{Effects on model performance of  (a) Varying Profiles R  (b) Varying Behaviors K  (c) Varying discount parameter $\delta$}
% \end{figure*}
% \begin{center}
% \begin{table*}
% \begin{tabular}{cp{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}
% p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}
% p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}}
% \toprule
% \multirow{2}{*}{\textbf{Method \textbackslash Data}} & \multicolumn{4}{c}{\textbf{AskUbuntu}} & \multicolumn{4}{c}{\textbf{Android}} & \multicolumn{4}{c}{\textbf{Travel}} & \multicolumn{4}{c}{\textbf{Chemistry}} & \multicolumn{4}{c}{\textbf{Christianity}}\\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
% & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC\\
% \midrule
% LRC & & & & & 0.78 & 0.67 & 0.72 & 0.74 & 0.80 & 0.70 & 0.75 & 0.76 & 0.81 & 0.65 & 0.73 & 0.75 & 0.62 & 0.81 & 0.70 & 0.66\\
% DMM & & & & & 0.84 & 0.61 & 0.70 & 0.74 & 0.75 & 0.84 & 0.79 & 0.78 & 0.65 & 0.77 & 0.71 & 0.68 & 0.62 & 0.92 & 0.74 & 0.68\\
% LadFG & & & & & 0.78 & 0.65 & 0.72 & 0.76 & 0.84 & 0.79 & 0.81 & 0.82 & 0.83 & 0.69 & 0.74 & 0.75 & 0.86 & 0.81 & 0.84 & 0.84\\
% BLDA & & & & & 0.80 & 0.65 & 0.72 & 0.75 & 0.81 & 0.79 & 0.79 & 0.80 & 0.74 & 0.68 & 0.71 & 0.72 & 0.79 & 0.78 & 0.79 & 0.80\\
% FEMA &-&-&-&-& 0.73 & 0.67 & 0.70 & 0.71 &  0.84 & 0.78 & 0.81 & 0.82 & 0.80 & 0.68 & 0.73 & 0.75 & 0.84 & 0.78 & 0.81 & 0.82\\
% Ours & & & & & 0.87 & 0.79 & 0.83 & 0.84 & 0.88 & 0.82 & 0.84 & 0.85 & 0.89 & 0.70 & 0.78 & 0.81 & 0.87 & 0.82 & 0.84 & 0.85\\
% \bottomrule
% \end{tabular}
% \end{table*}
% \end{center}
%
% \begin{center}
% \begin{table*}
% \begin{tabular}{cp{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}
% p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.02\linewidth}p{0.045\linewidth}}
% \toprule
% \multirow{2}{*}{\textbf{Method \textbackslash Data}} & \multicolumn{4}{c}{\textbf{CS1 Mooc}} & \multicolumn{4}{c}{\textbf{CS2 Mooc}} & \multicolumn{4}{c}{\textbf{Science Mooc}} & \multicolumn{4}{c}{\textbf{Math Mooc}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17}
% & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC & P & R & F1 & AUC \\
% \midrule
% LRC & & & & & 0.83 & 0.74 & 0.78 & 0.79 & 0.82 & 0.68 & 0.75 & 0.77 & 0.80 & 0.76 & 0.78 & 0.79\\
% DMM & & & & & 0.88 & 0.77 & 0.83 & 0.83 & 0.81 & 0.80 & 0.81 & 0.81 & 0.82 & 0.78 & 0.80 & 0.79\\
% LadFG & & & & & 0.84 & 0.78 & 0.81 & 0.82 & 0.82 & 0.79 & 0.80 & 0.80 & 0.79 & 0.73 & 0.76 & 0.78\\
% BLDA & & & & &  0.80 & 0.76 & 0.77 & 0.78 & 0.77 & 0.58 & 0.66 & 0.70 & 0.78 & 0.75 & 0.76 & 0.77\\
% FEMA &-&-&-&-& 0.83 & 0.76 & 0.79 & 0.80 & 0.72 & 0.69 & 0.70 & 0.72 & 0.74 & 0.73 & 0.74 & 0.73\\
% Ours & & & & &  0.87 & 0.83 & 0.85 & 0.86 & 0.85 & 0.82 & 0.83 & 0.84 & 0.85 & 0.82 & 0.84 & 0.84\\
% \bottomrule
% \end{tabular}
% \end{table*}
% \end{center}
\vspace{-7pt}
